Load Balancing in the Non-Degenerate Slowdown Regime

We analyse Join-the-Shortest-Queue in a contemporary scaling regime known as the Non-Degenerate Slowdown regime. Join-the-Shortest-Queue (JSQ) is a classical load balancing policy for queueing systems with multiple parallel servers. Parallel server queueing systems are regularly analysed and dimensioned by diffusion approximations achieved in the Halfin-Whitt scaling regime. However, when jobs must be dispatched to a server upon arrival, we advocate the Non-Degenerate Slowdown regime (NDS) to compare different load-balancing rules. In this paper we identify novel diffusion approximation and timescale separation that provides insights into the performance of JSQ. We calculate the price of irrevocably dispatching jobs to servers and prove this to within 15% (in the NDS regime) of the rules that may manoeuvre jobs between servers. We also compare ours results for the JSQ policy with the NDS approximations of many modern load balancing policies such as Idle-Queue-First and Power-of-$d$-choices policies which act as low information proxies for the JSQ policy. Our analysis leads us to construct new rules that have identical performance to JSQ but require less communication overhead than power-of-2-choices.

==> ECOMPANION.tex <==
%!TeX root = paper.tex

%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Main head for the e-companion
\ECHead{Additional Notation}

For our proofs, we will require some notation in addition to the notation required to state our proofs.

% M, M_{>3}

For the $k$th queueing network, we let $M^{(k)}_l(t)$ give the number of servers that have $l$ jobs at time $t$. We, also, define
\[
M^{(c)}_{\geq l}(t) = \sum_{l' \geq l} M^{(c)}_l(t)\qquad \text{and} \qquad M^{(c)}_{\leq l}(t) = \sum_{l'\leq l} M^{(c)}_l(t).
\]
Note that $I^{(k)}(t)=M^{(k)}_0(t)$. Further, we let 
\[
N^{(c)}_{\geq l}(t) = \sum_{l' \geq l} l M^{(c)}_l(t)
\]
the number of jobs in queues of size $l$ or more.

The following identity counts the number of jobs for queue sizes above and below $2$ and will be useful for our analysis of JSQ. 
\[
N^{(k)} = 2k - 2I^{(k)} - M^{(k)}_1 + N^{(k)}_{\geq 3}.
\]
which implies 
\begin{equation}\label{eq:MIdentity}
\Mk_1 = (2k - \Nk)-2\Ik + \Nk_{\geq 3}.
\end{equation}

\ECHead{Proofs of Statements}


\section{Outline of Theorem \ref{JSQ:Thrm}'s Proof.}

% EXPLAIN HIGH LEVEL IDEA OF THE PROOF
\Neil{The high level idea of the proof is...}

The process $N^{(k)}$ can be represented in the following form
\[
N^{(k)}(t) = {\mathcal N}_a\Big( (k\mu -\alpha)t\Big) - {\mathcal N}_d \left( \int_0^t \mu k - \mu I^{(k)}(s)  ds \right)
\]
where ${\mathcal N}_a$ and ${\mathcal N_d}$ are independent unit Poisson processes corresponding to arrivals and departures. 
Letting 
\[
{\mathcal M}^{(k)}_a (s) = \frac{{\mathcal N}_a (k^2 s)}{k} - k s\qquad \text{and}\qquad {\mathcal M}^{(k)}_d (s) = \frac{{\mathcal N}_d (k^2 s)}{k} - ks,
\]
we have that 
\[
\hat{N}^{(k)}(t) = {\mathcal M}_a\left( \mu t - \frac{\alpha}{k}t \right) - {\mathcal M}_a\left( \mu t - \frac{1}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) - \alpha t + \frac{1}{k}\int_0^{kt} I^{(k)}(s)ds
\]
In Lemma EC.3 part ii it is shown that 
\[
\frac{1}{k^2} \int_0^kt I^{(k)}(s) ds \Rightarrow 0
\]


thus by Billingsley ?? \Neil{fill in}, we have that 
\[
 \left({\mathcal M}_a\left( \mu t - \frac{\alpha}{k}t \right) - {\mathcal M}_a\left( \mu t - \frac{1}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) : t\geq 0\right)  \Rightarrow (\sqrt{2\mu}B(t) : t\geq 0) 
\]
where $B(t)$ is a standard Brownian motion.
The main difficulty that remains is to prove that 
\[
\frac{1}{k}\int_0^{kt} I^{(k)}(s) ds \xrightarrow[k\rightarrow \infty]{} \int_0^t  \frac{(2-\hat{N}(s))_+}{(\hat{N}(s) -1) } ds
\]

This is divided into two parts, 
\begin{itemize}
\item In section ?? it is shown that \Neil{}
\[
\frac{1}{k}\int_0^{kt} I^{(k)}(s) - \frac{\hat{M}^{(k)}_1(s)}{(1-\hat{M}^{(k)}_1(s) ) } ds \rightarrow 0.
\]
\item In section ??, we show that $\hat{M}^{(k)}_1(t)$ can be approximated by $(2-\hat{N}^{(k)}(t))_+$. 
\end{itemize}
This is then sufficient to show that 
\[
\int_0^{kt}  I^{(k)}(s) ds  - \int_0^{kt}  \frac{(2-\hat{N}^{(k)}(t))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds \xrightarrow[k\rightarrow 0]{} 0
\]  
So defining 
\[
\sqrt{2 \mu} {B}^{(k)}(t) = {\mathcal M}_a\left( \mu t - \frac{\alpha}{k}t \right) - {\mathcal M}_a\left( \mu t - \frac{1}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) + \int_0^{kt}  I^{(k)}(s) ds  - \int_0^{kt}  \frac{(2-\hat{N}^{(k)}(t))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds
\]
we have that 
\[
\hat{N}^{(k)}(t) =\sqrt{2 \mu} {B}^{(k)}(t) + \int_0^{kt}  \frac{(2-\hat{N}^{(k)}(t))_+}{(\hat{N}^{(k)}_1(s)-1 ) } - \alpha t ds 
\]
where $B^{(k)}$ converges weakly to a standard Brownian motion $B$. The solution to this differential equation in continuous with respect to changes in $B^{(k)}$, this is argued in Proposition ?? below. 


The arguments above imply that any limit point process $\hat{N}$ of this sequence must satisfy the stochastic differential equation
\[
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
\]
The sequence of random variables $( \hat{N}^{(k)} : k\in\bZ_+)$ is tight with respect to the uniform norm so such limit points must exist (This is proven in Proposition ?? below). 
Further, it is argued below that this SDE is path-wise unique (thus unique in law) and has sample paths that are strictly greater than one (see Proposition ??). This gives the uniqueness in distribution of the limit point $\hat{N}$. Remaining stated stationarity properties of this SDE are given below in Proposition ??.




\subsection{Properties of the $\hat{N}$ in its Stochastic Differential Equations}

\begin{proposition}[TIGHTNESS OF $\hat{N}$]
The laws of processes $( \hat{N}^{(k)} : k\in\bZ_+)$ are tight.	
\end{proposition}
\proof{Proof}
	a
\endproof



\begin{lemma}
	Consider the integral form
	\begin{equation}\label{IntForm}
	n(t) = n(0) + \sqrt{2\mu} b(t) + \mu \int_0^t \left[  \frac{(2-n(s))_+}{(n(s)-1)} - \alpha \right] dt.
	\end{equation}
	Let $b(t)$ is a continuous function and $n(t)$ is a strictly positive solution to the integral expression, above. If $(b^{(k)},n^{(k)})$ are a sequence of solution to the integral expression belonging to $D^2$ and such that $b^{(k)}$ converges uniformly on compacts to $b$
	then $n^{(k)}$ converges uniformly on compacts to $n$.
\end{lemma}




\proof{Proof}
Suppose $b(t)$ is continuous and such that $n(t)>0$. 
%
Let $\eta$ be the minimum value of $n(t)-1$ for $t\leq T$.
%
Thus the term in square-brackets in the integral form \eqref{IntForm} is Lipschitz continuous (with Lipschitz constant $\eta^{-2}$).  
% 
Let $\tau^{(k)}$ be the first time that $n^{(k)}\leq 1+ \eta/2$ occurs.
By assumption for each $\epsilon>0$, there exists a $K$ such the for all $k\geq K$ we have that 
\[
|b^{(k)}(0) - b(0) | 
+
\sqrt{2\mu}\sup_{t\leq T} \left| n^{(k)}(t) - n(t) \right| \leq \epsilon .
\]
Further we choose $\epsilon>0$ such that 
\begin{equation} \label{epsiloncond}
\epsilon < \frac{\eta}{2} e^{-\eta^{-2}T}
\end{equation}




With the triangle-inequality, we can bound the process for times $t\leq \tau^{(k)}\wedge T$ as follows
\[
| n^{(k)}(t) - n(t)| 
\leq 
| n^{(k)}(0) - n(0) | 
+ \sqrt{2\mu} |b^{(k)}(t)-b(t)| 
+  \mu \int_0^t 
\left|
\frac{(2-n^{(k)}(s))_+}{(n^{(k)}(s)-1)} - \frac{(2-n(s))_+}{(n(t)-1)}
\right| ds
\]
Thus applying the Lipschitz condition and maximizing over $t$ we have that
\[
\sup_{t\leq \tau^{(k)} \wedge T} 
| n^{(k)}(t) - n(t)| 
\leq 
| n^{(k)}(0) - n(0) | 
+ \sqrt{2\mu} \sup_{t\leq \tau^{(k)} \wedge T} |b^{(k)}(t)-b(t)| 
+  \mu \int_0^{\tau^{(k)} \wedge T}
\eta^{-2} \sup_{u\leq s} 
| n^{(k)}(u) - n(u)| ds 
\]
Applying Gronwall's Lemma, we have that
\begin{align}
\sup_{t\leq \tau^{(k)} \wedge T} 
| n^{(k)}(t) - n(t)|  
&\leq   
\left[ | n^{(k)}(0) - n(0) | 
+ \sqrt{2\mu} \sup_{t\leq T} |b^{(k)}(t)-b(t)| \right] e^{\eta^{-2} T} \\
&\leq \epsilon e^{\eta^{-2} T} \label{epsilonBound} \\
&< \frac{\eta}{2} \label{HitBound}
\end{align}
where the second inequality above holds by the definition of $\epsilon$ and the final inequality holds by condition \eqref{epsiloncond}. By Inequality \eqref{HitBound} we see that for our choice of $\epsilon$ that
\[
(n^{(k)}(t) -1) > (n(t) -1)  -\frac{\eta}{2} \geq \frac{\eta}{2} 
\]
for all times $t\leq \tau^{(k)}\wedge T$. Thus $\tau^{(k)}>T$, and therefore, Inequality \eqref{epsilonBound} now states 
\begin{equation}
\sup_{t\leq T} | n^{(k)}(t) - n(t)|
\leq   \epsilon e^{\eta^{-2} T}
\end{equation}
In otherwords, we see that as required
\[
\lim_{k\rightarrow\infty}\sup_{t\leq T} | n^{(k)}(t) - n(t)| = 0.
\]
\hfill \Halmos
\endproof
Note that the number of jobs in the $k$th system can be represented as follows:
\begin{equation}
N^{(k)}(t) 
= 
N^{(k)}(0) 
+ 
\mathcal N_A ( t\lambda^{(k)} )  
-
\mathcal N_D \Big( \mu \int_0^{t-} \left[ k - I^{(k)}(s) \right] ds \Big)
\end{equation}
where $\mathcal N_A$ and $\mathcal N_D$ are both unit Poisson processes. 

Therefore for the rescaled processes, adding and subtracting appropriate terms we have that
\begin{align*}
\hat{N}^{(k)}(t) 
=& \hat{N}^{(k)}(0) 
+
\frac{1}{k} \left[ \mathcal N_A ( tk\lambda^{(k)} )  - tk\lambda^{(k)}\right]
-
\frac{1}{k} \Big[ \mathcal N'_D (t k^2\mu) - k^2\mu t \Big] \\
&+ \frac{1}{k} \left[ \mathcal N'_D\left( \mu \int_0^{kt} I^{(k)}(s) ds \right) - \mu \int_0^{kt} I^{(k)}(s) ds \right] 
+ \mu \int_0^{kt} I^{(k)}(s) ds \\
&+ t [ \lambda^{(k)} - \mu ]
\\
=& \hat{N}^{(k)}(0) + \mathcal M^{(k)}_A (t)  - \mathcal M_D^{(k)}(t) + \mathcal M'^{(k)}_D (t)
+ \frac{1}{k}  \int_0^{kt} I^{(k)}(s) ds - \alpha t.
\end{align*}
Where $\mathcal M$ give martingales which converge to diffusions and $\mathcal M'$ converges to zero.




The following proposition summarizes the properties of SDE \eqref{JSQ:Diffusion}.
\begin{proposition}[JSQ of Diffusions]
	The SDE 
	\begin{equation}
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
	\end{equation}
	exists, is pathwise unique, is almost surely non-zero, has stationary distribution 
	\begin{equation}\label{JSQ:Equilibrium2}
	\frac{d\pi}{dn} = 
	\begin{cases}
	\exp \left\{ -\alpha (n-2) \right\}, & n \geq 2, \\
	(n-1)\exp \left\{ -(\alpha+1)(n-2) \right\}, & 1\leq n\leq 2.
	\end{cases}
	\end{equation}
	which is exponentially ergodic in the sense that ...
	and has expected value:
	\[
	\bE [N] = 
	\frac{
		e^{\alpha+1} 
		\Big[
		\frac{2}{(\alpha+1)^3}
		+
		\frac{1}{(\alpha+1)^2}
		\Big]
		-
		\Big[
		\frac{2}{(\alpha+1)^3}
		+
		\frac{3}{(\alpha+1)^2}
		+
		\frac{2}{(\alpha+1)}
		\Big]		
		+	
		\Big[
		\frac{1}{\alpha^2}
		+
		\frac{2}{\alpha}
		\Big]
	}
	{
		\frac{e^{(\alpha+1)}-1}{(\alpha+1)^2}
		+
		\frac{1}{\alpha(1+\alpha)}
	}
	\]
\end{proposition}
\proof{\Neil{Sketch Proof}}.(\Neil{See pages 5-6-7 on your NDS write.pdf for more details on continuity of solutions etc})
\Neil{Existence:} Existence is a consequence of the weak convergence result Theorem ??.\\
\Neil{Pathwise Uniqueness:} \Neil{You have two proofs here}  Is a consequence of Watanabe and Yamada pathwise-uniqueness Theorem. See Williams and Rogers, Theorem V.40.1. 	Given the event $\hat{N}=1$ does not occur, we can prove the result with a localization argument. In particular, for $\epsilon>0$ consider stopping time 
$\tau_\epsilon= \inf\{t : \hat{N}(t) = 1+\epsilon \}$. Then the processes $\hat{N}(t)$, for $t\leq \tau_\epsilon$ satisfies an SDE with Lispchitz coefficients. Such SDEs are known to be pathwise unique, for instance, see Rodgers and Williams, Theorem V.11.2 \NW{(Get reference)}. Thus for each $\epsilon>0$ the solutions to the SDE, \eqref{SDE}, are unique until time $\tau_\epsilon$. Further, by Lemma \ref{NotZero}, $\tau_\epsilon \rightarrow \infty$ as $\epsilon\rightarrow 0$. Thus this implies pathwise uniqueness of the SDE.\\
\Neil{Non-zero Property:} Is a consequence of the property of Bessel Processes. For $1< N < 2$ the process obeys the SDE
\begin{equation}
d \hat{N} (t) = \mu  \Big[ \frac{1}{\hat{N}-1}-(\alpha+1)\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
\end{equation}
which except for drift of $-(\alpha+1)$ is a Bessel process of Dimension 2. Of course by Girsanov's Theorem we can add and remove this drift (i.e. a zero probability event with drift is a zero probability event without a drift). It is well known that a $2$ dimensional Bessel process never hits zero (since two dimensional Brownian motion is Neighbourhood recurrent at zero, see Williams and Roger's Section VI.35 for a proof).\\
\Neil{Exponentially Ergodic:} This follows from notes of Martin Hairer (Convergence of Markov Processes, Section 7). \Neil{(Probably don't need this result.)}\\
\Neil{Expected Value Calculation:} This follows from repeated application of the identity,
\[
\int_0^{\infty} x^d e^{-\alpha x}dx = \frac{d!}{\alpha^{d+1}}
\]
for the calculation, see your pdf (Stationary Distributions.pdf).{\hfill \Halmos}
\endproof


\section{Timescale Separation}

\begin{theorem}
	Given $|Q_\kappa(0) - Q_{\kappa'}(0)| \leq 1$ and $I^{(k)}(0)=0$ and suppose that 
	\[
	\frac{N^{(k)}(0)}{k}\Rightarrow \hat{N}(0).
	\]
	For $1< \hat{N}(0) < 2$, 
	\[
	I^{(k)}\left(\frac{t}{k}\right) \Rightarrow \mathcal M(t)
	\]
	where $\mathcal M$ is a M/M/1 queue with arrival rate $(2 - \hat{N}(0))\mu$ and departure rate $\mu$.
	
	For $i \leq \hat{N}(0) \leq (i+1)$, $i\geq 2$ 
	\[
	M_{i-2} \left(\frac{t}{k}\right) \Rightarrow \mathcal M'(t)
	\] 
	where $\mathcal M'$ is an M/M/1 queue with arrival rate $\mu \hat{M}_{i-1}(0)$ and departure rate $\mu$.
\end{theorem}
\proof{Proof}{\Neil{To Do}}
\endproof


\section{State Space Collapse}
\begin{proposition}[State Space Collapse]\label{Thrm:StateSpaceCollapse}
\NW{$$ |M_1 - (2k - N_+)| \leq 2 k^{1/2} $$}
\end{proposition}

%%%% 
\Neil{(Reread and clean up the lemma below)}
The following is a basic equality on hitting probabilities of Markov chains.
\begin{lemma}\label{HittingLemma}
Consider a continuous time birth death process taking values $n$ in $\{0,...,x\}$. Let $f(n)$ be the rate of transitions from $n$ to $n+1$, for $n \neq x$, and $g(n)$ be the rate of transitions from $n$ to $n-1$ for $n\neq 1$. All other transition rates from $n$ are zero. The probability of hitting $x$ before $0$ starting from $1$ is given by the expression
\[
\frac{1}{\sum_{n=1}^x \prod^{n-1}_{m=1} \frac{g(m)}{f(m)}}. 
\]
\end{lemma}
\proof{Proof}
The $h_n^x$ be the probability of hitting $x$ before zero when starting from state $n$. 
%
It is clear that $h_n^x$ satisfies the expression
\[
(f(n) + g(n))  h_n^x = f(n) h_{n+1}^x + g(n) h_{n-1}^x 
\]
for $n=1,...x-1$ and $h^x_0=0$ and $h^x_x=1$. Let $u_n = h_n-h_{n-1}$ then the above expression simplifies to give
\[
0=f(n) u_{n+1} - g(n) u_n
\]
for $n=1,...,x$, which implies 
\[
u_n = u_1 \prod_{m\leq n-1} \frac{g(m)}{f(m)}
\]
for $n=1,..,x$. Now since 
\[
u_1^x =h_1^x - h_0^x = h_1^x \qquad \text{and} \qquad 1 = h^x_x - h^x_0 = \sum_{n=1}^x u_n 
\]
we have that
\[
 1=h_1^x   \sum_{n=1}^x \prod_{m\leq n-1} \frac{g(x)}{f(x)} 
\]
as required.\hfill \Halmos
\endproof

\Neil{Remark: This lemma holds under JSQ and IQF}
This lemma can immediately used to bound the number of idle servers in the following results
\begin{lemma}\label{lem:IdleBound}
i)	For $\epsilon>0$,
\[
\bP \left( \sup_{0\leq t\leq kT} \Ik(t) \geq k^{\frac{1+\epsilon}{2}} \right) \leq a k^2 e^{-b k^{\epsilon}} 
\]
where $a$ and $b$ are positive constants depending on $\mu$, $\alpha$ and $T$ only.\\

ii)
\[
\frac{1}{k}\int_0^{kt} I^{(k)}(s)ds \Rightarrow 0.
\]
\end{lemma}

Notice this Lemma implies that, when placed in the same probability space, a sequence JSQ networks will eventually never see a number of ilde servers above $k^{\frac{1+\epsilon}{2}}$. 
\proof{Proof of Lemma \ref{lem:IdleBound}}
i) Given $\Mk_1$ the number of queues of length $1$, the number of idle servers, $\Ik$ has transition rates
\begin{align*}
\Ik \nearrow \Ik +1 \quad &\text{at rate }\quad \mu \Mk_1\\
\Ik \searrow \Ik -1 \quad &\text{at rate }\quad \mu k-\alpha \quad (\text{when}\quad \Ik > 0).
\end{align*}
Since $M_1 \leq k - I^{(k)}$, we can dominate the process $I^{(k)}$ by the Markov chain $\tilde{I}$ given by the transition rates
\begin{align*}
\tilde{I} \nearrow \tilde{I} +1 \quad &\text{at rate }\quad \mu k - \mu \tilde{I}\\
\tilde{I} \searrow \tilde{I} -1 \quad &\text{at rate }\quad \mu k-\alpha \quad (\text{when}\quad \tilde{I} > 0).
\end{align*}
By Lemma \ref{HittingLemma} above, the probability of hitting $x$ before return to zero from state one is given by
\begin{align}
h^x_1 = \frac{1}{\sum_{n=1}^x \prod_{m \leq n-1} \left( \frac{\mu k-\alpha}{ \mu k - m}\right)} \label{Tagh}
&\leq 
\prod_{m \leq x-1} \left( \frac{ \mu k - m}{\mu k-\alpha}\right) \\
&\leq \exp\left\{ -\sum_{m\leq x-1}\left( \frac{m}{\mu k} - 2 \frac{\alpha}{\mu k} \right) \right\}
= \exp \left\{ -\frac{x(x-1)}{2\mu k} + \frac{2\alpha (x-1)}{\mu k}   \right\} \notag .
\end{align}
where in the first inequality we take only the lead term from the denominator of $h_1^x$; and in the second inequality, we apply the bound $e^{-2z}\leq 1-z \leq e^{-z}$ for $0\leq z\leq 1/2$. (Here we assume that $k$ is suitably large so that $\alpha/(\mu k)< 1/2$).  
Thus if we take $x= k^{\frac{1+\epsilon}{2}}$, for $\epsilon >0$, we have that 
\begin{equation}\label{excurisionbound}
h^{x}_1 \leq e^{-\frac{k^{\epsilon}}{2\mu}+ o(1)}.
\end{equation}


This bounds each individual excursion. Now we must (loosely) bound the possible number of such excursions.
Since the rate of creating idle servers is bounded above by a Poisson process of rate $\mu k$. Therefore the number of excursions in $\Ik$ from zero in time interval $[0,kT]$ is bounded above by, $Po(\mu T k^2)$, a Poisson random variable of mean $\mu T k^2$. A chernoff bound then gives,
\begin{equation}\label{PoissonBound}
\bP( Po(\mu T k^2) \geq (\mu+1) T k^2 ) \leq e^{-c k^2} 
\end{equation}
where $c$ is a constant depending of $\mu$ and $T$ only.

Thus applying a union bound and the bounds \eqref{excurisionbound} and \eqref{PoissonBound}, we have that 
\[
\bP\Big( \exists t\leq kT\; s.t.\; I^{(k)}(t) \geq k^{\frac{1+\epsilon}{2}} \Big) \leq (\mu +1)Tk^2 e^{-\frac{k^{\epsilon}}{2\mu}+ o(1)} +   e^{-c k^2} 
\]
It is not hard to see that for suitable choices of $a$ and $b$, we can achieve a bound of form required in Lemma \ref{lem:IdleBound}i).

We now prove part ii), which is an straightforward consequence of part i). Choose $\epsilon \in (0,1)$.  Thus
\begin{align*}
{\mathbb P} \left( \frac{1}{k^2}\int_0^{kT} I^{(k)}(s) ds \geq \epsilon \right) & \leq {\mathbb P} \left( \frac{T}{k} \cdot \!\!\sup_{0\leq t \leq kT} I^{(k)} (t) \geq \epsilon \right)\\
& \leq   {\mathbb P} \left(  \sup_{0\leq t \leq kT} I^{(k)}(t) \geq k^{(1+\epsilon)/2}\right)\xrightarrow[k\rightarrow \infty]{} 0
\end{align*} 
In the 2nd inequality above, we use the fact that for all $k$ sufficiently large $\epsilon > T k^{(-1+\epsilon)/2}$; and the above limit holds by part i).
\hfill \Halmos
\endproof

\Neil{NOW DO THE SAME PROPOSITION FOR THE VOLUME BELOW QUEUE SIZE 2 FROM YOU HANDWRITTEN NOTES}\\
\Neil{Remark: This lemma holds under JSQ and IQF}
\begin{lemma}\label{lem:VBound}
	For $\epsilon>0$,
	\[
	\bP \left( \exists t \leq kT\text{ s.t. } (2\Ik (t) + \Mk_1(t) )   \geq k^{\frac{1}{2}}\text{ and }M^{(k)}_{\geq 3}(t) \geq k^{\frac{1}{2}+\epsilon} \right) \leq a k^2 e^{-b k^{\epsilon}} 
	\]
	where $a$ and $b$ are positive constants depending on $\mu$, $\alpha$ and $T$ only.	
\end{lemma}
\proof{Proof}
Define
\[
\Vk(t)= 2\Ik(t) + \Mk_1(t)
\]
Notice that the transitions in $V(t)$ occur according to the following rates
\begin{align}
\Vk \nearrow \Vk +1 \quad &\text{at rate }\quad \Mk_1 + \Mk_2 = k\mu - \mu \Mk_{\geq 3} - \Ik \\
\Vk \searrow \Vk -1 \quad &\text{at rate }\quad \mu k - \alpha  \quad (\text{when}\quad \Vk > 0).
\end{align}
Suppose that $M_{\geq 3} \geq y$. Notice each time $M_{\geq 3}$ increases it must be that $\Vk=0$. So we analyse the excursions of $\Vk$ from zero when $M_{\geq 3} \geq y$. In particular, we want to bound the probability that $\Vk\geq x$. Let ${\tilde{V}}$ be defined by the transition rates
\begin{align*}
\tilde{V} \nearrow \tilde{V} +1 \quad &\text{at rate} \quad k\mu -\mu y \\
\tilde{V} \searrow \tilde{V} -1 \quad &\text{at rate} \quad k\mu -\alpha.
\end{align*}
By assumption $V\leq \tilde{V}$ and from Lemma \ref{HittingLemma} we have (by a bounds similar to \eqref{Tagh}) that


\begin{align*}
h^x_1 = \frac{1}{\sum_{n=1}^x \prod_{m \leq n-1} \left( \frac{\mu k-\alpha}{ \mu k - \mu y}\right)} 
&\leq 
 \left( \frac{ 1 - \frac{y}{k}}{1-\frac{\alpha}{\mu k}}\right)^{x-1} \leq \exp \left\{ -\frac{(x-1)y}{ k} + \frac{2\alpha (x-1)}{\mu k}   \right\} .
\end{align*}
Observe that if we let $x=k^{1/2}$ and $y=k^{1/2+\epsilon}$ then we have that 
\begin{equation}\label{hBound}
h_1^x \leq e^{-k^{\epsilon}+o(1)}.
\end{equation}

Again, this bounds each individual excursion. Now we must bound the possible number of such excursions.
Since the rate of increase in $\Vk$ is bounded above by a Poisson process of rate $\mu k$. Therefore the number of excursions in $\Vk$ from zero in time interval $[0,kT]$ is bounded above by, $Po(\mu T k^2)$, a Poisson random variable of mean $\mu T k^2$. A chernoff bound then gives,
\begin{equation}\label{PoissonBound}
\bP( Po(\mu T k^2) \geq (\mu+1) T k^2 ) \leq e^{-c k^2} 
\end{equation}
where $c$ is a constant depending of $\mu$ and $T$ only.

Thus applying a union bound and the bounds \eqref{hBound}and \eqref{PoissonBound}, we have that 
\[
\bP\Big( \exists t\leq kT\;\text{ s.t. }\; V^{(k)}(t) \geq k^{\frac{1}{2}}\text{ and } M^{(k)}_{\geq 3}(t) \geq x^{1/2+\epsilon}  \Big) \leq (\mu +1)Tk^2 e^{-\frac{k^{\epsilon}}{2\mu}+ o(1)} +   e^{-c k^2} 
\]
It is not hard to see that for suitable choices of $a$ and $b$, we can achieve a bound of form required in Lemma \ref{lem:VBound}. \hfill \Halmos
\endproof

\begin{lemma}
Suppose that $\tilde{I}$ is an M/M/1 queue with arrival rate $\alpha$ service rate $\beta$. Let $\tilde{T}$ be the length of the renewal cycle from the queue being of length $1$ to the queue being empty again. Then,
\[
{\mathbb P} (\tilde{T} \geq t ) \leq e^{\theta + \phi(\theta)t} \qquad \text{and}\qquad {\mathbb P} \left( \int_0^{\tilde{T}} \tilde{I}(s) ds \geq x\right) \leq e^{-\theta_0 \sqrt{cx}}
\] 	
where 
\[
\phi(\theta)=\alpha(e^{\theta}-1) +\beta(e^{-\theta}-1)  
\]
and  $\theta_0$ is such that $$\phi(\theta_0)+ c\theta_0 < 0.$$
\end{lemma}
\proof{Proof}\Neil{Sort out s and T} \Neil{Remove all the tildes, I --> Q ?}
We have that $\tilde{I}(0)=1$ and that
\[
\tilde{I}(s) = {\mathcal N}_{\alpha}(s) - {\mathcal N}_{\beta}(s)
\] 
for $t\leq \tilde{T}$ where ${\mathcal N}_\alpha$ and ${\mathcal N}_\beta$ are independent Poisson processes of rates $\alpha$ and $\beta$, respectively.  Note that
\[
\E \left[ e^{\theta ({\mathcal N}_{\alpha}(s) - {\mathcal N}_{\beta}(s))} \right]= e^{s \phi(\theta)}  \quad\text{where}\quad \phi(\theta)=\alpha(e^{\theta}-1) +\beta(e^{-\theta}-1)  
\]
(Note that, since $\alpha <\beta$, $\phi'(\theta)<0$. So $\phi(\theta)<0$ for some $\theta >0$.)	
Thus 
\[
X_t = \exp \left\{\theta \tilde{I}(t\wedge \tilde{T}  )  - (t\wedge \tilde{T})\phi(\theta) \right\}
\]
is a positive martingale which then gives
\[
{\mathbb E} \left[ e^{-\tilde{T}\phi(\theta)} \right] = \bE\left[ X_{\infty} \right]  \leq  {\mathbb E} \left[ X_0 \right] = e^{\theta}
\]
Applying a Chernoff bound, we get the inequality
\[
{\mathbb P} (\tilde{T} > t) \leq  {\mathbb E} \left[e^{-\phi(\theta) \tilde{T}} \right] e^{\phi(\theta)t} \leq e^{\theta + \phi(\theta)t}.
\]
This gives the required bound ??.
We could optimize the above bound over $\theta$ however the essential point is that $\phi(\theta) <0$ for $\theta >0$ and so the there is an exponential rate of convergence in the above bound. 

The second bound follows by a similar argument. Define 
\[
\tilde{I}^c(s) = {\mathcal N}_{\alpha}(s) - {\mathcal N}_{\beta}(s) + cs \quad \text{and}\quad 
X^c_t = \exp \left\{\theta I^c(t)  -\phi(\theta)t-ct\right\}
\]
for some constant $c$ such that $\alpha + c \leq \beta$. 
(Here we have essentially added an additional upward drift to our queueing process.) 
Again,
\[
\E \left[ e^{\theta ({\mathcal N}_{\alpha}(s) - {\mathcal N}_{\beta}(s) + cs) }  \right]= e^{s (\phi(\theta)+c\theta)}  \quad\text{where}\quad \phi(\theta)=\alpha(e^{\theta}-1) +\beta(e^{-\theta}-1)  
\]
Let $\tilde{T}_y$ be the first time that $X^c_t\geq y$ holds. Thus $X^c_{t\wedge \tilde{T}_z}$ is a positive martingale bounded above by $e^{\theta x}$. By the optional stopping theorem
\[
e^\theta = {\mathbb E} [ X_0^c] = {\mathbb E} [X^c_{\tilde{T}_c}] = {\mathbb E} [ e^{ \theta (z+1) - \tilde{T}_z (\phi(\theta) + c\theta)}  {\mathbb I} [ \tilde{T}_z < \infty] ]
\]

\Neil{Double check the z+1 here.}

Let $\theta^*$ be the largest solution to the equation $\phi(\theta^*) + c\theta^*=0$, we have that 
\[
{\mathbb P} (\tilde{T}_z<\infty) \leq e^{-\theta^* z} \leq e^{-\theta_0 z}
\]
Note that since $\phi(\theta) +c \theta$ is a convex function, zero at $\theta=0$ with $\phi'(0)+ c <0$. We have that $e^{\theta_0}$ upper bounds the above probability for any value of $\theta_0$ such that $\phi(\theta_0)+ c\theta_0 < 0$.

Now if $\tilde{T}_z<\infty$ then $\tilde{I}(t)$ lies below the line $(z-cs : s\geq 0)$. Thus 
\[
\int_0^{\tilde{T}_z} \tilde{I}(t) dt \leq \frac{z^2}{c} 
\] 
(note $\frac{z^2}{c}$ is the area of the triangle in the positive orthant with hypotenuses $(z-cs : s\geq 0)$.)  Therefore
\[
{\mathbb P} \Big( \int_0^{\tilde{T}}   \tilde{I}(t) dt \geq  \frac{z^2}{c}\Big) \leq e^{\theta_0 z}
\]
which after substitution gives the required result.

\hfill \Halmos\endproof

The following lemma argues that idleness occurs infrequently when $M_{\geq 3}$ is large.

\begin{lemma}
	\[
{\mathbb P}\left( \int_0^{kT} I^{(k)}(t) {\mathbb I} [ M_{\geq 3}(t) \geq k^{1/2 + \epsilon}]dt \geq k^{1/2+2\epsilon}\right)\leq A {k^{3/2}} e^{-Bk^{\epsilon}}
	\]
\end{lemma}
\proof{Proof}
	Given Lemma ?? (EC.3), we consider the event 	
\[
A:=\left\{ \exists t \leq kT\text{ s.t. } (2\Ik (t) + \Mk_1(t) )   \geq k^{\frac{1}{2}}\text{ and }M^{(k)}_{\geq 3}(t) \geq x^{\frac{1}{2}+\epsilon}\right\}
\]
We know from Lemma ?? that ${\mathbb P}(A) \leq ak^2 e^{-b k^{\epsilon}}$. 

Now consider $A^c$ the complement of $A$. On $A^c$, 
\begin{equation}\label{Mbound}
M_{1}^{(k)} \leq k^{1/2}.
\end{equation}
The idleness process has transition rates  

 \begin{align}
 &I^{(k)}\mapsto I^{(k)}+1 \qquad\text{at rate}\qquad \mu M_1^{(k)}\\
 &I^{(k)}\mapsto I^{(k)}+1 \qquad\text{at rate}\qquad \mu k -\alpha, \quad\text{ when }I^{(k)}>0
 \end{align}
Given \eqref{Mbound}, we consider the CTMC 
 \begin{align}
 &\tilde{I}\mapsto \tilde{I}+1 \qquad\text{at rate}\qquad \mu k^{1/2}\\
 &\tilde{I}\mapsto \tilde{I}+1 \qquad\text{at rate}\qquad \mu k -\alpha, \quad\text{ when } \tilde{I}^{(k)}>0
 \end{align}
Thus on event $A^c$, $I^{(k)}$ and $\tilde{I}$ can be coupled so that $I^{(k)}(t)\leq \tilde{I}(t)$ for all $t$ such that $0\leq t \leq kT$.

We now use Lemma ?? to bound the area under the excursions of $\tilde{I}(t)$. (Similar to EC.7 ??) We know that there are at most Poisson mean $\mu k^{3T/2}$ excursions of $\tilde{I}(t)$ in time $0$ to $kT$ and we know  
\[
{\mathbb P}\left( Po(\mu k^{3/2}T) \geq (\mu+1) k^{3/2} T \right) \leq e^{ck^{3/2}}
\]
For constant $c$ depending on $\mu$ and $T$ only.

Applying a union bound to these excursions, we have that 
\[
{\mathbb P}  \left( \int_0^{kT}  \tilde{I} (t) dt \geq x  \right)
\leq
(\mu+1) k^{3/2 }T {\mathbb P}  \left(  \int_0^{\tilde{T}} \tilde{I} (t)dt \geq \frac{x}{(\mu+1) k^{3/2} T}\right) + e^{-c \frac{3}{2}} 
\]
(I.e. in the above union bound, either there are less that $(\mu +1) k^{3/2}T$ ecusrions and then for the total area to be over $x$ the must be at least on excursion whose are is above $x/[(\mu+1) k^{3/2} T]$ or there are more that $(\mu+1)k^{3/2}T$ in which case ?? applied.) 

Now applying Lemma ?? (EC.4), where we note that we take parameter choices $\theta_0$, $c=\frac{k}{2}$ (notice $\phi(\theta_0))+ c \theta_0<0$ for all sufficiently large $k$) \Neil{Double Check this} So
\[
{\mathbb P} \left( \int_0^{\tilde{T}} \tilde{I}(t) dt \geq k^{ 2\epsilon-1}  \right)
\leq
(\mu+1) k^{3/2} T e^{-\gamma k^{\epsilon}} + e^{-ck^{3}{2}}
\]
which we can use to bound the integral of interest
\begin{align*}
{\mathbb P}\left( \int_0^{kT} I^{(k)}(t) {\mathbb I} [ M_{\geq 3}(t) \geq k^{1/2 + \epsilon}]dt \geq k^{1/2+2\epsilon}\right) &\leq {\mathbb P}(B\cap A^c) + {\mathbb P} (A)\\
& \leq (\mu +1) k^{3/2} T e^{-\gamma k^{\epsilon}} + e^{-ck^{3/2}}\\
&\leq A {k^{3/2}} e^{-Bk^{\epsilon}},
\end{align*}
where the last inequality hold for suitably chosen parameters $A$ and $B$. This gives the required bound.
\hfill \Halmos	\endproof

The following lemma which applies to Join-the-Shortest queue only, shows that $\Nk_{\geq 3}$ and $\Mk_{\geq 3}$ will be within a constant factor of one another.

\begin{lemma}
\Neil{fill this in}	
\end{lemma}

\proof{Proof of Proposition \ref{Thrm:StateSpaceCollapse}}
\eqref{eq:MIdentity}
Suppose that the two following events both hold:
\begin{align}
A 
&= 
\Big\{ I^{(k)}(t) \leq k^{\frac{1+\epsilon}{2}} \forall t\leq kT \Big\}\label{eq:Acond}
\\
B 
&= 
\Big\{ (2\Ik (t) + \Mk_1(t) )   \geq k^{\frac{1}{2}}\text{ and }M^{(k)}_{\geq 3}(t) \geq k^{\frac{1}{2}+\epsilon} \Big\}\label{eq:Bcond}
\end{align} 
We know by Lemma \ref{lem:IdleBound} and Lemma \ref{lem:VBound} that 
\[
\bP( A \cap B ) \geq 1- 2ak^2 e^{-bk^{\epsilon}}
\]
where $a$ and $b$ are constants depending on $\mu$, $\alpha$ and $T$.

We consider the identity:
\begin{equation}\label{eq:MIdentity}
\Mk_1 = (2k - \Nk)-2\Ik + \Mk_{\geq 3},
\end{equation}
(as was given in \eqref{eq:MIdentity}), under two separate conditions: 1. $M^{(k)}_{\geq 3} \leq k^{1/2+\epsilon}$ and 2. $M^{(k)}_{\geq 3} \geq k^{1/2+\epsilon}$.

First, when $M^{(k)}_{\geq 3} \leq k^{1/2+\epsilon}$, we know given event $A$ () and identity ?? that  
\[
| \M^{(k)}_1 - (2k-)
\]
\endproof


\section{Proof of Theorem \ref{I1F:Thrm}.}






==> ECOMPANION_2.tex <==
% !TeX root    = paper.tex
\section{Time Scale Separation}
\begin{lemma}
\[
J_A\left( 1- 4 \frac{\delta_k}{\mu \hat{M}_1^{(k)}(0)}\right) \leq J_A^{(k)} \leq J_A \left( 1+  4 \frac{\delta_k}{\mu \hat{M}_1^{(k)}(0)}\right)  
\] 
\end{lemma}



\begin{lemma}
\[
J_D \leq J_D^{(k)}	\leq J_D \left[ 1+ \frac{\alpha}{\mu k} \right]
\]
\end{lemma}

\begin{corollary}
	\[
	|J-J^{(k)}| \leq J \left[ \frac{4}{\mu M_1^{(k)}} \delta + 4\frac{\alpha}{\mu k}\right]
	\]	\end{corollary}
       

We also need jumps of the same type to occur, as the following lemma describes.
\begin{lemma}
	For constant C (not depending on k) we have that 
	\[
	{\mathbb P} \left( \hat{I}^{(k)}(J^{(k)}) -\hat{I}^{(k)} (J_-^{(k)}) \neq \hat{I}(J)-\hat{I}(J_-)\right)\leq C\delta_k
	\]
\end{lemma}




==> ECOMPANION_3.tex <==
% !TeX root   = paper.tex

%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this Appendix we prove our main result Theorem 1. A number of auxiliary results which are not specific to the line of investigation are contained in Appendix B.

%%% Main head for the e-companion
\section{Additional Notation}\label{sec:additional_notation}

Our proofs will require the following additional notation.
%
% M, M_{>3}
%
For the $k$ server JSQ system, we let $M^{(k)}_l(t)$ denote the number of servers that have $l$ jobs at time $t$. We, also, define
\[
M^{(k)}_{\geq l}(t) = \sum_{l' \geq l} M^{(k)}_{l'}(t)\qquad \text{and} \qquad M^{(k)}_{\leq l}(t) = \sum_{l'\leq l} M^{(k)}_{l'}(t).
\]
Note that $I^{(k)}(t)=M^{(k)}_0(t)$. Further, we let
\[
N^{(k)}_{\geq l}(t) = \sum_{l' \geq l} (l'-l + 1) M^{(k)}_{l'}(t)
\]
Think of $N^{(k)}_{\geq l}$ the number of jobs above queue level $l$. Further, given the NDS scaling \eqref{NNDS}, we define
\[
\hat{N}^{(k)}_{\geq l}(t) = \frac{N^{(k)}_{\geq l}(kt) }{k},\qquad \hat{M}^{(k)}_{\geq l}(t) =\frac{M^{(k)}_{\geq l}(kt)}{k},\quad  \text{and}\quad \hat{M}^{(k)}_{\leq l}(t) = \frac{M^{(k)}_{\leq l}(kt)}{k}.
\]




\section{Outline of Theorem \ref{JSQ:Thrm}'s Proof.}\label{sec:outline}

% EXPLAIN HIGH LEVEL IDEA OF THE PROOF
The process $N^{(k)}$ can be represented in the following form
\begin{equation}\label{NExpression}
N^{(k)}(t) - N^{(k)}(0) = {\mathcal N}_a\Big( (k -\alpha)\mu t\Big) - {\mathcal N}_d \left( \int_0^t \mu k - \mu I^{(k)}(s)  ds \right), \qquad t \geq 0 
\end{equation}
where ${\mathcal N}_a$ and ${\mathcal N_d}$ are independent unit rate Poisson processes corresponding to arrivals and departures. We can subtract the mean from these Poisson processes.
Under the NDS scaling, this gives the following expression
\begin{subequations}\label{NTerms}
	\begin{align}
	\hat{N}^{(k)}(t)- \hat{N}^{(k)}(0)  =& {\mathcal M}_a\left( \mu t - \frac{\alpha}{k}\mu t \right) - {\mathcal M}_d\left( \mu t - \frac{\mu}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) \label{NTermsa} \\
	& + \frac{\mu}{k^2}\int_0^{k^2t} \hat{I}^{(k)}(s)ds - \mu \int_0^{t}  \frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds \label{NTermsb}\\
	&- \alpha \mu t + \mu \int_0^{t}  \frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds.\label{NTermsc}
	\end{align}
\end{subequations}
where
\[
\hat{I}^{(k)}(t) ={I}^{(k)}\Big(\frac{t}{k}\Big) ,\qquad {\mathcal M}^{(k)}_a (s) = \frac{{\mathcal N}_a (k^2 s)}{k} - k s\qquad \text{and}\qquad {\mathcal M}^{(k)}_d (s) = \frac{{\mathcal N}_d (k^2 s)}{k} - ks.
\]
Both ${\mathcal M}_a^{(k)}$ and ${\mathcal M}_d^{(k)}$ are Martingales.

We consider the convergence of each term in \eqref{NTerms} separately. We will argue that the first term \eqref{NTermsa} converges to a Brownian motion; the second term \eqref{NTermsb} converges to zero; and third \eqref{NTermsc} has sufficient continuity of solutions with respect to the arrival/departure process given in \eqref{NTermsa} to converge to the required SDE. We now give a little more detail in reference to the following sections. 

First consider the term \eqref{NTermsa}. In Proposition \ref{lem:IdleBound}, it is shown that 
\[
\frac{1}{k^2} \int_0^{kt} I^{(k)}(s) ds \Rightarrow 0.
\]
This implies that arguments applied to $\mathcal{M}_a(\cdot)$ and $\mathcal{M}_d(\cdot)$ both weakly converge to the map $(t:t\geq 0) \mapsto (\mu t : t\geq 0)$. Thus, the Martingale Functional Central Limit Theorem gives that  \eqref{NTermsa} converges to a Brownian motion:

\[
 \left({\mathcal M}_a\left( \mu t - \frac{\alpha}{k}\mu t \right) - {\mathcal M}_a\left( \mu t - \frac{\mu}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) : t\geq 0\right)  \Rightarrow (\sqrt{2\mu}B(t) : t\geq 0) 
\]
where $B(t)$ is a standard Brownian motion. (A proof of the Martingale FCLT can be found in \cite{whitt2007} Theorem 2.1 and is stated in Theorem \ref{MgCLT}, below.) This deals with the term \eqref{NTermsa}.


Second we prove convergence to zero of \eqref{NTermsb}. Much of this article's technical novelty lies in proving the time-scale separation that 
\begin{align}
\label{eqTSS}
\left(\frac{1}{k^2}\int_0^{k^2t} \hat{I}^{(k)}(s) ds -\int_0^t  \frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s) -1) } ds\; :\; t\geq 0\right) \Rightarrow 0.
\end{align}
\noindent As discussed in Section \ref{sec:Heuristic} the idleness process, $\hat{I}^{(k)}$, is informed by the proportion of queues of size one, $\hat{M}^{(k)}_1$, which in turn is closely related to the mean queue size $\hat{N}^{(k)}$. We must obtain the limiting relationship between these quantities. 
This is divided into the following parts: 
\begin{itemize}
\item We show in Proposition \ref{Thrm:StateSpaceCollapse} that, with high probability,
\[
\sup_{0\leq t \leq T} \Big| \big(2-\hat{N}^{(k)}(t) \big)_+ - \hat{M}^{(k)}_1(t) \Big| = k^{-\frac{1}{2} + o(1)} .
\]
This implies that, with high probability, $\hat{I}^{(k)}$ undergoes transition rates of the form
\begin{subequations}\label{IMM1}
	\begin{align}
	&\hat{I}^{(k)}(t) \rightarrow \;\; \hat{I}^{(k)}(t) +1\;   &&\text{at rate }\quad \mu \hat{M}^{(k)}_1\Big(\frac{t}{k^2}\Big) =\mu\Big(2-\hat{N}^{(k)}\Big(\frac{t}{k^2}\Big) \Big)_+ + \mu k^{-\frac{1}{2} + o(1)}, &\\
	&\hat{I}^{(k)}(t) \rightarrow \Big(\hat{I}^{(k)}(t) -1\Big)_+\;   &&\text{at rate }\quad \mu \left( 1 -\frac{\alpha}{k}\right). &
	\end{align}
\end{subequations}
Section \ref{sec:PropEC2} is devoted to proving Proposition \ref{Thrm:StateSpaceCollapse}. 

\item We then prove that \eqref{eqTSS} holds in Proposition \ref{TimescaleIdleness}. To prove Proposition \ref{TimescaleIdleness}, we must show that the transitions \eqref{IMM1} are well approximated by the dynamics of an M/M/1 queue. To do this we first refine Proposition \ref{Thrm:StateSpaceCollapse} to show that the result holds over each excursion of the process $\hat{I}^{(k)}$. This is Proposition \ref{TightProp} proven in subsection \ref{subsec:Tight}. We then bound excursions and their transition rates above and below in Section \ref{BoundingI}. Finally we combine these in Section \ref{sec:Prop3Proof} where Proposition \ref{TimescaleIdleness} is proven. 
\end{itemize}
This verifies the convergence of \eqref{NTermsb}.

Third and final, we show convergence to the required SDE and analyze its properties.  
The processes \eqref{NTerms} and their limit diffusion are sequence of jump/differential equations of the form
\[
n(t) = n(0) + \sqrt{2\mu} b(t) + \mu \int_0^t \left[  \frac{(2-n(s))_+}{(n(s)-1)} - \alpha \right] ds.
\]
In this sequence, the terms corresponding to $b(t)$ converges to a Brownian motion. Similar to \cite{pang2007martingale}, we can argue that the solution $n$ to the above equation is a continuous function of $b$. This is proven in Lemma \ref{CTS_SDE} below. Thus the sequence of processes \eqref{NTerms} converges to an SDE of the required form
\[
d\hat{N}(t) =  \sqrt{2\mu} dB(t) + \mu\left[  \frac{(2-\hat{N}(t))_+}{(\hat{N}(t)-1)} - \alpha \right] dt.
\]
The sample-path properties of this SDE are analyzed in Lemma \ref{DiffZero}.
The stationary density of the above SDE is found in Proposition \ref{JSQ:EqPro}. The stationary expected queue size is a routine calculation.

These arguments, as outlined above, then give the proof of Theorem \ref{JSQ:Thrm}.
\begin{remark}
The above argument is made somewhat complicated by the discontinuity in coefficients of the above SDE at $\hat{N}=1$. However, it can be argued that $\hat{N}$ never hits $1$. This holds since at $\hat{N}=1$ the diffusion coefficient of the above SDE is similar to that of a Bessel Process of dimension $2$ -- a process which is known to never hit zero, cf. \cite[Theorem V.40.1.]{rogers2000diffusions} and Proposition \ref{DiffZero}. This allows us to prove weak convergence under an appropriate localizing sequence of stopping times, $(\tau^{(k)}(\eta) : k\geq 0)$, which then implies the required weak convergence. Further, it implies path-wise uniqueness of our SDE.
\end{remark}
\iffalse
This is then sufficient to show that 
\[
\int_0^{kt}  I^{(k)}(s) ds  - \int_0^{kt}  \frac{(2-\hat{N}^{(k)}(t))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds \xrightarrow[k\rightarrow 0]{} 0
\]  
So defining 
\[
\sqrt{2 \mu} {B}^{(k)}(t) = {\mathcal M}_a\left( \mu t - \frac{\alpha}{k}\mu t \right) - {\mathcal M}_a\left( \mu t - \frac{1}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) + \int_0^{kt}  I^{(k)}(s) ds  - \int_0^{kt}  \frac{(2-\hat{N}^{(k)}(t))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds
\]
we have that 
\[
\hat{N}^{(k)}(t) =\sqrt{2 \mu} {B}^{(k)}(t) + \mu \int_0^{kt}  \frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}_1(s)-1 ) } - \alpha \mu t ds 
\]
where $B^{(k)}$ converges weakly to a standard Brownian motion $B$. The solution to this differential equation in continuous with respect to changes in $B^{(k)}$, this is argued in Proposition ?? below. 


The arguments above imply that any limit point process $\hat{N}$ of this sequence must satisfy the stochastic differential equation
\[
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
\]
The sequence of random variables $( \hat{N}^{(k)} : k\in\bZ_+)$ is tight with respect to the uniform norm so such limit points must exist (This is proven in Proposition ?? below). 
Further, it is argued below that this SDE is path-wise unique (thus unique in law) and has sample paths that are strictly greater than one (see Proposition ??). This gives the uniqueness in distribution of the limit point $\hat{N}$. Remaining stated stationarity properties of this SDE are given below in Proposition ??.
\fi

\section{A First Idleness Bound}

The lemma below shows that the number of idle servers is always less than $k^{1/2+o(1)}$. This is then sufficient to prove convergence of the Brownian term found in the NDS limit. 

\begin{proposition}\label{lem:IdleBound}
	For $\epsilon>0$,
	\[
	\bP \left( \sup_{0\leq t\leq kT} \Ik(t) \geq k^{\frac{1}{2}+\epsilon} \right) \leq a k^2 e^{-b k^{\epsilon}} 
	\]
	where $a$ and $b$ are positive constants depending on $\mu$, $\alpha$ and $T$ only. Consequently,
	\[
	\frac{1}{k^2}\int_0^{kt} I^{(k)}(s)ds \Rightarrow 0
	\]
where convergence is uniform on compact time intervals.
\end{proposition}




Notice this Lemma implies that, when placed in the same probability space, a sequence of JSQ networks will eventually never see a number of idle servers above $k^{\frac{1}{2}+\epsilon}$. 
\proof{Proof}
Given the number of queues of length $1$, the number of idle servers, $\Ik$, has transition rates
\begin{align*}
\Ik \nearrow \Ik +1 \quad &\text{at rate }\quad \mu \Mk_1\\
\Ik \searrow \Ik -1 \quad &\text{at rate }\quad \mu(k-\alpha) \quad \text{for}\quad \Ik > 0.
\end{align*}
Since $M^{(k)}_1 \leq k - I^{(k)}$, we can stochastically dominate the process $I^{(k)}$ by the Markov chain $\tilde{I}$ given by the transition rates
\begin{align*}
\tilde{I} \nearrow \tilde{I} +1 \quad &\text{at rate }\quad \mu( k- \tilde{I})\\
\tilde{I} \searrow \tilde{I} -1 \quad &\text{at rate }\quad \mu(k-\alpha) \quad (\text{when}\quad \tilde{I} > 0).
\end{align*}
By Lemma \ref{HittingLemma}, the probability of $\tilde{I}$ hitting $x$ before return to zero from state one is given by
\begin{align*}
h^x_1 = \frac{1}{\sum_{n=1}^x \prod_{m \leq n-1} \left( \frac{ k-\alpha}{ k - m}\right)} \label{Tagh}
&\leq 
\prod_{m \leq x-1} \left( \frac{  k - m}{ k-\alpha}\right) \\
&\leq \exp\left\{ -\sum_{m\leq x-1}\left( \frac{m}{ k} - 2 \frac{\alpha}{ k} \right) \right\}
= \exp \left\{ -\frac{x(x-1)}{2 k} + \frac{2\alpha (x-1)}{ k}   \right\} \notag ,
\end{align*}
where, in the first inequality, we take only the lead term from the denominator of $h_1^x$; and, in the second inequality, we apply the bound $e^{-2z}\leq 1-z \leq e^{-z}$ for $0\leq z\leq 1/2$. (Here we assume that $k$ is sufficiently large so that $\alpha/ k< 1/2$).  
Thus if we take $x= k^{\frac{1}{2}+\epsilon}$, for $\epsilon >0$, we have that 
\begin{equation}\label{excurisionbound}
h^{x}_1 \leq e^{-\frac{k^{2\epsilon}}{2}+ o(1)} \leq e^{-\frac{k^{\epsilon}}{2}+ o(1)}.
\end{equation}


This bounds each individual excursion. Now we must bound the possible number of such excursions.
Since the rate of creating idle servers is given by departures which is bounded above by a Poisson process of rate $\mu k$. Therefore the number of excursions in $\Ik$ from zero in time interval $[0,kT]$ is bounded above by, $Po(\mu T k^2)$, a Poisson random variable of mean $\mu T k^2$. By Lemma \ref{PoissonBound}
\begin{equation}\label{PoissonBoundy}
\bP( Po(\mu T k^2) \geq 8\mu T k^2 ) \leq e^{-9 \mu T k^2} .
\end{equation}
Thus applying a union bound, the bounds \eqref{excurisionbound} and \eqref{PoissonBoundy} give that 
\[
	\bP \left( \sup_{0\leq t\leq kT} \Ik(t) \geq k^{\frac{1}{2}+\epsilon} \right)
=\bP\Big( \exists t\leq kT\; s.t.\; I^{(k)}(t) \geq k^{\frac{1}{2}+\epsilon} \Big) \leq 8\mu Tk^2 e^{-\frac{k^{\epsilon}}{2\mu}+ o(1)} +   e^{-9 \mu T k^2} \leq a e^{-bk^{\epsilon}} 
\]
where the final inequality holds for suitable choices of $a$ and $b$. This is the bound required in Proposition \ref{lem:IdleBound}.
The convergence 
\[
\frac{1}{k^2}\int_0^{kt} I^{(k)}(s)ds \Rightarrow 0
\]
 is now a straightforward consequence. For $\epsilon \in (0,\frac{1}{2})$, 
\begin{align*}
{\mathbb P} \left( \frac{1}{k^2}\int_0^{kT} I^{(k)}(s) ds \geq \epsilon \right) & \leq {\mathbb P} \left( \frac{T}{k} \cdot \!\!\sup_{0\leq t \leq kT} I^{(k)} (t) \geq \epsilon \right)\\
& \leq   {\mathbb P} \left(  \sup_{0\leq t \leq kT} I^{(k)}(t) \geq k^{\frac{1}{2}+\epsilon}\right)\xrightarrow[k\rightarrow \infty]{} 0.
\end{align*} 
In the 2nd inequality above, we use the fact that for all $k$ sufficiently large, $\epsilon > T k^{-1/2+ \epsilon}$.
\hfill \Halmos
\endproof

A consequence of the above proposition is the convergence to the Brownian motion term in our limiting SDE.

\begin{corollary}\label{Cor:MtoB}
\[
\left({\mathcal M}_a\left( \mu t - \frac{\alpha}{k} \mu t \right) - {\mathcal M}_a\left( \mu t - \frac{\mu}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) : t\geq 0\right)  \Rightarrow (\sqrt{2\mu}B(t) : t\geq 0) 
\]	
	\end{corollary}
\proof{Proof}
By Proposition \ref{lem:IdleBound}ii) 
\[
\left(\mu t - \frac{\mu}{k^2} \int_0^{kt} I^{(k)}(s)ds : t\geq 0\right) \Rightarrow  \mu \mathbf{e}
\]
Thus the Martingale Functional Central Limit Theorem applies (see Theorem \ref{MgCLT} for a statement and see \cite[Theorem 2.1 and Lemma 2.1]{whitt2007} for a proof) and so the result holds.\hfill \Halmos
\endproof




\section{State Space Collapse}\label{sec:PropEC2}
In this section, we provide a sequence of results that prove the following proposition.  

\begin{proposition}[State Space Collapse]\label{Thrm:StateSpaceCollapse} For $\epsilon >0$
\[
\bP\Big( \sup_{0\leq t\leq T} \Big|\big(2-\hat{N}^{(k)}(t)\big)_+ - \hat{M}^{(k)}_1(t) \Big| \geq k^{-1/2+\epsilon}\Big) \leq a \exp\{-b k^{\frac{\epsilon}{2}}\}
\]
for positive constants $a$ and $b$.
\end{proposition}

The proposition ensures that the number of jobs $\hat{N}^{(k)}$ can provide good proxy for the number of servers of length one, which in turn informs the transitions of the number of idle servers.

The proof of Proposition \ref{Thrm:StateSpaceCollapse}. Relies on the following lemma. After proving this lemma, we outline the proof of Proposition \ref{Thrm:StateSpaceCollapse}.

\begin{lemma}\label{Lem:AMIdentity}
	\begin{equation}\label{eq:AMIdentity}
	\big(2-\hat{N}^{(k)}(t)\big)_+ - \hat{M}^{(k)}_1(t)= \left(\hat{M}_1^{(k)}(t) + 2\frac{I^{(k)}(kt)}{k} - {\hat{N}^{(k)}_{\geq 3}(t)}\right)_+\!\! - \hat{M}_1^{(k)}(t).
	\end{equation}
\end{lemma}
\proof{Proof}
The following identity counts the number of jobs for queue sizes above and below $2$ and will be useful for our analysis of JSQ: 
\begin{equation*}
2k =  N^{(k)}  + 2I^{(k)} + M^{(k)}_1 - N^{(k)}_{\geq 3}
\end{equation*}
(See Figure \ref{Fig:Identity} for pictorial representation of this identity).
\begin{figure}[t]%
	\centering
	\includegraphics[width=0.9\textwidth]{figures/Identity.pdf}
	\caption{Representation of the identity $2k =  N^{(k)}  + 2I^{(k)} + M^{(k)}_1 - N^{(k)}_{\geq 3}$: $2k$ equals $N^{(k)}$ plus the number of jobs missing from box A which is $2 I^{(k)}$, plus the number missing from box B which is $M^{(k)}_1$, minus the number of jobs in box C which is $N^{(k)}_{\geq 3}$. 
		\label{Fig:Identity}}
\end{figure}%

The previous equality implies that
\begin{equation}\label{eq:MIdentity}
(2k - \Nk)_+ =  ( \Mk_1  +2\Ik - \Nk_{\geq 3})_+
\end{equation}
which after dividing by $k$ and subtracting $\hat{M}^{(k)}_1$ gives the required result. \hfill\halmos
\endproof

\iffalse
\Neil{This should not be here!}                                                                                                                                                     
\begin{corollary} 
	\[
	\sup_{0\leq t\leq \tau^{(k)}(\eta)} \left| \frac{1}{k} \int_{0}^{kt}	I^{(k)}(s)ds - \int_{0}^{t}\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}ds \right| \xrightarrow[k\rightarrow \infty]{} 0
	\]
	where the above convergence is convergence in probability.
\end{corollary}
\fi

The proof of Proposition \ref{Thrm:StateSpaceCollapse} requires us to appropriately bound the right-hand side of \eqref{eq:AMIdentity} in Lemma \ref{Lem:AMIdentity}. First in Proposition \ref{lem:IdleBound}, we showed that $I^{(k)} = k^{\frac{1}{2}+o(1)}$ with high probability. This implies that the number of idle servers does not have a significant impact on Proposition \ref{Thrm:StateSpaceCollapse}. Consequently,  $(2-\hat{N}^{(k)})_+$ can only differ significantly from $\hat{M}_1^{(k)}$, when both $\hat{M}_1^{(k)}$ and $N^{(k)}_{\geq 3}$ are large. However, this is not possible under a JSQ rule. This is proven in Lemma \ref{lem:VBound} and Lemma \ref{lem:Nbound}, and this point was discussed heuristically in Section \ref{sec:Heuristic}.

%\Neil{Remark: This lemma holds under JSQ and IQF}
%This lemma can immediately used to bound the number of idle servers in the following results

%\Neil{NOW DO THE SAME PROPOSITION FOR THE VOLUME BELOW QUEUE SIZE 2 FROM YOU HANDWRITTEN NOTES}\\
%\Neil{Remark: This lemma holds under JSQ and IQF}

\subsection{Further Idleness Bounds}\label{idlesness}
In this section we prove two somewhat more refined versions of Proposition \ref{lem:IdleBound} and each proof follows in a similar manner. Each lemma provides better bound on the terms in the identity \eqref{eq:AMIdentity}.
\begin{lemma}\label{lem:VBound}
	For $\epsilon>0$,
	\[
	\bP \left( \exists t \leq kT\text{ s.t. } (2\Ik (t) + \Mk_1(t) )   \geq k^{\frac{1}{2}}\text{ and }M^{(k)}_{\geq 3}(t) \geq k^{\frac{1}{2}+\epsilon} \right) \leq a_1  e^{-b_1 k^{\epsilon}} 
	\]
	where $a_1$ and $b_1$ are positive constants depending on $\mu$, $\alpha$ and $T$ only.	
\end{lemma}
\proof{Proof}
Define
\[
\Vk(t)= 2\Ik(t) + \Mk_1(t).
\]
(Notice this is the number of jobs that could be contained in boxes A and B in Figure \ref{Fig:Identity})

Notice that the transitions in $V^{(k)}(t)$ occur according to the following rates
\begin{align*}
\Vk \nearrow \Vk +1 \quad &\text{at rate }\quad \Mk_1 + \Mk_2 = k\mu - \mu \Mk_{\geq 3} - \mu \Ik \\
\Vk \searrow \Vk -1 \quad &\text{at rate }\quad \mu (k - \alpha)  \quad (\text{when}\quad \Vk > 0).
\end{align*}
Suppose that $M_{\geq 3} \geq y$. Notice that under JSQ $M_{\geq 3}$ increases only when $\Vk=0$. So we analyze the excursions of $\Vk$ from zero when $M_{\geq 3} \geq y$. In particular, we want to bound the probability that $\Vk\geq x$. Let ${\tilde{V}}$ be defined by the transition rates
\begin{align*}
\tilde{V} \nearrow \tilde{V} +1 \quad &\text{at rate} \quad k\mu -\mu y \\
\tilde{V} \searrow \tilde{V} -1 \quad &\text{at rate} \quad \mu (k -\alpha).
\end{align*}
By assumption excursions in $V^{(k)}$ are stochastically dominated by $\tilde{V}$. From Lemma \ref{HittingLemma}, we have that, when started from $\tilde{V}=1$, the probability of $\tilde{V}$ hitting $x$ before hitting zero is bounded as follows
\begin{align*}
h^x_1 = \frac{1}{\sum_{n=1}^x \prod_{m \leq n-1} \left( \frac{ k-\alpha}{  k - y}\right)} 
&\leq 
 \left( \frac{ 1 - \frac{y}{k}}{1-\frac{\alpha}{k}}\right)^{x-1} \leq \exp \left\{ -\frac{(x-1)y}{ k} + \frac{2\alpha (x-1)}{ k}   \right\} .
\end{align*}
where, in the first inequality, we take only the lead term from the denominator of $h_1^x$; and, in the second inequality, we apply the bound $e^{-2z}\leq 1-z \leq e^{-z}$ for $0\leq z\leq 1/2$.
Observe that if we let $x=k^{1/2}$ and $y=k^{1/2+\epsilon}$ then we have that 
\begin{equation}\label{hBound}
h_1^x \leq e^{-k^{\epsilon}+o(1)}.
\end{equation}

Again, this bounds each individual excursion. Now we must bound the possible number of such excursions.
Since the rate of increase in $\Vk$ is bounded above by a Poisson process of rate $\mu k$. Therefore the number of excursions in $\Vk$ from zero in time interval $[0,kT]$ is bounded above by, $Po(\mu T k^2)$, a Poisson random variable of mean $\mu T k^2$. Lemma \ref{PoissonBound} then gives that 
\begin{equation}\label{PoissonBound2}
\bP( Po(\mu T k^2) \geq 9 \mu T k^2 ) \leq e^{-10\mu T k^2} 
\end{equation}


Thus applying a union bound and the bounds \eqref{hBound}and \eqref{PoissonBound2}, we have that 
\[
\bP\Big( \exists t\leq kT\;\text{ s.t. }\; V^{(k)}(t) \geq k^{\frac{1}{2}}\text{ and } M^{(k)}_{\geq 3}(t) \geq k^{1/2+\epsilon}  \Big) \leq 9\mu Tk^2 e^{-\frac{k^{\epsilon}}{2\mu}+ o(1)} +   e^{-10 \mu T k^2} 
\]
It is not hard to see that for suitable choices of $a$ and $b$, we can achieve a bound of form required in Lemma \ref{lem:VBound}. \hfill \Halmos
\endproof

We now apply Lemma \ref{lem:VBound} to show that idleness occurs infrequently when $M_{\geq 3}$ is large. This will help us bound the maximum queue size in the next section. Again, the proof of Lemma \ref{2ndIdleBound} is a somewhat more sophisticated version of Proposition \ref{lem:IdleBound}.

\begin{lemma}\label{2ndIdleBound} For $\epsilon >0$, 
	\[
{\mathbb P}\left( \int_0^{kT} I^{(k)}(t) {\mathbb I} [ M_{\geq 3}(t) \geq k^{1/2 + \epsilon}]dt \geq k^{1/2+2\epsilon}\right)\leq a_2 {k^{2}} e^{-b_2 k^{\epsilon}}
	\]
	where $a_2$ and $b_2$ are positive constants depending on $\mu$, $\alpha$ and $T$ only.
\end{lemma}
\proof{Proof}
Given Lemma \ref{lem:VBound}, we consider the event 	
\[
A:=\left\{ \exists t \leq kT\text{ s.t. } (2\Ik (t) + \Mk_1(t) )   \geq k^{\frac{1}{2}}\text{ and }M^{(k)}_{\geq 3}(t) \geq k^{\frac{1}{2}+\epsilon}\right\}
\]
We know from Lemma \ref{lem:VBound} that ${\mathbb P}(A) \leq a_1k^2 e^{-b_1 k^{\epsilon}}$. 

Now consider $A^c$ the complement of $A$. On $A^c$, when $M^{(k)}_{\geq 3}(t)\geq k^{\frac{1}{2}+\epsilon}$ holds, it must be that
\begin{equation}\label{Mbound}
M_{1}^{(k)} \leq k^{1/2}.
\end{equation}
Recall the idleness process has transition rates  
 \begin{align*}
 &I^{(k)}\mapsto I^{(k)}+1 \qquad\text{at rate}\qquad \mu M_1^{(k)},\\
 &I^{(k)}\mapsto I^{(k)}-1 \qquad\text{at rate}\qquad \mu (k -\alpha), \quad\text{ when }\quad I^{(k)}>0.
 \end{align*}
So, given \eqref{Mbound}, we consider the CTMC 
 \begin{align*}
 &\tilde{I}\mapsto \tilde{I}+1 \qquad\text{at rate}\qquad \mu k^{1/2}\\
 &\tilde{I}\mapsto \tilde{I}-1 \qquad\text{at rate}\qquad \mu (k -\alpha), \quad\text{ when }\quad \tilde{I}^{(k)}>0.
 \end{align*}
Thus on event $A^c$, $I^{(k)}$ and $\tilde{I}$ are coupled so that $I^{(k)}(t)\leq \tilde{I}(t)$ for all $t$ such that $0\leq t \leq kT$.

We now bound the area under $(\tilde{I}(t) : 0\leq t \leq kT)$. We know that there are at most Poisson with mean $\mu k^{3/2}T$ excursions of $\tilde{I}(t)$ in time $0$ to $kT$ and, by Lemma \ref{PoissonBound}, we know that
\begin{equation}\label{thisPoissonBound}
{\mathbb P}\left( Po(\mu k^{3/2}T) \geq 9\mu k^{3/2} T \right) \leq e^{-10\mu T k^{3/2}}.
\end{equation}
Applying a union bound to these excursions, we have that 
\begin{equation}\label{yexpress}
{\mathbb P}  \left( \int_0^{kT}  \tilde{I} (t) dt \geq  y \right)
\leq
9\mu T k^{3/2 } {\mathbb P}  \left(  \int_0^{\tilde{T}} \tilde{I} (t)dt \geq \frac{y}{9\mu k^{3/2} T}\right) + e^{-10\mu T k^{3/2}}
\end{equation}
where $\tilde{T}$ is the length of an excursion of $\tilde{I}$.
(I.e. in the above union bound, either there are less that $9\mu k^{3/2}T$ excursions and then for the total area to be over $y$ there must be at least one excursion whose area is above $y/[9\mu k^{3/2} T]$, or, there are more than $9\mu k^{3/2}T$ excursions in which case \eqref{thisPoissonBound} is applied.) 

Now we apply Lemma \ref{ExcusionLemma} with parameter choices $\theta_0=1$, $c=\frac{k}{2}$, $x=k^{2\epsilon -1}$. (Notice $\phi(\theta_0))+ c \theta_0<0$ for all sufficiently large $k$). Thus we have that 
\[
{\mathbb P} \left( \int_0^{\tilde{T}} \tilde{I}(t) dt \geq k^{ 2\epsilon-1}  \right)
\leq
 e^{-\sqrt{\frac{\mu}{2}} (k^{\epsilon}-1)}
\]
Applying this to bound \eqref{yexpress} with $y=9\mu T k^{\frac{1}{2}+2\epsilon}$ gives
\[
{\mathbb P}  \left( \int_0^{kT}  \tilde{I} (t) dt \geq  9\mu T k^{\frac{1}{2}+2\epsilon} \right)
\leq
9\mu k^{3/2 }T   e^{-\sqrt{\frac{\mu}{2}} (k^{\epsilon}-1)} + e^{-10\mu T k^{3/2}}.
\]
Let $B$ be the event in the above probability (right-hand side above). We can now bound the integral of interest
\begin{align*}
{\mathbb P}\left( \int_0^{kT} I^{(k)}(t) {\mathbb I} [ M_{\geq 3}(t) \geq k^{1/2 + \epsilon}]dt \geq k^{1/2+2\epsilon}\right) &\leq {\mathbb P} (A) + {\mathbb P}(B\cap A^c)  \\
&\leq {\mathbb P} (A) + {\mathbb P} (B)\\
& \leq  a_1 k^2 e^{-b_1 k^{\epsilon}} + \left[ 9\mu k^{3/2 }T   e^{-\sqrt{\frac{\mu}{2}} (k^{\epsilon}-1)} + e^{-10\mu T k^{3/2}} \right].
\end{align*} 
From this inequality, it is clear that the required bound holds for suitably chosen parameters $a_2$ and $b_2$.
\hfill \Halmos	\endproof


\subsection{Bounding Queue Sizes}
To apply Lemma \ref{Lem:AMIdentity} and consequently prove Proposition \ref{Thrm:StateSpaceCollapse}, we must analyse $N_{\geq 3}^{(k)}$, the number of jobs queued in $3$rd position or above. 
However thus far in Section \ref{idlesness}, we have only gained bounds on $M^{(k)}_{\geq 3}$ the number of servers with $3$ or more jobs. To relate $M^{(k)}_{\geq 3}$ with $N^{(k)}_{\geq 3}$, we can apply bounds that bound the total queue size in NDS. (Our analysis here is specific  to JSQ. Other bounds might be used here to provide proofs for other dispatch rules.)

In this subsection the main result is the following lemma.

\begin{lemma}\label{lem:Nbound}
\[
{\mathbb P}\left( \max_{0\leq t\leq T} \left\{ \hat{N}^{(k)}(t)-\hat{N}^{(k)}(0) \right\}\geq n+3 \right) \leq a_3 e^{-b_3 \sqrt{n}}
\]
where $a_3$ and $b_3$ are positive constants that do not depend on $k$.
\end{lemma}

To prove this we bound the size of each excursion of the queue size process in Lemma \ref{Lemma8} and then bound the length of these excursions in Lemma \ref{Lemma9}. 

\begin{lemma}\label{Lemma8} 
For all times $s$ with $\hat{M}^{(k)}_{\geq 3}(s) \geq k^{-\frac{1}{2}+\epsilon}$ and $I^{(k)}(ks)=0$, let  $\tau$ be the next time that $\hat{M}^{(k)}_{\geq 3} < k^{-\frac{1}{2}+\epsilon}$ holds, specifically,
	$\tau = \min \left\{ t \wedge T : \hat{M}_{\geq 3}^{(k)}(t)< k^{-\frac{1}{2}+\epsilon} \right\}$. Given $s$ and $\tau$, the following bound holds
	\[
	\max_{s\leq t\leq \tau} \left\{ \hat{N}^{(k)}(t) - \hat{N}^{(k)}(s) \right\}\leq P.
	\]
where $P$ is a random variable such that
	\[
	\mathbb{P}\left(P\geq p+1\right) \leq 4 \exp\left\{-\frac{p^2}{8\mu T}\left( 1-\frac{p}{4\mu k T}\right)\right\}.
	\]
	\end{lemma}


\proof{Proof}
We know from \eqref{NExpression} that for $0\leq s \leq t\leq T$,
\begin{align*}
N^{(k)}(kt)- N^{(k)}(ks) =& {\mathcal N}_a \left( k\mu ( k -\alpha )t) -{\mathcal N}_a ( k\mu ( k -\alpha )s  \right) \\
& + {\mathcal N}_d \left( \int_0^t  \mu(k- I^{(k)}(u) )du \right) - {\mathcal N}_d \left( \int_0^s  \mu(k- I^{(k)}(u) )du \right)
\end{align*}
where $\mathcal{N}_a$ and $\mathcal{N}_d$ are unit Poisson processes. To prove the result we bound the excursions of $\hat{N}^{(k)}(t)$ given the bound on idleness Lemma \ref{2ndIdleBound} (which bounds the integral terms above).

Given $s$ is a time where $M^{(k)}_{\geq 3} (ks) \geq k^{\frac{1}{2} + \epsilon}$ and $I^{(k)}(ks)=0$.
(Note, each time $\max_{0\leq t'\leq t}\hat{N}^{(k)}(t')$ increases above $2+k^{1/2 +\epsilon}$, we must have $I^{(k)}(kt)=0$ and $M^{(k)}_{\geq 3} (ks') \geq k^{\frac{1}{2} + \epsilon}$.) Thus from Lemma \ref{2ndIdleBound} with high probability 
\begin{equation}\label{Intbound}
\int_{ks}^{kt} {I}^{(k)}(s)ds \leq k^{\frac{1}{2}+2\epsilon}
\end{equation}
for any $t$ such that $t\leq \tau$ where $\tau$ is the first time after $s$ such that $M_{\geq 3}^{(k)}(\tau) < k^{\frac{1}{2}+\epsilon}$
holds.
Thus defining $\bar{{\mathcal N}}(t)= {\mathcal N}(t)-t$, from \eqref{Intbound}, we have that 
\begin{align*}
&\hat{N}^{(k)}(t)-\hat{N}^{(k)}(s)\\ 
=& 
\frac{1}{k} 
{\mathcal N}_a \left( k\mu( k -\alpha) t \right) 
-
\frac{1}{k} 
{\mathcal N}_a \left( k\mu( k -\alpha) s \right)\\
&- \frac{1}{k} 
{\mathcal N}_d \left(  \int_0^{kt}  \mu(k- I^{(k)}(u) )du \right) 
+ 
{\mathcal N}_d \left( \int_0^{ks}  \mu(k- I^{(k)}(u) )du \right)
\quad\\
\leq &  
\frac{1}{k} 
{\mathcal N}_a \left( k\mu (k -\alpha) t \right) 
-
\frac{1}{k} 
{\mathcal N}_a \left( k\mu (k -\alpha) s \right)
\\
& 
- \frac{1}{k} 
{\mathcal N}_d \left(  \mu k^2 t -  k^{\frac{1}{2}+2\epsilon}- \mu \int_0^{ks}  I^{(k)}(u) du \right) 
+  
\frac{1}{k} 
{\mathcal N}_d \left(  \mu k^2 s - \mu \int_0^{ks}  I^{(k)}(u) du \right)
\\
=& 
\frac{1}{k} 
\bar{{\mathcal N}}_a \left( k\mu (k -\alpha) t \right) 
-
\frac{1}{k} \bar{{\mathcal N}}_a \left( k\mu (k -\alpha) s \right) - \alpha \mu (t-s)
\\
&- \frac{1}{k} 
\bar{{\mathcal N}}_d 
\left( 
	\mu k^2 t - k^{\frac{1}{2}+2\epsilon}
	- 
	\mu 
	\int_0^{ks}  I^{(k)}(u) du  
\right) 
+  
\frac{1}{k} 
\bar{{\mathcal N}}_d \left( \mu k^2 s - \mu \int_0^{ks}  I^{(k)}(u) du   \right) +k^{-\frac{1}{2}+2\epsilon}.
\end{align*}
We can maximize the left- and right-hand side of the above expression to give that
\begin{align*}
&
\max_{t : s\leq t\leq \tau}\left\{ \hat{N}^{(k)}(t) - \hat{N}^{(k)}(s) \right\}\\
\leq 
&\max_{0\leq s \leq t\leq T}
\Bigg\{  
\frac{1}{k} \bar{{\mathcal N}}_a \left( k\mu (k -\alpha) t \right) 
-\frac{1}{k} \bar{{\mathcal N}}_a \left( k\mu (k -\alpha) s \right) 
- \alpha (t-s)\\
&\qquad\qquad
- \frac{1}{k} \bar{{\mathcal N}}_d \left( \mu k^2 t - k^{\frac{1}{2}+2\epsilon}
- \mu \int_0^{ks}  I^{(k)}(u) du  \right) 
+  \frac{1}{k} \bar{{\mathcal N}}_d \left( \mu k^2 s - \mu \int_0^{ks}  I^{(k)}(u) du   \right) +k^{-\frac{1}{2}+2\epsilon} \Bigg\} \\
\leq & \left[  
\max_{0\leq t \leq T}\frac{1}{k} \bar{{\mathcal N}}_a \left( \mu k^2 t \right) 
- \min_{0\leq s \leq T}\frac{1}{k} \bar{{\mathcal N}}_a \left( \mu k^2 s \right) \right] 
+ \left[\max_{0\leq t \leq T} \frac{1}{k} \bar{{\mathcal N}}_d \left( \mu k^2  t \right) 
- \min_{0\leq s \leq T} \frac{1}{k} \bar{{\mathcal N}}_d \left( \mu k^2  s \right)\right] 
+ k^{-\frac{1}{2}+2\epsilon}=:P.
\end{align*}
So, we define $P$ to be the difference between the maximum and minimum of two Poisson processes. 
We can apply Lemma \ref{PoissonBound} to the 4 maximizations and minimization above. For instance,
\[
\mathbb{P} \left( \max_{0\leq t\leq T} \frac{1}{k}\bar{\mathcal{N}}_a(\mu k^2 t) \geq z \right) = \mathbb{P} \left(  \max_{0\leq t\leq \mu k^2 T} ( {\mathcal{N}}_a( t) - t ) \geq z k \right) \leq \exp\left\{-\frac{z^2}{2\mu T}\left(1-\frac{z}{\mu kT}\right)\right\}.
\]
Further we can assume that $k$ is sufficiently large so that $k^{-\frac{1}{2}+2\epsilon}<1$. Thus 
\[
\mathbb{P}\left(P\geq p+1\right) \leq 4 \exp\left\{-\frac{p^2}{8\mu T}\left( 1-\frac{p}{4\mu k T}\right)\right\}
\]
which gives a bound of the required form.

\hfill \Halmos
\endproof

The following lemma shows that every time there is an excursion away from $\hat{N}^{(k)}(0)=3$ then there is a strictly positive probability that $\hat{N}^{(k)}(t)$ will stay above $5/2$ until time $T$.

\begin{lemma}\label{Lemma9}
	Suppose that $\hat{N}^{(k)}(0)=3$ and $I^{(k)}(ks)=0$, let $\tau^{(k)}$ be the next time  such that $M^{(k)}_{\geq 3}(t)< k^{\frac{1}{2}+\epsilon}$ holds. Then there exists a strictly positive constant $q$ such for all $k$
	\[
	\mathbb{P} ( \tau^{(k)} > T) \geq q.
	\]
	\end{lemma}
\proof{Proof}
%Clearly, 
%\begin{equation}\label{events}
%\{ \tau^{(k)} > T\} =\{M^{(k)}_{\geq 3}(t) >  k^{\frac{1}{2}+\epsilon}, \forall t \leq T\}\supseteq \{ N^{(k)}(t) > \frac{5}{2}, \forall t\leq T \}.
%\end{equation}

%We lower-bound the probability of the event on the right-hand side of \eqref{events}. 
First observe
\begin{align}
\hat{N}^{(k)}(t) =& \hat{N}^{(k)}(0) + \frac{1}{k} {\mathcal N}_a \left( k(\mu k -\alpha) t \right) 
- \frac{1}{k} {\mathcal N}_d \left(  \int_0^{kt}  \mu(k- I^{(k)}(u) )du \right) \notag \\
\geq & 3+ \frac{1}{k} {\mathcal N}_a \left( k\mu( k -\alpha) t \right) 
- \frac{1}{k} {\mathcal N}_d \left(   \mu k^2 t \right) \label{InNHat} \\
=& 3+ \frac{1}{k} \bar{{\mathcal N}}_a \left( k \mu( k -\alpha) t \right) 
- \frac{1}{k} \bar{{\mathcal N}}_d \left(   \mu k^2 t \right) - \alpha \mu t.\notag
\end{align}
By the Martingale Functional Central Limit Theorem \ref{MgCLT} the last term converges to a 
Brownian motion with drift. That is
\[
\left(\frac{1}{k} \bar{{\mathcal N}}_a \left( k \mu ( k -\alpha) t \right) 
- \frac{1}{k} \bar{{\mathcal N}}_d \left(   \mu k^2 t \right) - \alpha \mu t : t\geq 0 \right)\Rightarrow \left(\sqrt{2\mu} B(t) -\alpha \mu  t : t\geq 0\right).
\]
Further, we know that 
\[
\bP \left( 3 + \sqrt{2\mu} B(t) -\alpha \mu t > \frac{5}{2}, \forall t \leq T \right) \geq 2q
\]
for some positive constant $q$. The above set is an open set with respect to the Skorohod topology on $[0,T]$. Thus by the Portmanteau Theorem applied to open sets (see \cite{billingsley2013convergence}): for all sufficiently large $k$
\begin{equation}\label{ProbHitBound}
\mathbb{P}\left(3+\frac{1}{k} \bar{{\mathcal N}}_a \left( k \mu (k -\alpha) t \right) 
- \frac{1}{k} \bar{{\mathcal N}}_d \left(   \mu k^2 t \right) - \alpha \mu t > 2\frac{1}{2} , \forall t\geq T \right) \geq q.
\end{equation}
Combining \eqref{InNHat} and \eqref{ProbHitBound} gives the required bound
\[
\mathbb{P}\left(\tau^{(k)} > T\right) = \mathbb{P}\Big( \hat{N}^{(k)}(t) > \frac{5}{2}, \forall t\leq T \Big)\geq q.  
\]
\hfill\Halmos
\endproof
We use the last lemma to obtain a bound on the maximum queue size under the JSQ policy.


\proof{Proof of Lemma \ref{lem:Nbound}} %We focus on the $k$th system and suppress the superscript on $k$ to ease notation.

	Let $\sigma_0$ be the first time that $\hat{N}^{(k)}(t)=\lceil \hat{N}^{(k)}(0) \rceil + 3$.
	Let $\hat{\tau}_i$ be the first time after $\sigma_i$ that $\hat{N}^{(k)}(t)=1.5$
	and let $\sigma_i$ be the first time after $\hat{\tau}_{i-1}$ that $\hat{N}(t) = 3$. Applying Lemma \ref{lem:VBound} note that  $M_{\geq 3}^{(k)}(t)<k^{\frac{1}{2}+\epsilon}$ must have occurred. So given Lemma \ref{Lemma9}, $\hat{\tau}_0-\sigma_0 > \tau^{(k)}$.
	
	By Lemma \ref{Lemma9}, 
	\begin{equation*}
		\bP (\tau_i - \sigma_i \geq T) \geq q>0
	\end{equation*}
	and by Lemma \ref{Lemma9}
	\begin{equation*}
  \bP \left( \max_{\sigma_i \leq t \leq \tau_i} \hat{N}^{(k)}(t) \geq p+3 \right) 
  \leq 
	\bP \left( P \geq p +3 \right)
\end{equation*}
where $P$ is as specified in Lemma \ref{Lemma9}.

So
\begin{equation*}
  \max_{0\leq t \leq T} \hat{N}^{(k)}(t) 
  \leq
  \sum_{i=1}^{G(q)} P_i + \lceil \hat{N}^{(k)}(0) \rceil + 3
\end{equation*}
where $G(q)$ is geometrically distributed with parameter $q$ and $P_i$ is an independent random variable with distribution $P$. So applying a union bound
\begin{align*}
  \bP \left( \sum_{i=1}^{G(q)} P_i \geq n \right) 
  &
  \leq 
  \bP \left( G(q) \geq \sqrt{n} \right)
  +
  \bP \left( \sum_{i=1}^{\sqrt{n}} P_i \geq  n \right)
 	\\ &
   \leq 
    \bP \left( G(q) \geq \sqrt{n} \right)
  +
  \sqrt{n}\bP \left( P \geq  \sqrt{n} \right) \leq a_3 e^{-b_3 \sqrt{n}}
\end{align*}
where the final inequality holds for appropriate positive constants $a_3$ and $b_3$.
\hfill \Halmos


\endproof

\subsection{Proof of Proposition \ref{Thrm:StateSpaceCollapse}}

With Lemma \ref{Lem:AMIdentity},  Lemma \ref{lem:VBound}, and Lemma \ref{lem:Nbound},  we can now prove Proposition \ref{Thrm:StateSpaceCollapse}.
In essence Lemma \ref{lem:VBound} and Lemma \ref{lem:Nbound}, combine to say that we cannot have both $\hat{M}_1^{(k)}$ and $N^{(k)}_{\geq 3}$ large at the same time. This bounds the error in identity Lemma \ref{Lem:AMIdentity} and thus shows that $(2-\hat{N}^{(k)}(t))_+$ and  $\hat{M}^{(k)}_1(t)$ must be close.


\proof{Proof of Proposition \ref{Thrm:StateSpaceCollapse}}
Suppose that the following three events all hold:
\begin{subequations}
	\begin{align}
A 
&= 
\Big\{ I^{(k)}(t) \leq k^{\frac{1}{2}+\epsilon},\, \forall t\leq kT \Big\}\label{eq:Acond}
\\
B 
&= 
\Big\{ 
	(2\Ik (t) + \Mk_1(t) )   
	\leq 
	k^{\frac{1}{2}}, 
	\forall t \leq kT\text{ such that }M^{(k)}_{\geq 3}(t) \geq k^{\frac{1}{2}+\epsilon} \Big\}\label{eq:Bcond}
\\
C
&= 
\Big\{\max_{0\leq s\leq T}  \hat{N}^{(k)}(s) \leq k^{\epsilon}\Big\}
\end{align} 
\end{subequations}
%
%
Applying a union bound, we know by Proposition \ref{lem:IdleBound},  Lemma \ref{lem:VBound}, and Lemma \ref{lem:Nbound} that 
\[
\bP( A \cap B \cap C ) \geq 1- a \exp\{-b k^{\frac{\epsilon}{2}}\}
\]
where $a$ and $b$ are constants depending on $\mu$, $\alpha$ and $T$.

From Lemma \ref{Lem:AMIdentity}, we have the identity:
\begin{equation}\label{eq:NMIndentity}
\big(2-\hat{N}^{(k)}(t)\big)_+ - \hat{M}^{(k)}_1(t) = \left(\hat{M}_1^{(k)}(t) + 2\frac{I^{(k)}(kt)}{k} - \frac{N^{(k)}_{\geq 3}(kt)}{k}\right)_+\!\! - \hat{M}_1^{(k)}(t).
\end{equation}
%
We analyze this equality under two separate conditions: 1. $N^{(k)}_{\geq 3}(kt) \leq k^{1/2+2\epsilon}$ and 2. $N^{(k)}_{\geq 3}(kt) \geq k^{1/2+2\epsilon}$.

First, we assume the condition $N^{(k)}_{\geq 3}(kt) \leq k^{1/2+2\epsilon}$ is met. We note the following elementary bound: for $x>0$,
\begin{equation*}
  |(x+y)_+ - x| = | -(x+y)_- +y | \leq (x + y)_- + |y| \leq 2|y|. 
\end{equation*}
Applying this bound to Identity \eqref{eq:NMIndentity} gives that
\[
\big| \big(2-\hat{N}^{(k)}(t)\big)_+ - \hat{M}^{(k)}_1(t) \big|
\leq 
2\Bigg|2\frac{I^{(k)}(kt)}{k} - \frac{N^{(k)}_{\geq 3}(kt)}{k}\Bigg| 
\leq 
4 k^{-\frac{1}{2}+\epsilon}
\] 
in the final inequality, above, we apply our condition, $N^{(k)}_{\geq 3} (kt) \leq k^{1/2+2\epsilon}$,  and our assumption that Event $A$ holds. 
So for the first case the required bound holds.

Second, assume that the condition ${N}^{(k)}_{\geq 3} (kt) \geq k^{1/2+2\epsilon}$ is met. We know that $1 + \max_{0\leq s\leq T}  \hat{N}^{(k)}(s)$ gives the maximum queue size achieved at any server. Thus,
\begin{equation*}
   {M}_{\geq 3}(kt) \times \max_{0\leq s\leq T}  \hat{N}^{(k)}(s)
   \geq 
    {N}_{\geq 3}^{(k)}(kt).
\end{equation*}
Thus, since Event C holds, we have that 
\begin{equation*}
  {M}_{\geq 3}(kt)
  \geq 
  \frac{
  		{N}^{(k)}_{\geq 3}(kt)
  		}{
  		\max_{s\leq T} \hat{N}^{(k)}(s)
  		}
  \geq  
  \frac{
  		k^{1/2+2\epsilon}
  		}{
  		k^{\epsilon}
  		}
  	=
  	k^{1/2+\epsilon}.
\end{equation*}
By this bound and since Event $B$ holds, we have 
\begin{equation*}
  (2\Ik (kt) + \Mk_1(kt) )   
	\leq 
	k^{\frac{1}{2}}.
\end{equation*}
Now applying this to Identity \eqref{eq:NMIndentity} gives
\begin{equation*}\label{eq:NMIndentity}
\Big|\big(2-\hat{N}^{(k)}(t)\big)_+ - \hat{M}^{(k)}_1(t) \Big| 
	\leq 
	\left(
		\frac{{M}_1^{(k)}(kt)}{k} 
		+ 
		2\frac{I^{(k)}(kt)}{k}
	\right)_+
		\!\! 
		+ 
		\frac{{M}_1^{(k)}(kt)}{k} \leq 2 k^{-1/2}.
\end{equation*}
as required.\hfill\halmos
\endproof


\section{Timescale Separation}

The main aim of this section is to prove Proposition \ref{TimescaleIdleness} as stated below. This addresses the convergence of term \eqref{NTermsb} as discussed in the outline of proof of Theorem \ref{JSQ:Thrm} in Section \ref{sec:outline}.

From Proposition \ref{Thrm:StateSpaceCollapse} we now see that $\big(2-\hat{N}^{(k)}(t)\big)_+$ provides a good estimate for $\hat{M}^{(k)}_1(t)$, the proportion of queues of length $1$. We present a slightly refined version of this result in Section \ref{subsec:Tight}. This then dictates the transitions of the idleness process which we analyse and bound in Section \ref{BoundingI}. After this we are in a position to prove Proposition \ref{TimescaleIdleness}.  

Our proof is slightly complicated by the necessity to provide a localizing sequence for our weak convergence result. Throughout this section we let $\tau^{(k)}(\eta)$ be the first time before time $T$ such that $\hat{N}^{(k)}(t)\leq 1+\eta$ holds. That is
\begin{equation*}
  \tau^{(k)}(\eta) = \min\{ t \leq T : \hat{N}^{(k)}(t)\leq 1+\eta  \} \wedge T
\end{equation*}

We analyze the number of idle servers, $\hat{I}^{(k)}$, over excursions from zero.
Let $T^{(k)}_m$ be the sequence of times, less than $k^2 \tau^{(k)}(\eta)$ where $\hat{I}^{(k)}$ hits zero. Specifically, $T_0^{(k)}=0$ and, for $m\in\mathbb{N}$,
\[
T^{(k)}_m 
= 
\inf\big\{ 
t\geq X_{m-1}^{(k)} 
: 
\hat{I}^{(k)}(t)=0 
\big\}
\wedge
\big\{ k^2 \tau^{(k)}(\eta) \big\}.
\]
In the above, expression $X_{m-1}^{(k)} $ is the next time after time $T_{m-1}^{(k)} $  where $\hat{I}^{(k)}(t)>0$ holds. 

As discussed above, we wish to prove the following Proposition. 

\begin{proposition} \label{TimescaleIdleness}
\[
	\sup_{0\leq t\leq \tau^{(k)}(\eta)} 
		\left| 
			\frac{1}{k^2} 
				\int_{0}^{k^2t}	\hat{I}^{(k)}(s)ds 
			- 
				\int_{0}^{t}	
					\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}
				ds 
			\right| 
	\xrightarrow[k\rightarrow \infty]{} 
	0
\]
where the above convergence is convergence in probability.
\end{proposition}




\subsection{Tightness bound}\label{subsec:Tight}
We wish to show that $\hat{I}^{(k)}$  behaves approximately as an M/M/1 queue. 
 We know that the $\hat{I}^{(k)}$ observes transition rates
 \begin{align*}
 &\hat{I}^{(k)}\mapsto \hat{I}^{(k)}+1 \qquad\text{at rate}\qquad \mu \hat{M}_1^{(k)}(t),\\
 &\hat{I}^{(k)}\mapsto (\hat{I}^{(k)}-1)_+ \quad\text{at rate}\qquad \mu \left( 1 -\frac{\alpha}{k} \right).
 \end{align*}
By Proposition \ref{Thrm:StateSpaceCollapse}, $\hat{M}_1^{(k)}(t)$ is well approximated by $\big(2-\hat{N}^{(k)}(t)\big)_+$. In this subsection, to show that these terms are approximately constant over excursions of $\hat{I}^{(k)}$. Thus, in the next subsection, we discuss how $\hat{I}^{(k)}$ behaves approximately as an M/M/1 queue.

We prove the following proposition, which is the main result in this subsection. It shows that $\hat{N}^{(k)}$ cannot oscillate greatly between excursions of $\hat{I}^{(k)}$.

\begin{proposition}\label{TightProp}
\[
	\mathbb{P} 
		\left( 
			\sup_{m\in\mathbb{Z}_+} 
			\sup_{T^{(k)}_m < t \leq T^{(k)}_{m+1}  } \left| 
					\hat{M}_1^{(k)}
						\left(\frac{t}{k^2} \right)
					-
					\left( 
							2
							-
							\hat{N}^{(k)}\left(\frac{T^{(k)}_m}{k^2} \right) 
					 \right)_+
				 \right| 
			\geq 
			2 k^{-1+\epsilon}   
		\right) 
	\leq 
	\gamma e^{-\beta k^{\epsilon/2}}.
\]
\end{proposition}
To prove this proposition, we require two lemmas. The first, Lemma \ref{lem:NhatBound}, shows that $\hat{N}$ does not vary greatly on the fast, $O(k^2)$, time scale -- which is the timescale at which the idle server process evolves. The second, Lemma \ref{lem:NhatBound3} shows that there are no long excursion of the Idle server process; that is, of order greater that $O(k^{\epsilon/2})$.


In the following two lemmas and the proof of Proposition \ref{TightProp}, we let 
\[
\delta^{(k)} = k^{-1+\epsilon} \qquad \text{and}\qquad S^{(k)} = k^{\epsilon/2}.
\]

\begin{lemma}\label{lem:NhatBound} For positive constants $\gamma_1$ and $\beta_1$,
\begin{equation*}\label{NhatBound}
	\mathbb{P}
	\left(
		\sup_{m\in\mathbb{Z}_+} 
		\sup_{T_m^{(k)}\leq t \leq T_m^{(k)}+S^{(k)}} 
		\left|
			\hat{N}^{(k)}\left(\frac{t}{k^2}\right) - \hat{N}^{(k)} \left(\frac{T_m^{(k)}}{k^2}\right)
		\right|
		\geq 
		{\delta^{(k)}}  
	\right)
	\leq 
 \gamma_1 e^{-\beta_1 k^{\epsilon/2}}.
\end{equation*}	
\end{lemma}

\proof{Proof.}
Let $ 0= J_0^{(k)}< J_1^{(k)} < J_2^{(k)}  <... $ be the jump times of the process $(\hat{N}^{(k)}(t/k^2) : 0\leq t \leq k^2 \tau^{(k)}(\eta))$. Since each time $T_m^{(k)}$ is initiated by a jump time, it suffices to prove the result for jump times $J^{(k)}_m$. 

We prove the lemma in three steps. First, we prove a similar bound to \eqref{NhatBound} but for a single jump. Second, we prove that the number of jumps is of order $O(k^2)$. Third, we combine the two bounds using a union bound to give the result.

First, let $J^{(k)}=J_m^{(k)}$ be a jump of our process. Similar to expression \eqref{NExpression}, there exist independent unit rate Poisson Processes $\mathcal{N}_a$ and $\mathcal{N}_d$ (representing arrival and departure processes) such that, for $t\geq 0$
\begin{align}\label{NPois}
\hat{N}^{(k)}\left(\frac{t+J^{(k)}}{k^2}\right)- \hat{N}^{(k)}\left( \frac{J^{(k)}}{k^2} \right) =&  \frac{1}{k}{\mathcal N}_a \left( \left(1  -\frac{\alpha}{k} \right)\mu t\right)   - \frac{1}{k}{\mathcal N}_d \left( \mu t - \frac{\mu }{k^3} \int_0^\frac{t}{k^2}  \hat{I}^{(k)}(s)ds \right).
\end{align}
Thus, for $0\leq t\leq S^{(k)}$
\begin{equation}\label{OscB}
\sup_{0\leq t \leq S^{(k)}}\left|\hat{N}^{(k)}\left(\frac{t+J^{(k)}}{k^2}\right)- \hat{N}^{(k)}\left( \frac{J^{(k)}}{k^2} \right)\right| \leq  \sup_{0\leq t \leq S^{(k)}} \left[ \frac{1}{k} \left[\mathcal{N}_a (\mu t ) + \mathcal{N}_d (\mu t ) \right] \right] \leq \frac{1}{k} \left[\mathcal{N}_a (\mu 
S^{(k)} ) + \mathcal{N}_d (\mu S^{(k)} ) \right].
\end{equation}
Since $k\delta^{(k)} \geq e^2 2\mu S^{(k)}$ for all suitably large $k$, we can apply Lemma \ref{PoissonBound} to give that
\begin{equation}\label{Po2}
\mathbb{P} \left(\frac{1}{k} \left[\mathcal{N}_a (\mu 
S^{(k)} ) + \mathcal{N}_d (\mu S^{(k)} ) \right] \geq \delta^{(k)}  \right) \leq e^{- 2 \mu S^{(k)}-\delta^{(k)} k }.
\end{equation}
Inequalities \eqref{Po2} and \eqref{OscB} give the bound
\begin{equation}\label{NhatBound2}
\mathbb{P}\left(\sup_{J^{(k)}\leq t \leq J^{(k)}+S^{(k)}} \left|\hat{N}^{(k)}\left(\frac{t}{k^2}\right) - \hat{N}^{(k)} \left(\frac{J^{(k)}}{k^2}\right)\right| \geq {\delta^{(k)}}  \right)\leq e^{-2\mu S^{(k)} -{\delta^{(k)}} k}.
\end{equation}	

Second, we count the number of jumps that can occur in the time interval $[0,k^2 T]$. Again, since $(\hat{N}^{(k)}(t/k^2) : t\geq 0)$ has arrivals and departures that occur as a Poisson process of rate less than $2\mu$ (c.f. \eqref{NPois}), we have that from Lemma \ref{PoissonBound} that
\[
\mathbb{P}( |m : J^{(k)}_m\leq k^2T | \geq 2e^2\mu k^2 T  ) \leq \mathbb{P}\left( Po(2\mu k^2 T) \geq 2e^2\mu k^2 T \right) \leq e^{- (1+e^2) 2\mu k^2 T}.
\]

Third, we condition on whether the event $\{ |m : J^{(k)}_m\leq k^2T | \geq 2e^2\mu k^2 T\}$ occurs or not. When we condition on the event holding we apply  the above inequality, and when the event does not hold we apply a union bound to the finite number of transitions holding:
\begin{align*}
&\mathbb{P}\left(\sup_{m : J^{(k)}_m\leq k^2T} \sup_{0\leq t \leq S^{(k)}} \left|\hat{N}^{(k)}\left(\frac{t+J_m^{(k)}}{k^2}\right) - \hat{N}^{(k)} \left(\frac{J_m^{(k)}}{k^2}\right)\right| \geq {\delta^{(k)}}  \right)\\
\leq & e^{- (1+e^2) 2\mu k^2 T} + 2e^2 \mu k^2 T \sup_{m \leq 2e^2 \mu k^2 T}  	\mathbb{P}\left(\sup_{0\leq t \leq S^{(k)}} \left|\hat{N}^{(k)}\left(\frac{t+J_m^{(k)}}{k^2}\right) - \hat{N}^{(k)} \left(\frac{J_m^{(k)}}{k^2}\right)\right| \geq {\delta^{(k)}}  \right)\\
\leq & e^{- (1+e^2) 2\mu k^2 T} + 2e^2 \mu k^2 T e^{-2\mu S^{(k)} -{\delta^{(k)}} k}\\
\leq & \gamma_1 e^{-\beta_1 k^{\epsilon/2}}
\end{align*}
where the last inequality holds for appropriate constants $\gamma_1$, $\beta_1$.
This gives the required inequality.
\hfill \halmos\endproof 

Next, in the following lemma, we show that there are no long excursions of $\hat{I}^{(k)}$.

\begin{lemma} \label{lem:NhatBound3}
	\[
	\mathbb{P} 
		\left( 
			\exists m 
			\text{ s.t. } 
				T^{(k)}_{m+1} 
				- 
				T^{(k)}_{m}
				\geq 
				S^{(k)} 
		\right) 
	\leq  
	 \gamma_2 e^{-\beta_2 k^{\epsilon/2}}
	\]
\end{lemma}



\proof{Proof}
Our State Space Collapse Proposition, Proposition \ref{Thrm:StateSpaceCollapse}, states that
\[
\bP\Big( 
	\sup_{0\leq t\leq T} 
		\Big|
			\big(2-\hat{N}^{(k)}(t)\big)_+ 
			- 
			\hat{M}^{(k)}_1(t) 
		\Big| 
	\leq 
	k^{-1/2+\epsilon}
	\Big) 
\geq 
1-  
a \exp \left\{-bk^{\frac{\epsilon}{2}}\right\}.
\]
On the above event, the following sequence of bounds hold for times $t\leq \tau(\eta)$:
\[
\hat{M}_1^{(k)} (t)
\leq 
(2-\hat{N}^{(k)})_+
+
k^{-\frac{1}{2}+\epsilon}
\leq 
1-\eta
+
k^{-\frac{1}{2}+\epsilon}
\leq 
1- \frac{\eta}{2},
\]
where in the final inequality we assume that $k$ is sufficiently large  that $k^{-\frac{1}{2}+\epsilon} \leq \frac{\eta}{2}$. Thus we have that that
\[
\mathbb{P} 
	\left( 
		\hat{M}^{(k)}_1 (t) 
		\leq 
		1-\frac{\eta}{2},
		\quad \forall t \leq \tau^{(k)}(\eta) 
	\right) 
\geq 
1
-
a 
	\exp 
		\left\{
			-bk^{\frac{\epsilon}{2}}
		\right\}.
\]

Thus since 
 \begin{align*}
 &\hat{I}^{(k)}\mapsto \hat{I}^{(k)}+1 \qquad\text{at rate}\qquad \mu \hat{M}_1^{(k)},\\
 &\hat{I}^{(k)}\mapsto \hat{I}^{(k)}-1 \qquad\text{at rate}\qquad \mu \left( 1 -\frac{\alpha}{k}\right), \quad\text{ when }\quad \hat{I}^{(k)}>0,
 \end{align*}
the above inequality show that, with probability greater that $1-a\exp\left\{-bk^{\frac{\epsilon}{2}}\right\}$, we can bound all excursions of $\hat{I}^{(k)} (t)$ above by an $M/M/1$ queue with arrival rate $\mu (1 - \eta /2)$ and departure rate $\mu\left( 1- \frac{\alpha}{k}\right)$. By Lemma \ref{ExcusionLemma}, $\tilde{T}$, the length of an excursion for this $M/M/1$ queue can be bounded by
	\begin{equation}\label{TtildeBound}
	{\mathbb P} (\tilde{T} \geq S^{(k)} ) 
	\leq 
	\sqrt{\tfrac{1- \frac{\alpha}{k}}{ (1 - \eta /2)}}
	e^{
		-(\sqrt{\mu- \frac{\alpha \mu }{k}}- \sqrt{\mu (1 - \eta /2)})^2 
		S^{(k)}	
		}
	 \leq  \tfrac{1}{ \sqrt{(1 - \eta /2)}}e^{-\mu \frac{\eta^2}{16} S^{(k)}}
	\end{equation}
In the second inequality, above, we apply the bound that $1- \sqrt{1-x} \geq x/2$ for $x\geq 0$ as follows:
\[
(\sqrt{\mu- {\alpha \mu }/{k}}- \sqrt{\mu (1 - \eta /2)})^2 
\geq 
(\sqrt{\mu}- \sqrt{\mu (1 - \eta /2)})^2 = \mu ( 1 - \sqrt{1-{\eta}/2} )^{2}\geq \mu \frac{\eta^2}{16}.
\]

Each excursion of $\hat{I}^{(k)}$ is initiated by a departure and the number of departures is bounded above by a Poisson random variable of parameter $\mu k^2 T$. We know that the probability that this random viable exceeds $e^2 \mu k^2 T$ can be bounded as in Lemma \ref{PoissonBound} that is
\[
\mathbb{P} 
	\left( 
		|m : T^{(k)}_m\leq \tau(\eta) | 
		\geq e^2\mu k^2 T
	\right)
\leq
e^{- (1+e^2) \mu k^2 T} 
\]
and the thus applying \eqref{TtildeBound} and a union bound when $e^2 \mu k^2 T$ excursions occur gives the bound
	\begin{align*}
	&
	\mathbb{P} 
		\left( 
			\exists m 
			\text{ such that } 
			T^{(k)}_{m+1} - T^{(k)}_{m} \geq S^{(k)}  
		\right) 
	\\
	&
	\leq 
	\mathbb{P} 
	\left( 
	|m : T^{(k)}_m\leq \tau(\eta) | 
	\geq e^2\mu k^2 T
	\right)
	+
	e^2\mu k^2 T
		{\mathbb P} (\tilde{T} \geq S^{(k)} ) 
	\\
	&
	\leq
	e^{- (1+e^2) \mu k^2 T}  	
	+
	\tfrac{e^2 \mu k^2 T}{ \sqrt{(1 - \eta /2)}}
		e^{-\mu \frac{\eta^2}{4} S^{(k)}} 
	\end{align*}
	which is a bound of the required form.
\hfill \halmos
\endproof

We now combine Lemmas \ref{lem:NhatBound} and \ref{lem:NhatBound3} to prove Proposition \ref{TightProp}.

\proof{Proof of Proposition \ref{TightProp}.}
Applying a union bound to Lemma \ref{lem:NhatBound} and Lemma \ref{lem:NhatBound3} gives
	\begin{align*}
	&
	\mathbb{P}
		\left(
			\sup_{m\in\mathbb{Z}_+} 
			\sup_{T^{(k)}_{m}\leq t \leq T^{(k)}_{m+1}} 
			\left|
				\hat{N}^{(k)}\left(\frac{t+T^{(k)}_{m}}{k^2}\right) 
				- 
				\hat{N}^{(k)} \left(\frac{T^{(k)}_{m}}{k^2}\right)
			\right|
		 \geq {\delta^{(k)}}  
		 \right)\\
	\leq &
	\mathbb{P}
	\left(
	\sup_{m\in\mathbb{Z}_+} 
	\sup_{T_m^{(k)}\leq t \leq T_m^{(k)}+S^{(k)}} 
	\left|
	\hat{N}^{(k)}\left(\frac{t}{k^2}\right) - \hat{N}^{(k)} \left(\frac{J_m^{(k)}}{k^2}\right)
	\right|
	\geq 
	{\delta^{(k)}}  
	\right)
	+
		\mathbb{P} 
		\left( 
		\exists m 
		\text{ s.t. } 
		T^{(k)}_{m+1} 
		- 
		T^{(k)}_{m}
		\geq 
		S^{(k)} 
		\right) 
	\\
	\leq & \alpha_1 e^{-\beta_1 k^{\epsilon/2}} + \alpha_2 e^{-\beta_2 k^{\epsilon/2}}.
	\end{align*}	
By Lipschitz continuity of  the function $\hat{N}\mapsto (2-\hat{N})_+$, the same bound holds with $(2-\hat{N})_+$ in place of $\hat{N}$, namely,
	\begin{align*}
	&\mathbb{P}
		\left(
			\sup_{m \in \mathbb{Z}_+} 
			\sup_{T^{(k)}_{m}\leq t \leq T^{(k)}_{m+1}}
				\left|
					\left(2- \hat{N}^{(k)}\left(\frac{t+T^{(k)}_{m}}{k^2}\right) \right)_+ 
					- 
					\left(2-  \hat{N}^{(k)} \left(\frac{T^{(k)}_{m}}{k^2}\right) \right)_+
				\right| 
		\geq {\delta^{(k)}} 
		\right)\\
	\leq & \alpha_1 e^{-\beta_1 k^{\epsilon/2}} + \alpha_2 e^{-\beta_2 k^{\epsilon/2}} .
	\end{align*}	
	Finally applying a union bound along with state space collapse, Proposition \ref{Thrm:StateSpaceCollapse}, we have that 
		\begin{align*}
		&\mathbb{P}
			\left(
				\sup_{m \in \mathbb{Z}_+} 
				\sup_{T^{(k)}_{m}\leq t \leq T^{(k)}_{m+1}} 				
					\left|
						\hat{M}^{(k)}_1\left(\frac{t+T^{(k)}_{m}}{k^2}\right)  
						- 
						\left(
							2
							-  
							\hat{N}^{(k)} \left(\frac{T^{(k)}_{m}}{k^2}\right) 
						\right)_+
					\right| 
				\geq {\delta^{(k)}} + k^{-1/2+\epsilon} 
			\right)\\
		\leq & \alpha_1 e^{-\beta_1 k^{\epsilon/2}} + \alpha_2 e^{-\beta_2 k^{\epsilon/2}} + a e^{-b k^{\epsilon/2}} \\
		\leq &  \gamma e^{-\beta k^{\epsilon/2}}
		\end{align*}	
for appropriate positive constants $\gamma $ and $\beta$. \hfill\halmos
\endproof 

We can now see that the idleness process, $\hat{I}^{(k)} $, behaves approximately as an M/M/1 queue over each excursion. Thus in what follows we will mostly focus on behaviour of $\hat{I}^{(k)}$ on time intervals $[T_{m-1}^{(k)},T_{m}^{(k)}]$. Considering the statement of Proposition \ref{TimescaleIdleness}, the following Lemma shows that there is a not a great deal of error introduced by effectively rounding down to the nearest excursion time $T_m$.

\begin{lemma}\label{LemTm}
	\begin{equation*}
		\sup_{m} \sup_{T^{(k)}_m \leq t \leq T^{(k)}_{m+1} }
		\left|
		\frac{1}{k^2} 
			\int_{T^{(k)}_m}^{k^2t} \hat{I}^{(k)} (s) ds
			-
			\int_{T^{(k)}_m/k^2}^{t}	
					\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}
				ds 
		\right|
			\xrightarrow[k\rightarrow\infty]{} 0
\end{equation*}
where the above convergence is convergence in probability.
\end{lemma}
\proof{Proof}
By Lemma \ref{lem:NhatBound3}
	\[
	\mathbb{P} 
		\left( 
			\exists m 
			\text{ s.t. } 
				T^{(k)}_{m+1} 
				- 
				T^{(k)}_{m}
				\geq 
				k^{\epsilon/2}
		\right) 
	\leq  
	 \gamma_2 e^{-\beta_2 k^{\epsilon/2}}
	\]	
and by Lemma \ref{lem:IdleBound}i)	For $\epsilon>0$,
	\[
	\bP \left( \sup_{0\leq t\leq kT} \Ik(t) \geq k^{\frac{1}{2}+\epsilon} \right) \leq a k^2 e^{-b k^{\epsilon}} 
	\]
Further, by assumption
\begin{equation*}
	\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}\leq \frac{2}{\eta}
\end{equation*}
for $s\leq \tau(\eta)$. 

The three bounds above show that with high probability
\begin{align*}
\sup_{m} \sup_{T^{(k)}_m \leq t \leq T^{(k)}_{m+1} }
	\left|
		\frac{1}{k^2} 
			\int_{T^{(k)}_m}^{k^2t} \hat{I}^{(k)} (s) ds
			-
			\int_{T^{(k)}_m/k^2}^{t}	
					\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}
				ds 
	\right|
\leq 
	{k^{-3/2+3\epsilon/2}} 
+ 
	\frac{2}{\eta}
	{k^{-2+\epsilon/2}}
\end{align*}
as required.
	\hfill\Halmos
\endproof

\subsection{Bounding Processes}\label{BoundingI}
 Proposition \ref{TightProp} says that $\hat{M}_1^{(k)}$, which dictates the arrival of idle servers, can be approximated by $(2-\hat{N}(T_m^{(k)}/k^2))_+ \pm 2 k^{-1/2+\epsilon}$  where here $T_{m}^{(k)}$ is the value of the last excursion of $\hat{I}^{(k)}$.  
So we now have that $\hat{I}^{(k)}(t)$, for times $t\in [T_m^{(k)},T_{m+1}^{(k)})$ observes transition rates
 \begin{align*}
 &\hat{I}^{(k)}\mapsto \hat{I}^{(k)}+1 \qquad\text{at rate}\qquad \mu (2-\hat{N}(T_m^{(k)}/k^2))_+ +o(1),\\
 &\hat{I}^{(k)}\mapsto (\hat{I}^{(k)}-1)_+ \quad\text{at rate}\qquad \mu \left( 1 -\frac{\alpha}{k} \right).
 \end{align*}


Thus, as we will now prove, $(\hat{I}^{(k)}(t) : t \in [T_m^{(k)},T_{m+1}^{(k)}])$, can be bounded by processes ${I}_+^{(k)}$ and ${I}_-^{(k)}$. Here, for $t\in [T_m^{(k)},T_{m+1}^{(k)}]$, we define  ${I}_+^{(k)}(t)$ and ${I}_-^{(k)}(t)$ to be the continuous time Markov chain with ${I}_\pm^{(k)}(T_m^{(k)})=0$ and with non-zero transition rates
 \begin{align*}
 &{I}^{(k)}_{\pm}\mapsto {I}^{(k)}_{\pm}+1 
	 \qquad\text{at rate}
	\qquad \lambda^{(k)}_{m,\pm},\\
 &{I}^{(k)}_{\pm}\mapsto ({I}^{(k)}_{\pm}-1)_+ 
	 \quad\text{at rate}\qquad 
	 \mu^{(k)}_{m,\pm}.
 \end{align*}
For the $m$th idleness excursion, that is for times $T^{(k)}_m\leq t < T^{(k)}_{m+1}$, we can define the rates
\begin{align}\label{Lambdaplus}
\lambda^{(k)}_{m,+}& := \mu (2-\hat{N}^{(k)}(T^{(k)}_m))_++ 2\mu k^{-1/2+\epsilon}, \qquad \mu^{(k)}_{m,+} := \mu - \frac{\alpha}{k},\\
\lambda^{(k)}_{m,-} & := \mu (2-\hat{N}^{(k)}(T^{(k)}_m))_+ - 2\mu k^{-1/2+\epsilon}, \qquad \mu^{(k)}_{m,-} := \mu .
\end{align}
Note that both ${I}_+^{(k)}$ and ${I}_-^{(k)}$ are M/M/1 queues on time intervals $[T_m^{(k)},T_{m+1}^{(k)}]$.
	
The following lemma shows that $I^{(k)}_+$ and $I^{(k)}_-$ bound $\hat{I}^{(k)}$  above and below.
\begin{lemma}\label{IdleCoupling}
The processes $I^{(k)}_+$ and $I^{(k)}_-$ may be chosen so that
	\[
	\mathbb{P} \left( I^{(k)}_-(t) \leq \hat{I}^{(k)}(t) \leq I_+^{(k)}(t), \forall t\leq \tau^{(k)}(\eta) \right) \geq 1 -\gamma e^{-\beta k^{\epsilon/2}}
	\]
	 where $\gamma$ and $\beta$ are positive constants (as given in Proposition \ref{TightProp}).
\end{lemma}
\proof{Proof}
For each excursion $T^{(k)}_m\leq t < T^{(k)}_{m+1}$, we can write $\hat{I}$ in the form 
\[
\hat{I}^{(k)}(t) = {\mathcal N}_{m,d}\left( \mu \int_{T^{(k)}_m}^t \hat{M}^{(k)}_1(u) du\right)
-
\mathcal{N}_{m,a}\left( \int_{T^{(k)}_m}^t  \mu \Big( 1 -\frac{\alpha}{k} \Big)  ds \right)
\]
where ${\mathcal N}_{m,d}$, $\mathcal{N}_{m,a}$ are independent Poisson processes. By Proposition \ref{TightProp} with probability greater that $1 -\gamma e^{-\beta k^{\epsilon/2}}$, we have that
\[
 \int_{T^{(k)}_m}^t  \lambda_-^{(k)}(s)ds \leq \mu \int_{T^{(k)}_m}^t \hat{M}^{(k)}_1(u) du \leq  \int_{T^{(k)}_m}^t  \lambda_+^{(k)}(s)ds
\]
Thus 
\begin{align*}
I^{(k)}_-(t) = & {\mathcal N}_{m,d}\left( \mu \int_{T^{(k)}_m}^t  \lambda_-^{(k)}(s)ds \right)
 -
 \mathcal{N}_{m,a}\left(  \int_{T^{(k)}_m}^t  \lambda_+^{(k)}(s)ds \right)
\\
\leq & 
\hat{I}^{(k)}(t) 
\\
\leq &
 {\mathcal N}_{m,d}\left( \mu \int_{T^{(k)}_m}^t  \lambda_+^{(k)}(s)ds \right)
-
\mathcal{N}_{m,a}\left(  \int_{T^{(k)}_m}^t  \mu_+^{(k)}(s)ds \right)
=I^{(k)}_+(t)
\end{align*}
as required. \hfill \halmos

\endproof

We now work to prove a result similar to Proposition \ref{TimescaleIdleness} for the processes $I_{+}^{(k)}$ and $I_{-}^{(k)}$.

\begin{lemma}\label{IntNI}
\begin{equation*}
\sup_{0 \leq t \leq \tau^{(k)}(\eta)}
	\left|
	\int_{0}^{t}
	\bigg[
		\frac{
			\lambda_{\pm}(k^2 s)
			}{
			\mu_{\pm}(k^2 s)-\lambda_{\pm}(k^2 s)}	 
		- \
		\frac{
			\big( 2- \hat{N}^{(k)}(s)\big)_{+} 
			}{ 
			\hat{N}^{(k)}(s) - 1
			}	
	\bigg]
	ds 
	\right| 
\xrightarrow[k\rightarrow\infty]{} 0
\end{equation*}
where here convergence is convergence in probability.
\end{lemma}
\proof{Proof}
Recalling the definitions of $\lambda_{\pm}(s)$ we have for instance, that,
\begin{align}
\frac{
	\lambda^{(k)}_{-}(k^2s)
	}{
	\mu_{-}(k^2 s)-\lambda^{(k)}_{-}(k^2s)
	}  
:= 
\frac{
	(2-\hat{N}^{(k)}(T^{(k)}_m))_+ - 2 k^{-1/2+\epsilon}
	}{
	\hat{N}^{(k)}(T^{(k)}_m)-1+2 k^{-1/2+\epsilon}.
}
\end{align}	
Now since $n\mapsto \frac{(2-n)_+}{n-1}$ is Lipschitz continuous on $n\geq 1+\eta/2$ with Lipschitz constant $2/\eta$. We can apply 
by Lemma \ref{lem:NhatBound} (with $S_k$ chosen so that Lemma \ref{lem:NhatBound3} holds):
\begin{align*}
&
\bigg|
		\frac{
			\lambda_{-}(k^2 s)
		}{
		\mu_{-}(k^2 s)-\lambda_{-}(k^2 s)}	 
	- \
	\frac{
		\big( 2- \hat{N}^{(k)}(s)\big)_{+} 
	}{ 
	\hat{N}^{(k)}(s) - 1
}	
\bigg|
\\
\leq &
\frac{2}{\eta}	\sup_{m\in\mathbb{Z}_+} 
	\sup_{T_m^{(k)}\leq t \leq T_{m+1}^{(k)}} 
	\left|
	\hat{N}^{(k)}\left(\frac{t}{k^2}\right) - \hat{N}^{(k)} \left(\frac{T_m^{(k)}}{k^2}\right)
	\right| + \frac{4}{\eta} k^{-1/2 + \epsilon}
\\	
\leq & 
	\frac{2}{\eta} \delta^{(k)}+ \frac{4}{\eta} k^{-1/2+\epsilon}.
	\end{align*}
	Applying this bound to the integral stated in the lemma gives the result. (The same bound for $\lambda_+$ and $\mu_+$ holds my a more-or-less identical argument.)
	\hfill\Halmos
\endproof




\begin{lemma}\label{IntIPlus}
Almost surely,
	\begin{align}\label{I+Integral}
	\limsup_{k\rightarrow\infty}
	\sup_{m \in \mathbb{Z}_{+}} 
			\frac{1}{k^2}  
			\int_0^{T_m^{(k)}}	
			\left[ 
				I_+^{(k)}(s) 
				-
				\frac{
					\lambda^{(k)}_+(s)
					}{
					\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
					}
			\right]
			ds 
=
&
0
\\
	\liminf_{k\rightarrow\infty}
	\inf_{m \in \mathbb{Z}_{+}} 
			\frac{1}{k^2}  
			\int_0^{T_m^{(k)}}	
			\left[ 
				I_-^{(k)}(s) 
				-
				\frac{
					\lambda^{(k)}_-(s)
					}{
					\mu_-^{(k)}(s)-\lambda_-^{(k)}(s)
					}
			\right]
			ds 
=
&
0
	\end{align}
\end{lemma}
\proof{Proof}
We prove the result for $I_+^{(k)}$. 
The result holds for $I_-^{(k)}$ by a more-or-less identical argument.
Let $T^+_{m+1}$ be the time after $T_m^{(k)}$ that $I^{(k)}_+(s)$ next empties. 
(Here we assume that the process $I^{(k)}_+(s)$ is allowed to continue past time $T_{m+1}^{(k)}$ to $T_{m+1}^{+}$ time with transition rates \eqref{Lambdaplus}.)
 Further, let 
\[
Z_m = 
	\int_{T_m}^{T_{m+1}^+} 
		I_+^{(k)}(s) 
		- 
		\frac{
			\lambda^{(k)}_+(s)
			}{
			\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
			} 
	ds.
\]
We can now expand the integral in \eqref{I+Integral} as follows
\begin{align}
&\frac{1}{k^2}  
	\int_0^{T_m^{(k)}}	
	\left[ 
		I_+^{(k)}(s) 
		-
		\frac{
			\lambda^{(k)}_+(s)
		}{
			\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
		}
	\right]
	ds \notag
	\\
= 
&
\frac{1}{k^2}
	\sum_{m'\leq m}
		\int_{T^{(k)}_{m'-1}}^{T^{(k)}_{m'}}
			I_+^{(k)} (s)
			-
			\frac{
				\lambda^{(k)}_+(s)
				}{
				\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
				}
		ds \notag
\\
=
&
\frac{1}{k^2} 
	\sum_{m'\leq m}
		Z_{m'}
-
\frac{1}{k^2}
	\sum_{m'\leq m}
	\int_{T_{m'}^{(k)}}^{T_{m'}^+}
	\bigg[
		I_+^{(k)}(s)
		-
		\frac{
			\lambda^{(k)}_+(s)
		}{
			\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
		}
		\bigg]	
	ds 
\\
\leq 
& 
\frac{1}{k^2} 
	\sum_{m'\leq m}
		Z_{m'}
+
\frac{1}{k^2}
	\sum_{m'\leq m}
	\int_{T_{m'}^{(k)}}^{T_{m'}^+}
		\frac{
			\lambda^{(k)}_+(s)
		}{
			\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
		}
	ds 	\label{ZExpand}
\end{align}
We now separately bound the summation over $Z$ and integral in \eqref{ZExpand}.

Firstly, for the summation over $Z$. 
%
The term $Z_m$ is the difference between the area under the excursion of an $M/M/1$ queue and its mean, see Lemma \ref{ExcusionLemma4}.
Thus, by Lemma \ref{ExcusionLemma4}, 
\[
\mathbb{E} \left[ Z_m \Big| \mathcal{F}_{T^{(k)}_m} \right] =0
\]
for all $m\in\mathbb{Z}_+$. 
In other words, the sum over $Z_m$ is a Martingale difference sequence. 
By Lemma \ref{ExcusionLemma}, $Z_m$ is of finite variance. So, by Lemma \ref{MgSLLN},
\[
\sup_{m} \left| \frac{1}{k^2}\sum_{m'\leq m} Z_{m'}\right| \xrightarrow[k\rightarrow\infty]{ a.s.}0
\]
\iffalse
Finally since the number of transitions that must occur before time $k^2T$ is eventually less that $(1+e^2)k^2T$ by Lemma \ref{PoissonBound}. We see that the required bound \eqref{I+Integral} holds and \eqref{I-Integral} follows by an analogous argument.
\fi

Now consider the second integral in \eqref{ZExpand}. Since we chose times $s\leq k^2 \tau^{(k)}(\eta)$, we have that 
\[
0\leq \frac{
	\lambda^{(k)}_+(s)
}{
	\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
}
\leq 
\frac{6\mu}{\eta}.
\]
Further we have that
\begin{align*}
	\frac{1}{k^2}
	\sum_{m'\leq m} 
		T^+_{m'} - T^{(k)}_{m'} 
&\leq 
	\frac{1}{k^2}
	\sum_{m'\leq m} 
		T^+_{m'} - T^{-}_{m'} 
\\
&=
	\frac{1}{k^2}
	\sum_{m'\leq m} 
		T^+_{m'} - \mathbb{E} T^+_{m'} 	
		- 
		\frac{1}{k^2}
	\sum_{m'\leq m} 
		T^{-}_{m'} -\mathbb{E} T^{-}_{m'} 
		+
				\frac{1}{k^2}
	\sum_{m'\leq m} 
		\mathbb{E} T^{+}_{m'} -\mathbb{E} T^{-}_{m'} \\
&
\xrightarrow[k\rightarrow\infty]{ a.s.}0 
\end{align*}
The first two terms above converge to zero, by Lemma \ref{MgSLLN}, since again they are a martingale difference sequence. The expectations in the final term can be calculated explicitly, in particular,
\begin{equation*}
		\mathbb{E} T^{+}_m =
		\frac{1}{1-\lambda_{m,+}^{(k)}/\mu_{m,+}^{(k)}} - \frac{1}{\lambda_{m,+}^{(k)}},
		\qquad 
		\mathbb{E} T^{-}_m =
		\frac{1}{1-\lambda_{m,-}^{(k)}/\mu_{m,-}^{(k)}} - \frac{1}{\lambda_{m,-}^{(k)}}
\end{equation*}
and thus $\mathbb{E} T^{+}_m - \mathbb{E} T^{+}_m $ convergences to zero since $\lambda_{m,+}^{(k)}$ and $\lambda_{m,-}^{(k)}$ (and $\mu_{m,+}^{(k)}$ and $\mu_{m,-}^{(k)}$) converge to the same value. 
Thus the 2nd integral in \eqref{ZExpand} also convergences to zero:
\begin{equation}
0\leq \frac{1}{k^2}
	\sum_{m'\leq m}
	\int_{T_{m'}^{(k)}}^{T_{m'}^+}
		\frac{
			\lambda^{(k)}_+(s)
		}{
			\mu_+^{(k)}(s)-\lambda_+^{(k)}(s)
		}
	ds 
\leq 
\frac{6\mu}{\eta}	\frac{1}{k^2}
	\sum_{m'\leq m} 
\left(	
	T^+_{m'} - T^{(k)}_{m'} 
\right) 
\xrightarrow[k\rightarrow\infty]{ a.s.}0 .
\end{equation}
Thus since each term in \eqref{ZExpand} converges to zero we have the required result.
\hfill \halmos
 
\endproof


\iffalse
\begin{lemma} Almost surely,
	\[
	\sup_{0\leq t\leq k^2 T} \left| \frac{1}{k^2} \sum_{m : T_m \leq t} T^+_m -T^-_m \right| \xrightarrow[k\rightarrow \infty]{} 0.
	\]
\end{lemma}
\proof{Proof} \Neil{This proof is a little sketchy fill in more details...}
Let 
\[
Z_m^+ = T_m^+ - \mathbb{E}T_m^+\qquad\text{and}\qquad Z_m^- = T_m^- - \mathbb{E}T_m^-
\]
Then by Lemma \ref{MgSLLN}
\[
\sup_{t\leq c k^2T} \left| \frac{1}{k^2}\sum_{i=1}^{k^2} Z^+_m\right| \xrightarrow[k\rightarrow\infty]{ }0,\qquad \sup_{t\leq c k^2T} \left| \frac{1}{k^2}\sum_{i=1}^{k^2} Z^-_m\right| \xrightarrow[k\rightarrow\infty]{ }0
\]
The result then holds by the fact that 
\[
\mathbb{E}T_m^+ - \mathbb{E}T_m^- \xrightarrow[k\rightarrow \infty]{ }0.
\]
(\Neil{Fill in details above...})
\hfill \halmos
\endproof
\fi

\subsection{Proof of Proposition \ref{TimescaleIdleness}}\label{sec:Prop3Proof}
We are now in a position to prove Proposition \ref{TimescaleIdleness}. 
With Lemma \ref{IdleCoupling}, we have found a suitable processes $I_-^{(k)}$ and $I_+^{(k)}$ to bound to the idleness processes $\hat{I}^{(k)}$. Further, in Lemmas \ref{IntNI} and \ref{IntIPlus}, we see that $I_-^{(k)}$ and $I_+^{(k)}$ obey a similar limit result to that required by Proposition  \ref{TimescaleIdleness}. We now put these together to prove the proposition.

\proof{Proof of Proposition \ref{TimescaleIdleness}.}
By Lemma \ref{IdleCoupling}, with probability greater than $1-\gamma e^{-\beta k^{\epsilon/2}}$ we have that
\begin{subequations}\label{Expanded0}
\begin{align}
&
\frac{1}{k^2}
	\int_{0}^{T^{(k)}_m} 
	\left[ 
		I_-^{(k)} (s) 
		-
		\frac{\lambda_-(s)
		}{
		\mu_-(s) - \lambda_-(s)
		} 
	\right]
		ds
+
	\int_{0}^{T^{(k)}_m/k^2}
	\Bigg[ 
		\frac{\lambda_-(k^2s)
		}{
		\mu_-(k^2s) - \lambda_-(k^2s) 
		}		
		-
		\frac{\big( 2- \hat{N}^{(k)}(s)\big)_+}{\hat{N}^{(k)}(s)-1} 
	\Bigg]
	ds 
\label{Expanded1}
\\
\leq 
&
	\frac{1}{k^2} 
		\int_{0}^{T_{m}^{(k)}} 
			\hat{I}^{(k)}(s) 
		ds 
		-
		\int_{0}^{ T_{m}^{(k)}/k^2} 
			\frac{\big( 2- \hat{N}^{(k)}(s)\big)_+}{\hat{N}^{(k)}(s)-1} 
		ds 
\notag
\\
\leq
&
\frac{1}{k^2}
	\int_{0}^{T^{(k)}_m} 
		\left[ 
			I_+^{(k)} (s) 
			-
			\frac{\lambda_+(s)
				}{
				\mu_+(s) - \lambda_+(s)
			} 
		\right]		
		ds
+
	\int_{0}^{T^{(k)}_m/k^2}
	\Bigg[ 
		\frac{
			\lambda_+(k^2 s)
			}{
			\mu_+(k^2 s) - \lambda_+(k^2 s)
			}		
	-
	\frac{\big( 2- \hat{N}^{(k)}(s)\big)_+}{\hat{N}^{(k)}(s)-1} 
\Bigg]
	ds.
	\label{Expanded3} 
\end{align}
\end{subequations}
The first integral in \eqref{Expanded1} and \eqref{Expanded3} converges in probability to zero by Lemma \ref{IntIPlus}. The second integral in \eqref{Expanded1} and \eqref{Expanded3} converges in probability by Lemma \ref{IntNI}. Thus 
\begin{equation*}
	\sup_{m} 
	\left|
	\frac{1}{k^2} 
	\int_{0}^{T^{(k)}_m} \hat{I}^{(k)} (s) ds
		-
		\int_{0}^{T^{(k)}_m/k^2}	
			\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}
				ds 
	\right|		\xrightarrow[k\rightarrow\infty]{} 0
\end{equation*}
where the above convergence is convergence in probability. Combining this with Lemma \ref{LemTm} gives Proposition \ref{TimescaleIdleness}.
\hfill\Halmos 
\endproof

\iffalse
\subsection{Controlling Errors}
The above Martingale result should be enough to say that

\[
\frac{1}{k^2} \left[  \int_0^{k^2t} I_+(s) ds  - \int_{0}^{k^2 t}  \frac{ \mu (2-\hat{N}^{(k)}(T^{(k)}_i))_++ C k^{-1/2+\epsilon}}{\mu - \frac{\alpha}{k} -\mu(2-\hat{N}^{(k)}(T^{(k)}_i))_++ C k^{-1/2+\epsilon}} ds \right] = \frac{M_{k^2 t}}{k^2} 
\]
Then dealing with error terms this is sufficient to show that 
\[
\frac{1}{k^2} \left[  \int_0^{k^2t} I_+(s) ds -  \int_{0}^{k^2 t}  \frac{ \mu (2-\hat{N}^{(k)}(s))_+ }{\mu-\mu(2-\hat{N}^{(k)}(s))_+} ds\right]\xrightarrow[k\rightarrow \infty]{u.o.c.} 0
\]

Similarly, we should have
\[
\frac{1}{k^2} \left[  \int_0^{k^2t} I_-(s) ds -  \int_{0}^{k^2 t}  \frac{ \mu (2-\hat{N}^{(k)}(s))_+ }{\mu-\mu(2-\hat{N}^{(k)}(s))_+} ds\right]\xrightarrow[k\rightarrow \infty]{u.o.c.} 0
\]
and thus, by the coupling bound
\[
\frac{1}{k^2} \left[  \int_0^{k^2t} \hat{I}^{(k)}(s) ds -  \int_{0}^{k^2 t}  \frac{ \mu (2-\hat{N}^{(k)}(s))_+ }{\mu-\mu(2-\hat{N}^{(k)}(s))_+} ds\right]\xrightarrow[k\rightarrow \infty]{u.o.c.} 0
\]
which is what is required in the sketch above.
\fi

\iffalse
\subsection{2nd Time Scale Separation}
\Neil{DO THIS SECTION LATER}

\begin{theorem}
	Given $|Q_\kappa(0) - Q_{\kappa'}(0)| \leq 1$ and $I^{(k)}(0)=0$ and suppose that 
	\[
	\frac{N^{(k)}(0)}{k}\Rightarrow \hat{N}(0).
	\]
	For $1< \hat{N}(0) < 2$, 
	\[
	I^{(k)}\left(\frac{t}{k}\right) \Rightarrow \mathcal M(t)
	\]
	where $\mathcal M$ is a M/M/1 queue with arrival rate $(2 - \hat{N}(0))\mu$ and departure rate $\mu$.
	
	For $i \leq \hat{N}(0) \leq (i+1)$, $i\geq 2$ 
	\[
	M_{i-2} \left(\frac{t}{k}\right) \Rightarrow \mathcal M'(t)
	\] 
	where $\mathcal M'$ is an M/M/1 queue with arrival rate $\mu \hat{M}_{i-1}(0)$ and departure rate $\mu$.
\end{theorem}
\proof{Proof}{\Neil{To Do}}
\endproof
\fi

\iffalse


\subsection{Bounds for a Single Jump}
We provide bounds on our coupling for a single jump. Note that 
\[
\hat{I}^{(k)} (t) = \hat{I}^{(k)} (0) + {\mathcal N}_d\left( \mu \int_0^t \hat{M}^{(k)}_1 \big( \frac{s}{k^2} \big) ds  \right) - {\mathcal N}_A\left( \mu \int_0^t \frac{\lambda^{(k)}}{k} \bI \left[\hat{I}^{(k)} \big( s \big) = 0 \right] ds  \right).
\]
Let 
\[
J^{(k)}=J^{(k)}_A \wedge J^{(k)}_d
\]
be the next jump of $\hat{I}^{(k)}$. The two terms above correspond to the jump being the arrival and departure of an Idle server, respectively. More explicitly, for independent exponential mean 1 random variables $E_A$ and $E_D$ we have that 
\[
\mu \int_0^{J_A^{(k)}} \hat{M}_1^{(k)}\left( \frac{s}{k^2} \right) ds = E_A, \qquad \text{and}\qquad \int_0^{J_D^{(k)}} \frac{\lambda^{(k)}}{k} {\mathbb I} [\hat{I}^{(k)}(s)=0]ds=E_D.
\]

Further we let $J_A$ and $J_D$ solve the equations
\[
\mu J_A \hat{M}^{(k)} (0) =E_A,\qquad \mu J_D = E_D, 
\]
where $E_A$ and $E_D$ are as defined above, and we let
\[
J=J_A\wedge J_D.
\]


\[
J^{(k)}=
\]


\begin{lemma}
	\[
	J_A\left( 1- 4 \frac{\delta_k}{\mu \hat{M}_1^{(k)}(0)}\right) \leq J_A^{(k)} \leq J_A \left( 1+  4 \frac{\delta_k}{\mu \hat{M}_1^{(k)}(0)}\right)  
	\] 
\end{lemma}



\begin{lemma}
	\[
	J_D \leq J_D^{(k)}	\leq J_D \left[ 1+ \frac{\alpha}{\mu k} \right]
	\]
\end{lemma}

\begin{corollary}
	\[
	|J-J^{(k)}| \leq J \left[ \frac{4}{\mu M_1^{(k)}} \delta + 4\frac{\alpha}{\mu k}\right]
	\]	\end{corollary}


We also need jumps of the same type to occur, as the following lemma describes.
\begin{lemma}
	For constant C (not depending on k) we have that 
	\[
	{\mathbb P} \left( \hat{I}^{(k)}(J^{(k)}) -\hat{I}^{(k)} (J_-^{(k)}) \neq \hat{I}(J)-\hat{I}(J_-)\right)\leq C\delta_k
	\]
\end{lemma}


\begin{lemma}
	\[
	{\mathbb P} \left( |J-J^{(k)} | \leq 4 \frac{\delta_k}{\mu \hat{M}_1^{(k)}(0) }J, I^{(k)}(J^{(k)}) = I(J) \right) \geq 1- C \delta_k - \epsilon_k
	\]
\end{lemma}
\fi


\section{Properties of Stochastic Differential Equations for $\hat{N}$}
Thus far we have focused on the weak convergence of the stochastic processes $\hat{N}^{(k)}$. 
In this section we focus on the properties of the limit stochastic differential equation:
\begin{equation*}
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0.
\end{equation*}
In Lemma \ref{CTS_SDE} we prove continuity of solutions of the above SDE with respect to data given by the driving process $(B(t): t \geq 0)$.
In Lemma \ref{DiffZero} we prove path-wise uniqueness of solutions.
In Proposition \ref{JSQ:EqPro} we characterize the stationary distribution of this SDE.  

\begin{lemma}\label{CTS_SDE}
	Consider the integral form
	\begin{equation}\label{IntForm}
	n(t) = n(0) + \sqrt{2\mu} b(t) + \mu \int_0^t \left[  \frac{(2-n(s))_+}{(n(s)-1)} - \alpha \right] dt.
	\end{equation}
	Let $b(t)$ be a continuous function and $n(t)$ a solution to the integral expression, above, with $n(t)$ strictly greater than 1. %If $(b^{(k)},n^{(k)})$ are a sequence of solution to the integral expression belonging to $D^2$ and such that $b^{(k)}$ converges uniformly on compacts to $b$
	%then $n^{(k)}$ converges uniformly on compacts to $n$.
%
If we let $\tau^{(k)}(\eta)$ be the first time that $n^{(k)}(s) \leq 1+ \eta $ and $b^{(k)}$ converges to $b$ uniformly on compacts in $[0,\tau^{(k)}(\eta)]$, i.e. for all $\eta>0$ and $T>0$
	\[
	\sup_{0\leq t \leq \tau^{(k)}(\eta)\wedge T} |b^{(k)}(t) - b(t)| \xrightarrow[k\rightarrow\infty]{} 0
	\]
	then $n^{(k)}$ approaches $n$ uniformly on compacts, that is,
\begin{equation*}
		\sup_{0\leq t \leq T} 
|n^{(k)}(t) - n(t)| \xrightarrow[k\rightarrow\infty]{} 0
\end{equation*}

\end{lemma}




\proof{Proof}
Suppose $b(t)$ is continuous and such that $n(t)>0$. 
%
Let $\eta$ be the minimum value of $n(t)-1$ for $t\leq T$.
%
Note that on this domain the function $n\mapsto (2-n)_+/(n-1)$ is Lipschitz continuous with Lipschitz constant $\eta^{-1}$. 
% 
Let $\tau^{(k)}=\tau^{(k)}(\eta/2)$ be the first time that $n^{(k)}\leq 1+ \eta/2$ occurs.
By assumption for each $\epsilon>0$, there exists a $K$ such the for all $k\geq K$ we have that 
\[
|n^{(k)}(0) - n(0) | 
+
\sqrt{2\mu}\sup_{t\leq T} \left| b^{(k)}(t) - b(t) \right| \leq \epsilon .
\]
Further we choose $\epsilon>0$ such that 
\begin{equation} \label{epsiloncond}
\epsilon < \frac{\eta}{2} e^{-\eta^{-1}T}
\end{equation}




With the triangle-inequality, we can bound the process for times $t\leq \tau^{(k)}\wedge T$ as follows
\[
| n^{(k)}(t) - n(t)| 
\leq 
| n^{(k)}(0) - n(0) | 
+ \sqrt{2\mu} |b^{(k)}(t)-b(t)| 
+  \mu \int_0^t 
\left|
\frac{(2-n^{(k)}(s))_+}{(n^{(k)}(s)-1)} - \frac{(2-n(s))_+}{(n(t)-1)}
\right| ds
\]
Thus applying the Lipschitz condition and maximizing over $t$ we have that
\begin{align*}
&\sup_{t\leq \tau^{(k)} \wedge T} 
| n^{(k)}(t) - n(t)| \\
&\leq 
| n^{(k)}(0) - n(0) | 
+ \sqrt{2\mu} \sup_{t\leq \tau^{(k)} \wedge T} |b^{(k)}(t)-b(t)| 
+  \mu \int_0^{\tau^{(k)} \wedge T}
\eta^{-1} \sup_{u\leq s} 
| n^{(k)}(u) - n(u)| ds .
\end{align*}
Applying Gronwall's Lemma, we have that
\begin{align}
\sup_{t\leq \tau^{(k)} \wedge T} 
| n^{(k)}(t) - n(t)|  
&\leq   
\left[ | n^{(k)}(0) - n(0) | 
+ \sqrt{2\mu} \sup_{t\leq T\wedge \tau^{(k)}} |b^{(k)}(t)-b(t)| \right] e^{\eta^{-1} T} \\
&\leq \epsilon e^{\eta^{-1} T} \label{epsilonBound} \\
&< \frac{\eta}{2} \label{HitBound}
\end{align}
where the second inequality above holds by the definition of $\epsilon$ and the final inequality holds by condition \eqref{epsiloncond}. By Inequality \eqref{HitBound} we see that for our choice of $\epsilon$ that
\[
(n^{(k)}(t) -1) > (n(t) -1)  -\frac{\eta}{2} \geq \frac{\eta}{2} 
\]
for all times $t\leq \tau^{(k)}\wedge T$. Thus $\tau^{(k)}>T$, and therefore, Inequality \eqref{epsilonBound} now states 
\begin{equation}
\sup_{t\leq T} | n^{(k)}(t) - n(t)|
\leq   \epsilon e^{\eta^{-1} T}
\end{equation}
In other words, we see that as required
\[
\lim_{k\rightarrow\infty}\sup_{t\leq T} | n^{(k)}(t) - n(t)| = 0.
\]
\hfill \Halmos
\endproof





The following proposition summarizes the properties of SDE \eqref{JSQ:Diffusion}.
\begin{lemma}\label{DiffZero}
	A solution to the SDE 
	\begin{equation}\label{SDE1}
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
	\end{equation}
	exists, and is path-wise unique. Further the explosion time is almost surely not finite.
\end{lemma}
\proof{Proof}
We can prove the result with a localization argument. In particular, for $\epsilon \in (0,\frac{1}{2})$, we consider the stopping times 
$\tau_\epsilon= \inf\{t : \hat{N}(t) = 1+\epsilon \}$ and define $\tau_1 = \lim_{\epsilon\rightarrow 0} \tau_{\epsilon}$ to be the explosion time of the SDE \eqref{SDE1}. The processes $\hat{N}(t)$, for $t\leq \tau_\epsilon$ satisfies an SDE with Lipschitz coefficients. Such SDEs are known to be path-wise unique, for instance, see \cite{rogers2000diffusions}, Theorem V.11.2. So solutions to the SDE, \eqref{SDE1}, are path-wise unique until time $\tau_\epsilon$.
% 
So path-wise uniqueness holds on each time interval $[0,\tau_\epsilon)$.

We will now show that, almost surely, $\tau_1=\infty $, and thus, path-wise uniqueness holds for all time.
%
Notice that without loss of generality, we may assume that the initial condition satisfies $1<\hat{N}(0)<2$ (because if the limit $\lim_{\epsilon\rightarrow 0} \tau_\epsilon $ were finite then there exists a stopping time such that $\hat{N}(\tau_\epsilon ) < 2$ and invoking the strong Markov property we can start from this time instead -- Note, local Lipschitz continuity of coefficient ensures the process is Strong Markov up to its time of explotion.) Further, let $\tau_2 = \inf\{t : \hat{N}(t) = 2 \}$. Notice that, by a similar argument, if $\mathbb P ( \tau_1 < \infty ) >0$ then $\mathbb P ( \tau_1 < \tau_2 ) >0$. (If explosion occurs then, every time there must be a positive probability that explosion occurs before $\hat{N}$ hits to $2$.)

For times $t < \tau_1 \wedge \tau_2$ the process obeys the SDE
\begin{equation}
d \hat{N} (t) = \mu  \Big[ \frac{1}{\hat{N}-1}-(\alpha+1)\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0.
\end{equation}
Notice that aside from the drift of $-(\alpha+1)$ the above processes is similar to a Bessel process. (In particular, if we remove the drift term $-(\alpha+1)$ then $(\hat{N}-1)/\sqrt{2\mu} $ would be is a Bessel process of Dimension 2.) By Girsanov's Theorem we can add and remove this drift, with an exponential change of measure. Thus on each compact time interval, a zero probability event with drift is a zero probability event without a drift. It is well known that a $2$ dimensional Bessel process is non-explosive, since two dimensional Brownian motion is neighbourhood recurrent at zero, see \cite{rogers2000diffusions} Section VI.35 for a proof. Thus $\mathbb P ( \tau_1 < \tau_2 ) = 0$. Thus the result now follows from the existence and uniqueness of SDEs with Lipschitz coefficients. 
	(Further, an alternative proof is provided by the Watanabe-Yamada path-wise uniqueness theorem; see \cite{rogers2000diffusions} Theorem V.40.1.)
	\hfill \Halmos
\endproof 

\iffalse
(\Neil{See pages 5-6-7 on your NDS write.pdf for more details on continuity of solutions etc})
\Neil{Existence:} Existence is a consequence of the weak convergence result Theorem ??.\\
\Neil{Pathwise Uniqueness:} \Neil{You have two proofs here}  Is a consequence of Watanabe and Yamada path-wise uniqueness Theorem. See Williams and Rogers, Theorem V.40.1. 	Given the event $\hat{N}=1$ does not occur,  Further, by Lemma \ref{NotZero}, $\tau_\epsilon \rightarrow \infty$ as $\epsilon\rightarrow 0$. Thus this implies path-wise uniqueness of the SDE.\\
\Neil{Non-zero Property:} 
\iffalse
\Neil{Exponentially Ergodic:} This follows from notes of Martin Hairer (Convergence of Markov Processes, Section 7). \Neil{(Probably don't need this result.)}\\
\Neil{Expected Value Calculation:} This follows from repeated application of the identity,
\[
\int_0^{\infty} x^d e^{-\alpha x}dx = \frac{d!}{\alpha^{d+1}}
\]
for the calculation, see your pdf (Stationary Distributions.pdf).
\fi
\fi


\begin{proposition}\label{JSQ:EqPro}
	The SDE 
	\begin{equation}
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
	\end{equation}
has a stationary distribution with probability density function 
	\begin{equation}\label{JSQ:Equilibrium2}
	\frac{d\pi}{dn} \propto 
	\begin{cases}
	\exp \left\{ -\alpha (n-2) \right\}, & n \geq 2, \\
	(n-1)\exp \left\{ -(\alpha+1)(n-2) \right\}, & 1\leq n\leq 2.
	\end{cases}
	\end{equation}
and this distribution has expected value:
	\begin{align} \label{ENHat}
	\bE [\hat{N}] 
%= 1+ \left[ \frac{1}{\alpha (1+\alpha)^2} + \frac{e^{1+\alpha}}{(1+\alpha)^2} \right]^{-1}\left[  \frac{\alpha^2+4\alpha+1}{\alpha^2 (1+\alpha)^3} + \frac{2 e^{\alpha+1}}{(1+\alpha)^3} \right]\\
=	1+ \left[ \frac{1}{\alpha (1+\alpha)^2} + \frac{e^{1+\alpha}}{(1+\alpha)^2} \right]^{-1}\left[  \frac{\alpha^2+4\alpha+1}{\alpha^2 (1+\alpha)^3} + \frac{2 e^{\alpha+1}}{(1+\alpha)^3} \right]
\iffalse
	\frac{
		e^{\alpha+1} 
		\Big[
		\frac{2}{(\alpha+1)^3}
		+
		\frac{1}{(\alpha+1)^2}
		\Big]
		-
		\Big[
		\frac{2}{(\alpha+1)^3}
		+
		\frac{3}{(\alpha+1)^2}
		+
		\frac{2}{(\alpha+1)}
		\Big]		
		+	
		\Big[
		\frac{1}{\alpha^2}
		+
		\frac{2}{\alpha}
		\Big]
	}
	{
		\frac{e^{(\alpha+1)}-1}{(\alpha+1)^2}
		+
		\frac{1}{\alpha(1+\alpha)}
	}
\fi 
	\end{align}
\end{proposition}
\proof{Proof}
Applying the substitution $X= \frac{1}{\sqrt{\mu}} \hat{N}$, we have that 
\begin{align}
d X =& \sqrt{2} d B_t + \sqrt{\mu} \left[ \frac{(2-\sqrt{\mu}X)_+}{(\sqrt{\mu}X-1)} - \alpha \right] dt \notag\\
=& \sqrt{2} d B_t - V'(X) dt \label{DiffForm}
\end{align}
where $V(x)$ is a function with derivative 
\[
V'(x) =\sqrt{\mu} \left[ \alpha - \frac{(2-\sqrt{\mu}x)_+}{(\sqrt{\mu}x-1)}   \right]
\]
The diffusion \eqref{DiffForm} is a Langevin Diffusion. It is well known that such diffusions have an invariant measure given by
\[
\tilde{\pi}(x)= \exp\{-V(x) \}.
\]
This can be verified directly as $\pi$ is a stationary solution to the Fokker-Plank equations. (A more exacting analysis giving exponential convergence of Langevin diffusions to stationarity is given in \cite{roberts1996}.)

What remains are somewhat tedious calculations resulting in the required expression \eqref{JSQ:Equilibrium2} and \eqref{ENHat}. For \eqref{JSQ:Equilibrium2}, integrating the expression for $V'(x)$ we get that 
\begin{align*}
V(x) 
&= \sqrt{\mu} \int_{\frac{2}{\sqrt{\mu}}}^{x} \alpha - \frac{(\frac{2}{\sqrt{\mu}}-x)_+}{(x-\frac{1}{\sqrt{\mu}})}dx\\
&= \sqrt{\mu} \alpha \left(x-\frac{2}{\sqrt{\mu}}\right) + \sqrt{\mu}\mathbb{I}\left[1<\sqrt{\mu}X<2\right] \int_{x}^{\frac{2}{\sqrt{\mu}}} \frac{\frac{2}{\sqrt{\mu}}-x}{x-\frac{1}{\sqrt{\mu}}}dx\\
&=
\sqrt{\mu} \alpha \left(x-\frac{2}{\sqrt{\mu}}\right) + \sqrt{\mu}\mathbb{I}\left[1<\sqrt{\mu}X<2\right] \int_{x}^{\frac{2}{\sqrt{\mu}}} \left[ \frac{\frac{1}{\sqrt{\mu}}}{x-\frac{1}{\sqrt{\mu}}} - 1 \right] dx\\
&=\sqrt{\mu} \alpha \left(x-\frac{2}{\sqrt{\mu}}\right) + \sqrt{\mu}\mathbb{I}\left[1<\sqrt{\mu}X<2\right]
\left[ 
\frac{1}{\sqrt{\mu}} \log \left(\frac{1}{\sqrt{\mu}}\right) - \frac{1}{\sqrt{\mu}} \log \left(x-\frac{1}{\sqrt{\mu}}\right) + \left(x-\frac{1}{\sqrt{\mu}}\right)
\right]
\end{align*}
Therefore we arrive at an invariant distribution $\tilde{\pi}$ with density
\[
\frac{d \tilde{\pi}}{d x}= \exp\{-V(x) \} = 
\begin{cases}
\exp \left\{-\sqrt{\mu}\alpha \left( x- \frac{2}{\sqrt{\mu}} \right)\right\} & \text{if } x \geq \frac{2}{\sqrt{\mu}} \\
\left( \sqrt{\mu} x -1 \right)\exp \left\{ -\sqrt{\mu}(\alpha +1) \left( x -\frac{2}{\sqrt{\mu}}\right)  \right\} & \text{if } x < \frac{2}{\mu}.
\end{cases}
\]


So substituting back $X= \frac{1}{\sqrt{\mu}} \hat{N}$, we see the stationary distribution for $\hat{N}$, $\pi(n)$, is given by.
\[
\frac{d \pi }{d n} =
\begin{cases}
C\exp\{-\alpha (n-2)\}, & \text{if } n \geq 2, \\
C (n-1)\exp \{- (\alpha +1) (n-2) \}, & \text{if } 1\leq n \leq 2.
\end{cases}
\]
where 
\[
C= \int_0^2 (n-1)\exp \{- (\alpha +1) (n-2) \} dn + \int_2^\infty \exp\{-\alpha (n-2)\} dn
\] 
is a normalizing constant that we will now calculate.  


To calculate the normalizing constant $C$ and the expectation \eqref{ENHat}. We make use of the following standard (Gamma function) identity
\[
\int_{0}^{\infty} n^s e^{-\theta n}dn= \frac{s!}{\theta^{s+1}}.
\] 

First, we calculate the two terms in the expression for $C$, above. Namely
\begin{align*}
&\int_1^2 (n-1) e^{- (\alpha+1)(n-2) } dn \\
= &\int_{1}^{\infty} (n-1) e^{-(\alpha+1)(n-1)} \cdot e^{-(\alpha+1)}dn- \int_2^{\infty} (n-2) e^{-(\alpha+1)(n-2)}dn - \int_2^\infty e^{- (\alpha +1) (n-2)}dn \\
=& e^{\alpha+1} \frac{1}{(\alpha+1)^2} - \frac{1}{(\alpha+1)^2} - \frac{1}{(\alpha+1)}
\end{align*}
and
\begin{align*}
\int_2^\infty e^{-\alpha(n-2)} dn = \frac{1}{\alpha}. 
\end{align*}
Thus
\begin{equation}\label{Ccalc}
	C= \frac{e^{(\alpha+1)}-1}{(\alpha+1)^2} + \frac{1}{\alpha} - \frac{1}{\alpha+1}.
\end{equation}

Second, we calculate the expected value of $\hat{N}$. 
\begin{align*}
C\mathbb{E} \hat{N} & = \int_1^2 n(n-1) e^{-(\alpha+1)(n-2)} dn + \int_2^\infty n e^{-\alpha(n-2)}dn \\
&=\int_1^\infty \underbrace{n(n-1)}_{n(n-1)=(n-1)^2 + (n-1)} e^{-(\alpha+1)(n-2)} dn \\
&\quad - \int_2^\infty \underbrace{n(n-1)}_{n(n-1)=(n-2)^2 + 3(n-2)+2} e^{-(\alpha+1)(n-2)} dn \\
&\quad\quad + \int_2^\infty \underbrace{n}_{n=(n-2)+2} e^{-\alpha(n-2)}dn\\
&= e^{(\alpha+1)} \left[ \int_0^\infty n^2 e^{-(\alpha+1)n}dn + \int_0^\infty n e^{-(\alpha+1) n}dn \right]\\
&\quad - \left[ \int_0^\infty n^2 e^{-(\alpha+1)n } dn + 3 \int_0^\infty n e^{-(\alpha+1)n}dn + 2 \int_0^\infty e^{-(\alpha+1)n}dn\right]\\
& \quad\quad + \left[ \int_0^\infty ne^{-\alpha n}dn + 2\int_0^\infty e^{-\alpha n}dn \right] \\
& = e^{(\alpha+1)} \left[\frac{2}{(\alpha+1)^3} + \frac{1}{(\alpha+1)^2}\right] \\
 &\quad - \left[ \frac{2}{(\alpha+1)^3} + \frac{3}{(\alpha+1)^2} + \frac{2}{(\alpha+1)}\right]\\
 &\quad\quad + \left[ \frac{1}{\alpha^2} + \frac{2}{\alpha} \right].
\end{align*}
This and the value of $C$ calculated above gives the stationary expectation
\begin{equation*}
\mathbb{E} \hat{N} =	\frac{
		e^{\alpha+1} 
		\Big[
		\frac{2}{(\alpha+1)^3}
		+
		\frac{1}{(\alpha+1)^2}
		\Big]
		-
		\Big[
		\frac{2}{(\alpha+1)^3}
		+
		\frac{3}{(\alpha+1)^2}
		+
		\frac{2}{(\alpha+1)}
		\Big]		
		+	
		\Big[
		\frac{1}{\alpha^2}
		+
		\frac{2}{\alpha}
		\Big]
	}
	{
		\frac{e^{(\alpha+1)}-1}{(\alpha+1)^2}
		+
		\frac{1}{\alpha(1+\alpha)}
	}.
\end{equation*}
The formula \eqref{ENHat} is a somewhat simplified form of this expression.
\hfill \Halmos 
\endproof 

\begin{lemma}\label{StationaryProp}
\iffalse 
\begin{equation*}
	d\hat{N}_{IQF} (t)
= 
\mu \left[
		\frac{1}{\hat{N}_{IQF}-1}
		-
		\alpha 
	\right]  dt
+
\sqrt{2\mu}dB(t),\qquad t\geq 0.
\end{equation*}
Note that $\hat{N}_{IQF} $ is a Bessel process with drift $-\alpha \mu t$. 
This process has stationary distribution
$({\pi}_{IQF}(n): n \geq 1)$ with density:
\begin{equation*}
	\frac{d\pi_{IQF}}{dn}
	\propto 	
\begin{cases}
\exp \{-\alpha(n-2) \}	 &	n\geq 2, \\
(n-1) \exp \{ -(\alpha +1)(n-2)\}	& 1\leq n \leq 2.
\end{cases}
\end{equation*}
Here the stationary expected queue size is
\begin{equation*}
	\mathbb{E} [ \hat{N}_{IQF} ] 
	=
	1+ \frac{2}{\alpha}.
\end{equation*}
\fi 
The Idle-Queue-First NDS approximation given by
\begin{equation*}
	d\hat{N}_{IQF} (t)
= 
\mu \left[
		\frac{1}{\hat{N}_{IQF}-1}
		-
		\alpha 
	\right]  dt
+
\sqrt{2\mu}dB(t),\qquad t\geq 0
\end{equation*}
has a stationary expected queue size of
\begin{equation*}
	\mathbb{E} [ \hat{N}_{IQF} ] 
	=
	1+ \frac{2}{\alpha}.
\end{equation*}
\end{lemma}
\proof{Proof}
Note that $\hat{N}_{IQF} $ is a Bessel process with drift $-\alpha \mu t$. Following a more-or-less identical steps from \eqref{DiffForm} through to \eqref{Ccalc}. We see that this process has stationary distribution
$({\pi}_{IQF}(n): n \geq 1)$ with density:
\begin{equation*}
	\frac{d\pi_{IQF}}{dn}
	= 	
\alpha^{2}(n-1)\exp \{-\alpha(n-1) \}.
\end{equation*}
From this it is straightforward calculation to show that
\[
\mathbb{E} [ \hat{N}_{IQF} ]  = 1+ \int_1^\infty \alpha^2 (n-1)^2 e^{-\alpha (n-1)} dn = 1 + \frac{2}{\alpha}.
\]
\hfill\Halmos 
\endproof

Notice from Lemma \ref{StationaryProp} and Central Queue expected queue size \eqref{CQED} that 
\begin{equation}
 \sup_{\alpha} \frac{\mathbb{E}\big[{\hat{N}_{IQF}}\big]}{\mathbb{E}{\big[\hat{N}_{CQ}\big]}} 
=
\sup_{\alpha}
\left\{
\frac{
1 + \frac{2}{\alpha}
}{
1 + \frac{1}{\alpha}
}
\right\}
=
2
\end{equation}
This obtains the expression \eqref{IQF/CQ} from Section \ref{Comparison}. 
Further from \eqref{ENHat} we obtain that 
\begin{align*}
\frac{
\mathbb{E} \hat{N}_{JSQ}
}{
\mathbb{E} \hat{N}_{CQ}
}
&=
\frac{\alpha}{1+\alpha}
\left[ 
	1+ \left[ \frac{1}{\alpha (1+\alpha)^2} + \frac{e^{1+\alpha}}{(1+\alpha)^2} \right]^{-1}\left[  \frac{\alpha^2+4\alpha+1}{\alpha^2 (1+\alpha)^3} + \frac{2 e^{\alpha+1}}{(1+\alpha)^3} \right]
\right]
\\
&=
1- \frac{1}{1+\alpha}
+
\frac{1}{(1+\alpha)^2}
\left[ 
\frac{
\alpha^{2} +4\alpha +1
+2\alpha^2 e^{1+\alpha}
}{
1+\alpha e^{1+\alpha}
}
\right].
\end{align*}
We see that the above expression is continuous for  $\alpha\in (0,\infty)$ and that
\begin{equation*}
\lim_{\alpha\rightarrow \infty}
\frac{
\mathbb{E} \hat{N}_{JSQ}
}{
\mathbb{E} \hat{N}_{CQ}
}	
= 1 
\qquad \text{and} \qquad 
\lim_{\alpha\rightarrow 0}
\frac{
\mathbb{E} \hat{N}_{JSQ}
}{
\mathbb{E} \hat{N}_{CQ}
}	= 1 .
\end{equation*}
Thus this ratio between JSQ and CQ is bounded. 
Due to the combination of exponentials and polynomials there does not appear to be closed form solution for the value of the ratio between JSQ and CQ. However placing in the numerical solver we see that
 \begin{equation*}
\sup_{\alpha >0}
\frac{
\mathbb{E} \hat{N}_{JSQ}
}{
\mathbb{E} \hat{N}_{CQ}
}
\approx 1.13547 	< 1.14
\end{equation*}
and the maximum is achieved at $\alpha =0.209082$ (here we give the first six significant digits). This is the stated expression \eqref{JSQ/CQ} and further is plotted in Figure \ref{fig:NDS_JSQ_IQF}.

\iffalse 
\begin{corollary}
\[
	\pi_{CQ} \leq_{st} \pi_{JSQ} =_{st} \pi_{I1F} \leq_{st} \pi_{IQF}.
\]

\[ \sup_{\alpha} \frac{{\mathbb E}[\hat{N}_{JSQ}]}{{\mathbb E}[\hat{N}_{CQ}]} \leq 1.14 .\]  

\[ \sup_{\alpha} \frac{\mathbb{E}\big[{\hat{N}_{IQF}}\big]}{\mathbb{E}{\big[\hat{N}_{JSQ}\big]}} = 2 .\]  	
\end{corollary}
The second equality above follows by an elementary calculation. 
Thus 
\begin{equation*}
\max_{\alpha\in [0,\infty]}
\frac{
\mathbb{E} \hat{N}_{JSQ}
}{
\mathbb{E} \hat{N}_{CQ}
}
< \infty.	
\end{equation*}
\fi 


\section{Proof of Theorem}\label{sec:main_theorem_proof}

What now follows is the proof of Theorem \ref{JSQ:Thrm}. 

\proof{Proof of Theorem \ref{JSQ:Thrm}}
Recall from \eqref{NTerms}, we may write $\hat{N}^{(k)}(t)$ in the form
\begin{subequations}\label{NTerms2}
	\begin{align}
	\hat{N}^{(k)}(t)- \hat{N}^{(k)}(0)  =& {\mathcal M}_a\left( \mu t - \frac{\alpha}{k} \mu t \right) - {\mathcal M}_d\left( \mu t - \frac{\mu}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right) \label{NTerms2a} \\
	& + \frac{\mu}{k^2}\int_0^{k^2t} \hat{I}^{(k)}(s)ds - \mu \int_0^{t}  \frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds \label{NTerms2b}\\
	&- \alpha \mu t + \mu \int_0^{t}  \frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}_1(s)-1 ) } ds.\label{NTerms2c}
	\end{align}
\end{subequations}
First consider the right-hand side of \eqref{NTerms2a}. By Corollary \ref{Cor:MtoB} (and the Martingale FCLT) we have that 
\[
\left( {\mathcal M}^{(k)}_a\left( \mu t - \frac{\alpha}{k}\mu t \right) - {\mathcal M}^{(k)}_d\left( \mu t - \frac{\mu}{k^2} \int_0^{kt} I^{(k)}(s)ds  \right)  : t\geq 0\right)\Rightarrow ( \sqrt{2\mu} B(t) : t \geq 0)
\]

Next consider \eqref{NTerms2b}. By Proposition 
\ref{TimescaleIdleness}, for all $\eta >0$
\[
	\sup_{0\leq t\leq \tau^{(k)}(\eta)} 
		\left| 
			\frac{1}{k^2} 
				\int_{0}^{k^2t}	\hat{I}^{(k)}(s)ds 
			- 
				\int_{0}^{t}	
					\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}
				ds 
			\right| 
	\xrightarrow[k\rightarrow \infty]{} 
	0.
\]
So defining 
\[
\epsilon^{(k)}(t \wedge \tau^{(k)}(\eta))
=
\frac{1}{k^2} 
		\int_{0}^{k^2(t\wedge \tau^{(k)}(\eta))}	\hat{I}^{(k)}(s)ds 
	- 
		\int_{0}^{(t\wedge \tau^{(k)}(\eta))}	
			\frac{(2-\hat{N}^{(k)}(s))_+}{(\hat{N}^{(k)}(s)-1 )}
				ds ,
\]
we have that 
\[
(\epsilon^{(k)}(t \wedge \tau^{(k)}(\eta)) : t\geq 0, \eta^{-1}\in {\mathbb N}) \Rightarrow 0.
\]
By the Skorohod representation theorem, there exists a probability space were this convergence is almost sure (See \cite{billingsley2013convergence}). That is, almost surely 
\begin{align*}
&\left( \left( {\mathcal M}^{(k)}_a\left( \mu t - \frac{\alpha}{k}\mu t \right) - {\mathcal M}^{(k)}_d\left( \mu t - \frac{\mu}{k^2} \int_0^{kt}\!\! I^{(k)}(s)ds  \right) ,\; \epsilon^{(k)}(t \wedge \tau^{(k)}(\eta))   \right)  : 0\leq t \leq T, \eta^{-1}\in {\mathbb N}\right)\\
&\xrightarrow[k\rightarrow \infty]{u.o.c.} ( (\sqrt{2\mu} B(t),0) : 0\leq t \leq T, \eta^{-1}\in {\mathbb N})	
\end{align*}

Therefore, Lemma \ref{CTS_SDE} applies to give that, almost surely,
\[
(\hat{N}^{(k)}(t): t\geq 0) \xrightarrow[k\rightarrow\infty]{u.o.c.} (\hat{N}(t): t\geq 0) 
\] 
where $(\hat{N}(t): t\geq 0)$ satisfies the S.D.E. 
	\begin{equation}
	d \hat{N} (t) = \mu  \Big[ \frac{(2-\hat{N})_+}{\hat{N}-1}-\alpha\Big] dt + \sqrt{2\mu} \;dB (t), \qquad t\geq 0
	\end{equation}
Here we note that by Proposition \ref{DiffZero} almost surely $\hat{N}(t)>1$ for all $t$, so the conditions of the limit process in Lemma \ref{CTS_SDE} are satisfied. This gives the required weak convergence result. 

The remaining properties on the stationary distribution of $\hat{N}(t)$ are given in Proposition \ref{JSQ:EqPro}. This completes the proof of Theorem \ref{JSQ:Thrm}. \hfill \Halmos
\endproof
\newpage 


==> ECOMPANION_3_Aux.tex <==
\section{Auxiliary Lemmas}\label{sec:auxiliary_lemmas}
This section contains a few somewhat elementary lemmas that will be used repeatedly. 
This Section can be skipped on first reading and referred back to when required.

\begin{lemma}\label{PoissonBound}
	For $Po(\mu)$, a Poisson random variable with parameter $\mu$, it holds that
	\[
	{\mathbb P} \left( Po(\mu) \geq x  \right) \leq e^{-x-\mu },\qquad	\forall x\geq \mu e^2. 
	\]
	and for $\mathcal{N}(t)$ a unit Poisson process
	\begin{align*}		
	&{\mathbb P} \left( \sup_{0\leq t \leq T} (\mathcal{N}(t) -t)\geq z \right) \leq \exp\big\{-\frac{z^2}{2T}\big(1-\frac{z}{T}\big)\big\},\\
		&		{\mathbb P} \left( \inf_{0\leq t \leq T} (\mathcal{N}(t) -t) \leq -z \right) \leq 2\exp\big\{-\frac{z^2}{2T}\big(1-\frac{z}{T}\big)\big\}.
	\end{align*}
	\end{lemma}
	
\proof{Proof}
	A  Chernoff bound gives
	\[
	{\mathbb{P}}\left(Po(\mu) \geq x \right) \leq e^{-\theta x }\mathbb{E}e^{\theta Po(\mu)} 
	= \exp \left\{ -\theta x + \mu \left(e^\theta -1\right)  \right\}.
	\]
	Minimizing over $\theta \geq 0$, the above is minimized at $\theta = \log (x/\mu)$. Therefore 
	\[
	\mathbb{P} \left(Po(\mu) \geq x  \right) \leq \exp \left\{ - \mu \left[ \left( 1- \frac{x}{\mu}\right)+ \frac{x}{\mu}\log\frac{x}{\mu}\right] \right\}.
	\]
	By assumption $\log \frac{x}{\mu}\geq 2$, substituting this into the logarithms in the square brackets above gives
	\[
	\mathbb{P}\left( Po(\mu) \geq x \right) \leq e^{-\mu - x}
	\]
This gives the first bound. The second follows similarly. By Doob's sub-martingale inequality
\[
{\mathbb P} \left( \sup_{0\leq t \leq T} (\mathcal{N}(t) -t) \geq z \right) \leq e^{-\theta (T+z) }\mathbb{E}e^{\theta Po(T)} = \exp \left\{ - T \left[ -\frac{z}{T} + \left(1+ \frac{z}{T} \right)\log\left(1+ \frac{z}{T} \right)\right] \right\}
\]
where we take $\theta =  \log ((z+T)/\mu)$ as above. Applying the bound $\log (1+y) \geq y-{y^2}/{2}$, gives that
\[
- T \left[ -\frac{z}{T} + \left(1+ \frac{z}{T} \right)\log\left(1+ \frac{z}{T} \right)\right] \leq - T \left[ -\frac{z}{T} + \left(1+ \frac{z}{T} \right)\frac{z}{T}\left(1- \frac{z}{2T} \right)\right] = -\frac{z^2}{2T}\big(1-\frac{z}{T}\big).
\]
The same bound holds for the event $\left\{\inf_{0\leq t \leq T} (\mathcal{N}(t) -t) \leq -z\right\}$ by an identical argument.
\hfill \halmos
\endproof

%%%% 

The following is a basic equality on hitting probabilities of Markov chains.
\begin{lemma}\label{HittingLemma}
	Consider a continuous time birth death process taking values $n$ in $\{0,...,x\}$. Let $f(n)$ be the rate of transitions from $n$ to $n+1$, for $n \neq x$, and $g(n)$ be the rate of transitions from $n$ to $n-1$ for $n\neq 0$. All other transition rates from $n$ are zero. The probability of hitting $x$ before $0$ starting from initial state $1$ is given by the expression
	\[
	\frac{1}{\sum_{n=1}^x \prod^{n-1}_{m=1} \frac{g(m)}{f(m)}}. 
	\]
	(here we apply the convention that $\prod_{m=1}^0 \frac{f(m)}{g(m)}=1$  )
\end{lemma}
\proof{Proof}
The $h_n^x$ be the probability of hitting $x$ before zero when starting from state $n$. 
%
It is clear that $h_n^x$ satisfies the expression
\[
(f(n) + g(n))  h_n^x = f(n) h_{n+1}^x + g(n) h_{n-1}^x 
\]
for $n=1,...x-1$ and $h^x_0=0$ and $h^x_x=1$. Let $u_n = h_n-h_{n-1}$ then the above expression simplifies to give
\[
0=f(n) u_{n+1} - g(n) u_n
\]
for $n=1,...,x-1$, which implies 
\[
u_n = u_1 \prod_{m\leq n-1} \frac{g(m)}{f(m)}
\]
for $n=1,..,x$. Now since 
\[
u_1^x =h_1^x - h_0^x = h_1^x \qquad \text{and} \qquad 1 = h^x_x - h^x_0 = \sum_{n=1}^x u_n ,
\]
we have that
\[
1=h_1^x   \sum_{n=1}^x \prod_{m\leq n-1} \frac{g(x)}{f(x)} 
\]
as required.\hfill \Halmos
\endproof

\begin{lemma}\label{ExcusionLemma}
	Suppose that $Q$ is an M/M/1 queue with arrival rate $\alpha$ and service rate $\beta$, with $\beta > \alpha$. Let $\tilde{T}$ be the length of the renewal cycle from the queue being of length $1$ to the queue being empty again. Then,
	\begin{equation}\label{ExcusionLemma1}
	{\mathbb P} (\tilde{T} \geq t ) \leq e^{\theta + \phi(\theta)t} \qquad \text{and}\qquad {\mathbb P} \left( \int_0^{\tilde{T}} Q(s) ds \geq x\right) \leq e^{-\theta_0 (\sqrt{cx}-1)}
	\end{equation}
	where  $\phi(\theta)=\alpha(e^{\theta}-1) +\beta(e^{-\theta}-1) $, $c>0$
	and  $\theta_0$ is such that $\phi(\theta_0)+ c\theta_0 \leq 0.$
	In particular, $\phi(\theta)$ is minimized by $\theta = \frac{1}{2}\log \frac{\beta}{\alpha}$ and thus
	\begin{equation}\label{ExcusionLemma2}
	{\mathbb P} (\tilde{T} \geq t ) \leq \sqrt{\tfrac{\beta}{\alpha}}e^{-(\sqrt{\beta}- \sqrt{\alpha}) t} .
	\end{equation}
\end{lemma}
\proof{Proof.}
We have that $Q(0)=1$ and that
\[
Q(t) -1 = {\mathcal N}_{\alpha}(t) - {\mathcal N}_{\beta}(t)
\] 
for $t\leq \tilde{T}$ where ${\mathcal N}_\alpha$ and ${\mathcal N}_\beta$ are independent Poisson processes of rates $\alpha$ and $\beta$, respectively.  Note that
\[
\E \left[ e^{\theta ({\mathcal N}_{\alpha}(t) - {\mathcal N}_{\beta}(t))} \right]= e^{t \phi(\theta)}  \quad\text{where}\quad \phi(\theta)=\alpha(e^{\theta}-1) +\beta(e^{-\theta}-1)  .
\]
(Note that, since $\alpha <\beta$, $\phi'(\theta)<0$. So $\phi(\theta)<0$ for some $\theta >0$.)	
Thus 
\[
X(t) = \exp \left\{\theta Q(t\wedge \tilde{T}  )  - (t\wedge \tilde{T})\phi(\theta) \right\}
\]
is a positive martingale which then gives
\[
{\mathbb E} \left[ e^{-\tilde{T}\phi(\theta)} \right] = \bE\left[ X({\infty}) \right]  \leq  {\mathbb E} \left[ X(0) \right] = e^{\theta}.
\]
Applying a Chernoff bound, we get the inequality
\[
{\mathbb P} (\tilde{T} > t) \leq  {\mathbb E} \left[e^{-\phi(\theta) \tilde{T}} \right] e^{\phi(\theta)t} \leq e^{\theta + \phi(\theta)t}.
\]
This gives the required bound on the left-hand side of \eqref{ExcusionLemma1}.
We now optimize $\phi(\theta)$ to gain inequality \eqref{ExcusionLemma2}. In particular, 
\[
0=\phi'(\theta) = \alpha e^{\theta} - \beta e^{-\theta}  \quad \text{which implies} \quad  \theta^* = \frac{1}{2} \log \frac{\beta}{\alpha}.
\]
Substituting back into $\phi$ gives
\[
\phi(\theta^*)= \alpha \left(\sqrt{\frac{\beta}{\alpha}} -1 \right) + \beta \left(\sqrt{\frac{\alpha}{\beta}} -1 \right)=- \left(\sqrt{\beta} -\sqrt{\alpha} \right)^2
\] 
which then gives the required bound
	\[
	{\mathbb P} (\tilde{T} \geq t ) \leq \sqrt{\tfrac{\beta}{\alpha}}e^{-(\sqrt{\beta}- \sqrt{\alpha})^2t} .
	\]


The bound  on the right-hand side of \eqref{ExcusionLemma1} follows by a similar argument, as follows. Define 
\[
Q^c(s)  := Q(s) +cs= 1+{\mathcal N}_{\alpha}(s) - {\mathcal N}_{\beta}(s) + cs \quad \text{and}\quad 
X^c (t) := \exp \left\{\theta Q^c(t)  -\phi(\theta)t-ct\right\}
\]
for some constant $c$ such that $\alpha + c \leq \beta$. 
(Here we have essentially added an additional upward drift to our queueing process.) 
Again,
\[
\E \left[ e^{\theta ({\mathcal N}_{\alpha}(s) - {\mathcal N}_{\beta}(s) + cs) }  \right]= e^{s (\phi(\theta)+c\theta)}  \quad\text{where}\quad \phi(\theta)=\alpha(e^{\theta}-1) +\beta(e^{-\theta}-1).  
\]
Let $\tilde{T}_z$ be the first time that $Q^c(t)\geq z$ holds, for $z\geq 1$. For any $\theta$ with $\phi(\theta)+c\theta \geq 0$, $X^c({t\wedge \tilde{T}_z})$ is a positive martingale bounded above by $e^{\theta z}$. By the Optional Stopping Theorem
\[
e^\theta = {\mathbb E} [ X^c(0)] = {\mathbb E} [X^c({\tilde{T}_z})] = {\mathbb E} [ e^{ \theta z - \tilde{T}_z (\phi(\theta) + c\theta)}  {\mathbb I} [ \tilde{T}_z < \infty] ].
\]
Let $\theta^*$ be the largest solution to the equation $\phi(\theta^*) + c\theta^*=0$. We have that 
\[
{\mathbb P} (\tilde{T}_z<\infty) \leq e^{-\theta^* (z-1)} 
\]
and thus for any $\theta_0\leq \theta^*$
\[
{\mathbb P} (\tilde{T}_z<\infty) \leq e^{-\theta_0 (z-1)}.
\]
Note that since $\phi(\theta) +c \theta$ is a convex function, zero at $\theta=0$ with $\phi'(0)+ c <0$. Thus $\theta_0\leq \theta*$ iff $\phi(\theta_0)+ c\theta_0 \leq 0$.

Now if $\tilde{T}_z =\infty$ then $Q(t)$ lies below the line $(z-cs : s\geq 0)$. Thus, the area under the $Q(t)$ before it hits zero is less that the area of the triangle in the positive orthant with hypotenuse $(z-cs : s\geq 0)$. That is
\[
\int_0^{\tilde{T}} Q(t) dt < \frac{z^2}{c} .
\] 
Therefore
\[
{\mathbb P} \Big( \int_0^{\tilde{T}}   Q(t) dt \geq  \frac{z^2}{c}\Big) \leq \mathbb{P}(\tilde{T}_z <\infty) \leq e^{-\theta_0 (z-1)}
\]
which after substituting $x= z^2/c$ gives the required bound \eqref{ExcusionLemma1}.

\hfill \Halmos\endproof

\iffalse
\begin{corollary}\label{ExcusionLemma3}
Suppose that $Q_1$ and $Q_2$ are two an M/M/1 queues with respective arrival rates $\alpha_1$ and $\alpha_2$  and service rates $\beta_1$ and $\beta_2$. Further we suppose that both queues are stable with $\beta_1 > \alpha_1$ and $\beta_2 > \alpha_2$, and that $Q_1$ dominates $Q_2$ in the sense that $\alpha_1>\alpha_2$ and $\beta_1 < \beta_2$. Let $\tilde{T}$ be the length of the renewal cycle of $Q_1$ from the queue being of length $1$ to the queue being empty again. Then, there exists a coupling of queues $Q_1$ and $Q_2$ such that $Q_1(t) \geq Q_2(t)$ for all $t$ and such that
\begin{equation}\label{ExcusionLemma4}
	 {\mathbb P} 
	 	\left( 
	 		\int_0^{\tilde{T}} \Big[ Q_1(s) - Q_2(s) \Big] ds 
	 		\geq 
	 		x
	 	\right) 
	 \leq 
	 e^{-\theta_0 (\sqrt{cx}-1)}
\end{equation}
where  $\phi(\theta)=(\alpha_1-\alpha_2)(e^{\theta}-1) +(\beta_2-\beta_1)(e^{-\theta}-1) $, $c>0$
	and  $\theta_0$ is such that $\phi(\theta_0)+ c\theta_0 \leq 0.$
\end{corollary}

\proof{Proof.}
Notice we can couple so that $Q_1(t) \geq Q_2(t)$ for all $t$ by considering the Markov chain with transition rates:
\begin{align*}
&
(Q_1,Q_2) \rightarrow  	(Q_1+1,Q_2+1) 
\quad\text{at rate}
\quad  \lambda_2, 
&& 
(Q_2,Q_2) \rightarrow  	((Q_1-1)_+,(Q_2-1)_+) 
\quad\text{at rate}
\quad  \mu_2, \\
&
(Q_2,Q_2) \rightarrow  	(Q_1,Q_2) \quad\text{at rate}\quad  \lambda_1 - \lambda_2,
&& (Q_1,Q_2) \rightarrow  	(Q_1,Q_2) \quad\text{at rate}\quad  \mu_2 - \mu_1.
\end{align*}
 Note that under this coupling $Q_1(t) \geq Q_2(t)$ and $Q_1(t)-Q_2(t)$ is an M/M/1 queue with arrival rate $\lambda_1- \lambda_2$ and service rate $\mu_2 -\mu_1$. The required bound \eqref{ExcusionLemma4} is now an immediate consequence of Lemma \ref{ExcusionLemma}.
 \hfill\Halmos  
\endproof
\fi

\begin{lemma}\label{ExcusionLemma4}
	Suppose that $Q$ is an M/M/1 queue with arrival rate $\alpha$ and service rate $\beta$, with $\beta > \alpha$ let $\tilde{T}$ be the length of the excursion of the $M/M/1$ queue started from zero then 
	\[
	\mathbb{E} \left[ \int_0^{\tilde{T}}\!\! \Big( Q(s) - \frac{\alpha}{\alpha-\beta} \Big) ds \right] = 0.
	\]
\end{lemma}
\proof{Proof}
The stationary distribution of $Q$ (or indeed any irreducible Markov chain) can be expressed as 
\[
\mathbb{P}_\pi (Q=q) 
	=
	\frac{
		1
		}{
		\mathbb{E} [\tilde{T}]  
		}
	\mathbb{E}  
	\left[  
		\int_0^{\tilde{T}} 
			\mathbb{I} [ Q(t) = q]
		dt
	\right] .
\]
where here $\mathbb{P}_\pi$ is the stationary distribution of $Q$. In other words, since the stationary distribution of $Q$ is geometric, we have that
\begin{equation*}
	\mathbb{E} \left[
		\int_0^{\tilde{T}} 
			\Big(
				1- \frac{\alpha}{\beta}
			\Big) 
			\Big(
				\frac{\alpha}{\beta}
			\Big)^{q}
		dt
		\right]  
	=
	\mathbb{E}  
	\left[  
		\int_0^{\tilde{T}} 
			\mathbb{I} [ Q(t) = q]
		dt
	\right] .
\end{equation*}
Multiplying by $q$ and summing over $q\in \mathbb{Z}_+$ gives the result. \hfill \Halmos 
\endproof

The following is a Functional Strong Law of Large Numbers for $L^2$ martingales and is an extension of \cite{williamsprobability} Theorem 12.13a) and Section 12.4.

\begin{lemma}[A Martingale Functional Strong Law of Large Numbers]\label{MgSLLN} Suppose that 
	\[
	M_n:= \sum_{i=1}^{n} Z_i
	\]
	defines a Martingale and is such that, for some constant $C$,
	\[
	\mathbb{E}\left[ Z_k^2 | \mathcal{F}_{k-1} \right] \leq C
	\]
	then, for all $T>0$,
	\[
	\lim_{n\rightarrow \infty}\sup_{0\leq t \leq T } \left| \frac{M_{\lfloor tn \rfloor }}{n} \right| =0.
	\]	
\end{lemma}
\proof{Proof}
By assumption, the increasing process
\[
<\! M\! >_n := \sum_{k \leq n} \mathbb{E} \left[ Z_k^2 | \mathcal{F}_{k-1} \right]  
\]
is such that $<\! M\! >_n\leq nC$. By \cite[Theorem 12.13a and 12.4]{williamsprobability}  
\begin{align*}
&\lim_{n\rightarrow \infty} \frac{M_n}{<\! M\! >_n} =0 \qquad \text{on the event}\qquad \left\{<\! M\! >_n=\infty\right\}, \\
&\lim_{n\rightarrow \infty} M_n \quad \text{exists and is finite on the event }\quad \left\{<\! M\! >_n<\infty\right\} .
\end{align*} 
Since $<\! M\! >_n\leq nC$, in both instances we have that
\[
\lim_{n\rightarrow \infty}\frac{M_n}{n} =0.
\] 




Expanding this statement, 
\begin{equation*}
\forall \epsilon >0,\quad \exists \tilde{N} \quad\text{s.t.} \quad \forall n> \tilde{N}, \qquad \left| \frac{M_n}{n}  \right| \leq \epsilon.
\end{equation*}
Notice, this also bounds our process for all suitably large times:
\begin{equation*}
\forall \epsilon >0,\quad \exists \tilde{N} \quad\text{s.t.} \quad \forall t n> \tilde{N} ,\qquad \left| \frac{M_{\lfloor tn \rfloor}}{n}  \right| \leq \epsilon t.  
\end{equation*}
This just leaves a finite number of terms, that is $\tilde{N}$ terms, to deal with. We apply the crude bound, if $tn \leq \tilde{N}$
\begin{equation*}
\left| \frac{M_{\lfloor tn \rfloor}}{n}  \right| \leq \frac{1}{n} \max_{k=1,...,\tilde{N}}  |M_k|
\end{equation*}
Notice, we can make the right-hand side of this expression small by taking $n$ much larger that $\tilde{N}$. Thus we can collect together these two cases
\begin{equation*}
\left| \frac{M_{\lfloor tn \rfloor}}{n}  \right| \leq  
\begin{cases}
\epsilon t, & \text{if } tn > \tilde{N}\\
\frac{1}{n}\max_{k=1,...,\tilde{N}}  |M_k|, &\text{if } tn \leq \tilde{N}
\end{cases}
\end{equation*}
By bounding $t\leq T$ the first case can be made arbitrarily small and, then, by choosing $n$ suitably large compared to $\tilde{N}$ the second case can be made arbitrarily small. This then proves that 
\[
\lim_{n\rightarrow \infty}\sup_{0\leq t \leq T } \left| \frac{M_{\lfloor tn \rfloor }}{n} \right| =0
\]	
as required.\hfill \halmos
\endproof

The following result is the central limit theorem counterpart of the above strong law of large numbers result. For it's proof, we refer the interested reader to the excellent survey of \cite{whitt2007}.

\begin{theorem}[Martingale Functional Central Limit Theorem]\label{MgCLT}
If $M^{(k)}=(M^{(k)}(t) : t\geq 0)$, $k\geq 0$ is sequence of continuous time Martingales whose quadratic variation $[M^{(k)}]$ converge in the Skorohod topology to the identify function:
\[
[M^{(k)}] \Rightarrow \mathbf{e}\qquad\text{as} \quad k\rightarrow \infty
\]
then 
\[
M^{(k)}\Rightarrow B
\]
where $B$ is a standard Brownian motion.
\end{theorem}
For a proof of this result see \cite[Theorem 2.1 and Lemma 2.1]{whitt2007}. The proof of the Martingale Functional Central Limit consists of verifying tightness of the Martingale sequence and then verifying L\'evy's characterization of Brownian motion for any limit of this relatively compact sequence.

\subsection{Comparison of stationary distributions}
In Section \ref{Comparison}, we state that the following stochastic bounds hold
\[
	\pi_{CQ} \leq_{st} \pi_{JSQ} =_{st} \pi_{I1F} \leq_{st} \pi_{IQF},
\]
and we state that this follows since the drift terms of each stochastic process, corresponding to $CQ$, $JSQ$, $I1F$ and $IQF$ dominate each other. This result follows from the following lemma. 

\begin{lemma}\label{St_Dom}
Consider positive recurrent stochastic differential equations 
\begin{align*}
	dX_1(t) &= - d_1(X_1(t)) dt + \sqrt{2} dB(t) \\
	dX_2(t) &= - d_2(X_2(t)) dt + \sqrt{2} dB(t) 	
\end{align*}
with stationary distributions $\pi_1(x)$ and $\pi_2(x)$ with support on $(0,\infty)$. 
%
If the drift of these processes are continuous on $(0,\infty)$ and satisfy $d_1(x)\geq d_2(x)$ then
\[
\pi_1 \leq_{st} \pi_2\ .
\]
\end{lemma}

(Within the proof, we provide comments as to how the result extends to a reflected Brownian motion with drift, as is given for the Central Queue NDS diffusion.)
\proof{Proof}
The diffusions $X_1$ and $X_2$ are Langevin Diffusions. Specifically, their generators and forward-equation are of the form
\[
\mathcal L  = \frac{d^2}{d x^2} - V'(x) \frac{d}{dx}
\]
for some differentiable function $V(x)$. 
Setting $V'_1(x) = d_1(x)$ and $V'_2(x)=d_2(x)$ 
This can be verified directly with It\^{o}'s formula. The invariant measure for such diffusions has density given by $m(x) = e^{-V(x)}$. This holds  since $\mathcal L^\dagger m(x) = 0 $ which can be verified substitution into the adjoint of the generator above, or by substitution into the Kolmogorov forward-equation. (For reflected Brownian motion with drift the same form of invariant measure holds. So our results apply here also.)

We now directly calculate and compare the stationary distributions for these processes. First note that
\[
-V_1(y) +V_1(x)=\int_x^y -d_1(u) {\rm d}u \leq \int_x^y -d_2(u) {\rm d}u = -V_2(y) + V_2(x)\ .
\]
Taking exponentials and integrating once more gives
\begin{equation}\label{Vineq}
\int_x^\infty e^{-V_1(y) + V_1(x)} {\rm d}y \leq \int_x^\infty e^{-V_2(y) + V_2(x)} {\rm d}y\ .
\end{equation}

Now note that
\[
\mathbb P_{\pi_1} ( X_1 \geq x) 
= 
\frac{
\int_x^\infty e^{-V_1(y)} dy 
}{
\int_0^\infty e^{-V_1(y)} dy
}.
\]
Taking logarithms and differentiating with respect to $x$ gives
\begin{align*}
	\frac{d}{dx} \log \mathbb P_{\pi_1} ( X_1 \geq x)  
	&
	= \int_x^\infty e^{-V_1(y) + V_1(x)} {\rm d}y
	\\
	&
	\leq  
	 \int_x^\infty e^{-V_2(y) + V_2(x)} {\rm d}y
	 =
	 \frac{d}{dx} \log \mathbb P_{\pi_2} ( X_2 \geq x)  \ .
\end{align*}
In the inequality above, we apply \eqref{Vineq}.  Thus after integrating and taking exponentials, we have that
\[
\mathbb P_{\pi_1} ( X_1 \geq x)   \leq \mathbb P_{\pi_2} ( X_2 \geq x)  
\]
Thus are required we have that $\pi_1 \leq_{st} \pi_2$.
\hfill \Halmos
\endproof





==> ECOMPANION__Neil_Walton_s_conflicted_copy_2016-12-10_.tex <==

%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ECSwitch

%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Main head for the e-companion
\ECHead{Proofs of Statements}


\section{Proof of Conjecture xxx.}


\section{Proof of Theorem \ref{thm:W_process_convergence}}
\begin{repeattheorem}[Theorem~\ref{thm:W_process_convergence}] Denoting the diffusion-scaled workload for the $r$th LPS system by $\ds W(t)$, we have:
  \begin{align}
    \ds W &\dto W^*,
  \end{align}
  where $W^*$ is a RBM with drift $-\theta(\Delta(W^*(t)) \wedge K)$ and variance $\sigma^2 = \lambda m^2(c_a^2+c_s^2)$, satisfying the initial condition 
\begin{align*}
\ds W(0) &\dto W^*(0).
\end{align*}
\end{repeattheorem}




==> LITERATURE__Neil_Walton_s_conflicted_copy_2017-02-14_.tex <==
% !TeX root    = paper.tex

\section{Literature Review} \label{sec:literature}
We review policies used for parallel server models, paying particular attention to results on JSQ and its variants; then we review asymptotic methods used to analyze these systems; finally, we review recent work on the non-degenerate slowdown regime.

\subsubsection*{Parallel Server Models}  

The earliest mathematical analysis' of Join-the-Shortest Queue are \cite{haight1958two, kingman1961two, flatto1977two}. In each case, a system with two servers is analysed. 
It was subsequently proved by \cite{winston1977optimality} that, for exponentially distributed job sizes, JSQ minimizes the number of jobs amongst policies with past queue size and arrival information. See \cite{liu1995sample} for an elegant coupling proof of this result.

The Central Queue (CQ) policy goes back to Erlang and Kendall. When the arrival and service distribution is specified, the model is called the $M/M/k$ or $G/G/k$ queue. With FIFO scheduling rule at servers, Central Queue is equivalent to the policy where jobs are dispatched to the queue with least work, see \cite[Chapter XII]{asmussen2008applied}. Thus, CQ is optimal under the broad class of dispatch policies. (In particular those having knowledge of each jobs work load, its distribution and past arrivals and assuming FIFO service at each queue). Again, see \cite[Chapter XII]{asmussen2008applied}.

Although CQ and JSQ are practical policies in some applications, such as call centres where the number of servers is moderate, in other applications, such as data centers, dispatch decision are made on the arrival of each job and with limited state information. For this reason, there has been considerable interest in finding simple policies that emulate the optimal behavior of JSQ and CQ.

\cite{mitzenmacher2001power} and \cite{vvedenskaya1996queueing} analyzed the Power-of-$d$ choices policies. One motivation for Power-of-$d$ rule is as a policy that tries to approximately emulate the performance of JSQ by randomly sampling a subset of servers. A second motivation comes from data center applications where compute jobs must be co-located with the data. By replicating each data on $d$ randomly chosen servers, the load balancing of compute tasks behaves as if the the $d$ servers were randomly sampled on the arrival of the task.   %Essentially attempting to emulate the performance of JSQ over a smaller randomly selected subset of queues.
 An alternative mechanism to emulate JSQ is to prioritize idle servers when dispatching tasks as exhibited in Idle-Queue-First Policy, see \cite{lu2011join}. As discussed above IQF emulates the behavior of an $M/M/\infty$ queue in a mean-field asymptotic and thus can be argued to outperform Po$d$. See \cite{stolyar2015pull} for a more detailed analysis and discussion. Accordingly the analysis of these policies and variants have attracted growing research interest with articles such as \cite{tsitsiklis2012power}, \cite{mukherjee2015universality}, \cite{gamarnik2016delay} and \cite{jonckheere2016asymptotics} each analyzing different trade-offs present in this modeling framework.

\iffalse
\cite{mitzenmacher2001power}\\
\cite{vvedenskaya1996queueing}\\
\cite{lu2011join}\\
\cite{stolyar2015pull}\\
\fi

%MORE RECENT WORK\\

As indicated above, although analysis of classical policies such as CQ and JSQ goes back more than fifty years, the development of more modern data centre applications have necessitated new policy variants and new methods to compare and analyse them.



\subsubsection*{Methods for Asymptotic Analysis}
We now review scaling regimes applied to CQ and JSQ%., and then we review the scaling properties that we find inherently for JSQ in the NDS regime.

Heavy traffic limits were first proposed by Kingman in order to provide simplified descriptions of queueing system that extract the key characteristics and differences in different queueing processes (this is our motivation for choosing to study load balancing in the NDS regime as well). 
Inglehart and Whitt \cite{IgWh70} first characterized the limiting diffusions of the Central Queue policy under a heavy traffic scaling.
A heavy traffic analysis of the Joint-the-Shortest-Queue for 2 servers is provided by \cite{foschini1978basic}. Following this work \cite{halfin1981heavy} developed a scaling regime for the central queue policy where the number of servers was allowed to grow with the load parameters (often called the Halfin-Whitt, or Quality-Efficiency-Driven regime). \cite{borst2004dimensioning} motivate, reformulate and refine the Halfin-Whitt regime as the cost minimizing regime for call center dimensioning. More recently \cite{eschenfeldt2015join} provide an analysis of JSQ in the Halfin-Whitt regime.  In addition to further literature review, \cite{pang2007martingale} provides a good review of methods used to characterize the limiting diffusions in the Halfin-Whitt regime. 

Mean field limits have commonly been applied to the modeling of large queueing systems, particularly in settings where queues behave approximately independently (as in the case for the Power-of-$d$ load balancing systems -- see \cite{Bramson2012}). A mean field analysis of Po$d$ was given by \cite{vvedenskaya1996queueing} and further by \cite{bramson2013decay}. Introducing dependence between queues can substantially improve performance. A mean field analysis of this effect is given by \cite{tsitsiklis2012power} and for the IQF policies by \cite{stolyar2015pull}.

\subsubsection*{Non-Degenerate Slowdown}
The Non-Degenerate Slowdown Regime was first introduced by \cite{atar2012diffusion}. Atar attributes first use of this scaling to \cite{whitt2003multiserver} and \cite{gurvich2004design} (in addition to private communications with A. Mandelbaum and G. Shaikhet) and motivates the use of NDS in call centres from emprical work where customers' slowdown can be large, \cite{brown2005statistical}.

Subsequent work in the non-degenerate slowdown regime developed notions of optimality and control, see \cite{atar2011asymptotically} and \cite{atar2014scheduling}.
Independently, the work of \cite{maglaras2013optimal} also consider the non-degenerate slowdown regime where the scaling regime is motivated by a cost minimization objective. 

The NDS regime is relatively new scaling asymptotic with most key papers appearing in the last 5 years and originating form motivations on call centre applications. Our work advocates the use of NDS in order to distinguish between load balancing policies and is primarily motivated by recent data center applications. 

\iffalse
Halfin-Whitt \cite{halfin1981heavy}\\
QED \cite{borst2004dimensioning}\\

Atar \cite{atar2012diffusion}, Gurvich \cite{gurvich2004design}, Whitt \cite{whitt2003multiserver}, Maglaras \cite{maglaras2013optimal}.\\

Follow up work by Atar \cite{atar2011asymptotically} \cite{atar2014scheduling}, \\

Empircal Work  justifying NDS in call centres \cite{brown2005statistical}.
\fi

\varun{Following paragraph needs polishing}
From a mathematical perspective, there are a rich set of phenomena that occur in the NDS regime. We find that there is separation of time-scales between a several important components of our process. Separation of timescale in Markov processes is first analysed by ???. For queueing systems, the analysis of Hunt and Kurtz provides a Martingle approach to the analysis of queueing systems. Our analysis benefited much from which further rich source of methods on analysis of timescale separations is ??. The authors chiefly opt to mimic the coupling approach of Walton ??.  Separation of timescales provides yields many limit processes as reversible Markov chains, which in turn implies the insensitivity to distribution of several phenomena. Analogous use of this time scale separation priniple is applied for insensitivity of abondoment in a Halfin-Whitt asymptotic Dai ??. Finally, understanding the separation of time-scales of the idleness process is of central importance to achieving optimal queue size behavior and leads us to analyze the I1F policy. 

\iffalse
In addition to charactering the diffusion limits under this scaling we find that properties such as time-scale separation and insensitivity are important to understanding these processes.


Fluid Limits
Heavy Traffic

A heavy traffic analysis of the Joint-the-Shortest Queue is provided by \cite{foschini1978basic}

Halfin Whitt 




QED
Mean Field
reverisiblity
time-scale separation.

\fi


==> ecompanion_v02.tex <==

%% Here starts the e-companion (EC)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ECSwitch

%\ECDisclaimer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Main head for the e-companion
\ECHead{Online Companion to}

\section{Diffusion Analysis for the Workload Processes and Its Implications}

Following from the dynamic equation \eqref{eq:workload-dynamics}, the diffusion scaled workload is
\begin{equation}\label{eq:workload-diffusion}
  \ds W(t) = \ds W(0)+\frac{1}{r}\sum_{i=1}^{\ssp{\Lambda}(r^2t)}v_i 
  - \frac{1}{r}\int_0^{r^2t}\ssp{\mu}(\ssp{Z}(s))\id{\ssp{W}(s)>0}ds
\end{equation}
Now, introduce the notation
\begin{align}
  \label{eq:Kiefer-fs}
  \fls K(t,x) &= \frac{1}{r^2}\sum_{i=1}^{\cl{r^2t}}\id{v_i\le x}\\
  \label{eq:Kiefer-ds}
  \ds K(t,x) &= r[\fls K(t,x) - t F(x)].
\end{align}
The second term in on the right hand side of \eqref{eq:workload-diffusion} can be written as
\begin{align*}
  &\quad r\int_0^t\int_0^\infty x d\fls K(\frac{1}{r^2}\ssp{\Lambda}(r^2s),x)\\
  &=\int_0^t\int_0^\infty x d\ds K(\frac{1}{r^2}\ssp{\Lambda}(r^2s),x)
  +\frac{1}{r}\int_0^t\int_0^\infty x dF(x) d\ssp{\Lambda}(r^2s)\\
  &=\int_0^t\int_0^\infty x d\ds K(\frac{1}{r^2}\ssp{\Lambda}(r^2s),x)
  + m\int_0^t d \frac{1}{r}[\ssp{\Lambda}(r^2s)-\lambda r^2s]+\lambda rmt.
\end{align*}
The last term on the right hand side of \eqref{eq:workload-diffusion} can be written as
\begin{align*}
  &\quad - r\int_0^t \ssp{\mu}(r\ds Z(s)) \id{\ssp{W}(r^2s)>0}ds\\
  &= \int_0^t r[\lambda m-\ssp{\mu}(r\ds Z(s))] ds + r\int_0^t \id{\ds W(s)=0}ds-\lambda rmt\\
  &= \int_0^t r[\lambda m-\ssp{\mu}(r\Delta(\ds W(s)))] ds 
  +  \int_0^t r[\ssp{\mu}(r\ds Z(s))-\ssp{\mu}(r\Delta(\ds W(s)))] ds \\
  &\quad  + r\int_0^t \id{\ds W(s)=0}ds-\lambda rmt\\
  &= \int_0^t \ssp{\theta}\left(\Delta(\ds W(s))\right) -
              \theta\left(\Delta(\ds W(s))\right)  ds
  +  \int_0^t r[\ssp{\mu}(r\ds Z(s))-\ssp{\mu}(r\Delta(\ds W(s)))] ds \\
  &\quad + \int_0^t \theta\left(\Delta(\ds W(s))\right)   ds
  + r\int_0^t \id{\ds W(s)=0}ds-\lambda rmt
\end{align*}
In summary, we can write the workload process as
\begin{equation}\label{eq:workload-diffusion-map}
  \begin{split}
    \ds W(t)
    &= \ds W(0) + \ds M_s(t) + \ds M_a(t) + \ds G_1(t) + \ds G_2(t)\\
    &\quad + \int_0^t \theta\left(\Delta(\ds W(s))\right) ds 
    + r\int_0^t \id{\ds W(s)=0}ds,
  \end{split}
\end{equation}
where
\begin{align}
  \label{eq:3}
  \ds M_s(t) &= \int_0^t\int_0^\infty x d\ds K(\frac{1}{r^2}\ssp{\Lambda}(r^2s),x),\\
  \ds M_a(t) &= m\int_0^t d \frac{1}{r}[\ssp{\Lambda}(r^2s)-\lambda r^2s],\\
  \ds G_1(t) &= \int_0^t r[\ssp{\mu}(r\ds Z(s))-\ssp{\mu}(r\Delta(\ds W(s)))] ds,\\
  \ds G_2(t) &= \int_0^t \ssp{\theta}\left(\Delta(\ds W(s))\right) -
              \theta\left(\Delta(\ds W(s))\right)  ds.
\end{align}

The following lemma is an extension of the classical one-dimensional Skorohod problem. The proof can be found in \cite{LeeWeerasinghe2011}.  
\begin{lemma}\label{lem-reflection-map}
  Suppose $g$ is a Lipschitz continuous function. For any $x\in\D(\R^+)$, there exists a unique pair $(y,z)\in\D^2(\R^+)$ satisfying
  \begin{align}
    \label{eq:var-sko-1}
    & z(t) = \int_0^tg(z(s))ds + x(t) + y(t),\\
    \label{eq:var-sko-1.5}
    & z(t)\ge 0,\quad \textrm{for all }t\ge 0,\\
    \label{eq:var-sko-2}
    & y(0) = 0 \textrm{ and $y$ is non-decreasing},\\
    \label{eq:var-sko-3}
    & \int_0^t z(s) dy(s) = 0.
  \end{align}
  More over, denote $z=\psi(x)$. The mapping $\psi:\D(\R^+)\to \D(\R^+)$ is continuous in the uniform topology on compact set. 
\end{lemma}


\proof{Proof of Theorem~\ref{thm:W_process_convergence} } 
  We first study the first 4 terms on the right hand side of equation \eqref{eq:workload-diffusion-map}.  For the initial condition $\ds W(0)$, its convergence to some random variable $w_0$ is part of the assumption.  

  According to Lemma~3.8 in \cite{KrichaginaPuhalskii1997}, 
  \begin{equation*}
    \int_0^t\int_0^\infty x d\ds K(\frac{1}{r^2}\ssp{\Lambda}(r^2s),x)
    \dto m M_s(t),\quad\textrm{as }r\to\infty,
  \end{equation*}
  where $M_s(t)$ is a reflected Brownian motion with zero drift and variance $c_s^2$. 
  
  It follows from the assumption~\eqref{eq:HT-arrival} that
  \begin{align*}
    \ds M_a(t)
    =m\ds \Lambda(t)\dto m M_a(t), \quad \textrm{as }r\to\infty.
  \end{align*}
  
  We now study the terms $\ds G_1$ and $\ds G_2$. By tightness proved in Section~\ref{sec:state-space-collapse}, for any $\epsilon>0$, there exists $C$ such that $\prs{\Omega_r^c}\le \epsilon$, where $\Omega_r = \left\{\sup_{t\in[0,T]}\max\left(\ds Z(s), \Delta \ds W(s)\right)\le C\right\}$. On the event $\Omega_r$, we have that
  \begin{align*}
    \ds G_1(t) &\le L_n \sup_{s\in[0,t]}\|\ds Z(s)-\ds W(s)\| T,\\
    \ds G_2(t) &= \int_0^t \epsilon ds = \epsilon T.
  \end{align*}
  This implies that $\ds G_1(\cdot)\dto 0$ and $\ds G_2(\cdot)\dto 0$ as $r\to\infty$.

  Let $\ds Y(t)=r\int_0^t \id{\ds W(s)=0}ds$, it is easy to see that 
  \begin{equation}
    \int_0^t \ds W(s)d\ds Y(s) = 0.
  \end{equation}
  Thus $(\ds W,\ds Y)$ is the solution to the reflection mapping in Lemma~\ref{lem-reflection-map}. So 
  \begin{equation*}
    \ds W = \psi\left(\ds W(0) + \ds M_s+\ds M_a+\ds G_1+\ds G_2\right).
  \end{equation*}
  By continuous mapping theorem, $\ds W\dto W^*$, where $W^*=\psi(w_0+ m M_s(t) + m M_a(t))$. In other words, the limit $W^*$ satisfies
  \begin{align}
    W^*(t) = w_0 + m M_s(t) + m M_a(t) -\theta(\Delta(W^*))(t) + Y^*(t),
  \end{align}
  with $Y^*(0)=0$ and being non-decreasing and 
  \begin{equation}
    \int_0^t W^*(s)d Y^*(s) = 0.
  \end{equation}
  Thus, we have shown that the diffusion limit of the workload process is a RBM with state dependent drift $-\theta(\Delta_K(W^*(t)) \wedge K)$ and variance $m(c_s^2+c_a^2)$. 
\Halmos
\endproof

% -----------------------------------------------------------------------------------

\proof{Proof of Theorem~\ref{thm:W_ss_convergence} } 
\Halmos
\endproof

\proof{Proof of Corollary~\ref{cor:gen_approximation} } 
\Halmos
\endproof

\proof{Proof of Corollary~\ref{cor:final_approximation} }
\Halmos
\endproof


\section{State Space Collapse for the Sd-LPS system}
\label{sec:state-space-collapse}

Recall the definition of $\psi$ in \eqref{eq:sharing}. This represents the key difference between the Sd-LPS model and the LPS model studied in \cite{ZDZ2009, ZhangDaiZwart2011}. This different prevents us from citing the results directly from the literature. In this section, we adopt the frameworks developed in \cite{ZDZ2009, ZhangDaiZwart2011} by repeating necessary notations and definitions. We try to minimize the technical details while maintaining this section to be self-contained. We emphasize the difference in analysis brought by the specifics of the Sd-LPS model.

\subsection{Measure-valued Modeling}
Though the model we have introduced is quite clear, the mathematical analysis require more information about the systems to be explicitly involved due to general service time distributions. Following the framework \cite{ZDZ2009, ZhangDaiZwart2011}, we introduce a measure-valued state descriptor $(\ssp\buf(\cdot),\ssp\ser(\cdot))$ for the $r$th system, which describes the status of the system.  Let $\ssp\buf(\cdot)$ and $\ssp\ser(\cdot)$ be $\M_1$-valued (all measures defined on $(0,\infty)$) stochastic processes.  For any Borel set $A\subset(0,\infty)$, $\buf(t)(A)$ denotes the total number of jobs in buffer whose job size belongs to $A$ and $\ser(t)(A)$ denotes the total number of jobs in service whose residual job size belongs to set $A$. It is clear that we have the following relationship 
\begin{align*} 
  \ssp{Q}(t)=\inn{1}{\ssp\buf(t)},\quad \ssp{Z}(t)=\inn{1}{\ssp{\ser}(t)}.
\end{align*}
Following \eqref{eq:cumulative} and \eqref{eq:K-r}, the accumulative service amount is
\begin{equation}
  \label{eq:accum-ser-r}
  \ssp{S}(s,t) = \int_s^t\psi(\ssp{Z}(\tau))d\tau.
\end{equation}
Introduce 
\begin{align}
  \ssp{B}(t) &= \ssp\Lambda(t)-\ssp{Q}(t).\label{eq:B(t)}
\end{align}
The intuitive explanation for $\ssp{B}$ is that $\ssp{B}(t)$ is the index of the last job who has entered service by time $t$ and
\begin{equation*}
  \ssp{B}(s,t)=\ssp{B}(t)-\ssp{B}(s)
\end{equation*}
represents the number of jobs which have entered the service during time interval $(s,t]$. 
Denote $\ssp{a}_i$ the $i$th jump point of the arrival process $\ssp\Lambda(t)$, and $\ssp\tau_i$ the time when the $i$th arriving job start to receive service.
The evolution of the system can be written as
\begin{align}
  \ssp\buf(t)(A)&=\sum_{i=\ssp{B}(t)+1}^{\ssp\Lambda(t)}\delta_{v_i}(A)\label{eq:stoc-dym-eqn-B}\\
  \ssp\ser(t)(A)&=\ssp\ser(0)(A+\ssp{S}(0,t))
  +\sum_{i=\ssp{B}(0)+1}^{\ssp{B}(t)}\delta_{v_i}(A+\ssp{S}(\ssp\tau_i,t)),\label{eq:stoc-dym-eqn-S}
\end{align}
for any Borel set $A\subseteq(0,\infty)$ and $t\ge 0$, where $\delta_a$ denotes the Dirac measure of point $a$ on $\R$ and $A+y=\{a+y:a\in A\}$.  We call \eqref{eq:stoc-dym-eqn-B} and \eqref{eq:stoc-dym-eqn-S} the \emph{stochastic dynamic equations}.
Using state descriptor $(\ssp\buf,\ssp\ser)$, we can recover the workload $\ssp{W}(t)$ at time $t>0$ by 
\begin{equation}
  \ssp{W}(t)=\inn{\chi}{\ssp\buf(t)+\ssp\ser(t)},
\end{equation}
where $\chi$ denotes the identity function on $\R$.

Let $\nu$ denote the probability measure associated with the service time distribution $G$, and $\nu_e$ be the \emph{equilibrium} measure of $\nu$, i.e.
$\nu_e([0,x])=\frac{1}{\beta}\int_0^x\nu((y,\infty))dy$ for all $x\ge 0$.  We introduce a strengthened version of the mapping $\Delta_K$ as the follows.  Let $\Delta_{K,\nu}:\R_+\to\M\times\M$ be the lifting map associated with the probability measure $\nu$ and constant $K$ given by
\begin{equation*}
  \Delta_{K,\nu} w=\Bigl(\frac{(w-K\beta_e)^+}{\beta}\nu,
  \frac{w\wedge K\beta_e}{\beta_e}\nu_e\Bigr)
  \quad\textrm{ for }w\in\R_+.
\end{equation*}

Assume there exists $(\xi^*,\mu^*)\in\M\times\M$ such that
\begin{align}
  \label{eq:cond-initial}
  (\ds\buf(0),\ds\ser(0))&\dto(\xi^*,\mu^*),\\
  \label{eq:cond-initial-u}
  \inn{\chi^{1+p}}{\ds\buf(0)+\ds\ser(0)}&\dto\inn{\chi^{1+p}}{\xi^*+\mu^*}\quad \textrm{for some }p>0,
\end{align}
as $r\to\infty$, and
\begin{align}
  \label{eq:cond-init-ssc}
  & (\xi^*,\mu^*)=\Delta_{K,\nu}w^*,\\
  \label{eq:cond-initial-noatom}
  & \mu^* \textrm{ has no atoms}. 
\end{align}
We aim to prove the following full version of the state space collapse 
\begin{theorem}[Full State Space Collapse]\label{thm:full-ssc}
  Under the conditions \eqref{eq:HT-arrival}--\eqref{eq:cond-HT} and \eqref{eq:cond-initial}--\eqref{eq:cond-initial-noatom}, for any $T>0$,
  \begin{equation*}
    \sup_{t\in[0,T]}\pov[(\ds\buf(t),\ds\ser(t)),\Delta_{K,\nu}\ds W(t)]
    \dto 0\quad\textrm{ as }r\to\infty.    
  \end{equation*}
\end{theorem}
It is clear that Theorem~\ref{thm:full-ssc} implies Proposition~\ref{prop:state_space_collapse}. The rest of this section is devoted to the proof of the full SSC.

\subsection{Tightness of Shifted Fluid Scaled Processes}
The key idea of proving SSC, which was originally developed by \cite{Bramson1998}, is to ``chop'' the diffusion scaled processes into pieces. 

\noindent\textbf{Shifted Fluid Scaling}
\begin{equation}
  \sfs\buf(t)=\frac{1}{r}\ssp{\buf}(rl+rt),\quad
  \sfs\ser(t)=\frac{1}{r}\ssp{\ser}(rl+rt),
\end{equation}
for all $m\in\N$ and $t\ge 0$.
To see the relationship between these two scalings, consider the diffusion scaled process on the interval $[0,T]$, which corresponds to the interval $[0,r^2T]$ for the unscaled process.  Fix a constant $L>1$, the interval will be covered by the $\fl{rT}+1$ overlapping intervals 
\[[rl,rl+rL]{\hskip 15 pt}l=0,1,\cdots,\fl{rT}.\] 
For each $t\in[0,T]$, there exists an $l\in\{0,\cdots,\fl{rT}\}$ and $s\in[0,L]$ (which may not be unique) such that $r^2t=rl+rs$. Thus 
\begin{equation}\label{eq:relation-frm-dr}
  \ds{\buf}(t)=\sfs{\buf}(s),\quad\ds{\ser}(t)=\sfs{\ser}(s).
\end{equation}
This will serve as a key relationship between fluid and diffusion scaled processes.

The quantities $\ssp{Q}(\cdot)$, $\ssp{Z}(\cdot)$, $\ssp{X}(\cdot)$, $\ssp{W}(\cdot)$ are essentially functions of $(\ssp{\buf}(\cdot),\ssp{\ser}(\cdot))$, so the scaling for these quantities is defined as the functions of the corresponding scaling for $(\ssp{\buf}(\cdot),\ssp{\ser}(\cdot))$. For example
\begin{align*}
  % \sfs{Q}(t)&=\inn{1}{\sfs\buf(t)}=\frac{1}{r}\ssp{Q}(rl+rt),\\
  % \sfs{Z}(t)&=\inn{1}{\sfs\ser(t)}=\frac{1}{r}\ssp{Z}(rl+rt),\\
  % \sfs{X}(t)&=\inn{1}{\sfs\ser(t)+\sfs\ser(t)}=\frac{1}{r}\ssp{X}(rl+rt),\\
  \sfs{W}(t)&=\inn{\chi}{\sfs\buf(t)+\sfs\ser(t)}=\frac{1}{r}\ssp{W}(rl+rt).
\end{align*}
We define the shifted fluid scaling for the arrival process as
\begin{equation*}
  \sfs \Lambda(t)=\frac{1}{r}\ssp{\Lambda}(rl+rt),
\end{equation*}
for all $t\ge 0$.  By \eqref{eq:B(t)}, the shifted fluid scaling for
$\ssp{B}(\cdot)$ is
\begin{equation*}
  \sfs B(t)=\sfs E(t)-\sfs Q(t),
\end{equation*}
for all $t\ge 0$.
A shifted fluid scaled version of the stochastic dynamic equations
\eqref{eq:stoc-dym-eqn-B} and \eqref{eq:stoc-dym-eqn-S} can be written
as, for any $A\subset (0,\infty)$, $0\le s\le t$,
\begin{eqnarray}
  \label{eq:mechanism-B}
  &&\begin{split}
    \sfs\buf(t)(A)&=\sfs\buf(s)(A)
    +\frac{1}{r}\sum_{i=r\sfs E(s)+1}^{r\sfs E(t)}\delta_{v_i}(A)\\
    &\quad-\frac{1}{r}\sum_{i=r\sfs B(s)+1}^{r\sfs B(t)} \delta_{v_i}(A),
  \end{split}\\
  \label{eq:mechanism-S}
  &&\begin{split}
    \sfs\ser(t)(A)&=\sfs\ser(s)(A+\ssp{S}(rl+rs,rl+rt))\\
                  &\quad+\frac{1}{r}\sum_{i=r\sfs B(s)+1}^{r\sfs B(t)}
                   \delta_{\ssp{v}_i}(A+\ssp{S}(\ssp{\tau}_i,rl+rt)).
  \end{split}
\end{eqnarray}
We point out that the accumulative service process $\ssp{S}$ is never scaled because it tracks the received service amount for each individual customer. However, via some algebra we can see that
\begin{equation}
  \label{eq:accum-ser-sfs}
  \ssp{S}(rl+rs,rl+rt) 
  = \int_{fl+rs}^{rl+rt} \frac{\ssp{\mu}(\ssp{Z}(\tau))}{\ssp{Z}(\tau)}d\tau
  = \int_{s}^{t} \frac{\ssp{\mu}(r\sfs{Z}(\tau))}{\sfs{Z}(\tau)}d\tau.
\end{equation}
This gives two interesting observations. First, the shifted fluid scaling is essentially fluid scaling, meaning the shifted fluid scaled processes should be close to some fluid model solutions. Second, the corresponding fluid model is essentially the same as the fluid model in \cite{ZhangDaiZwart2011} since by \eqref{eq:cond-HT} that
\begin{equation*}
  \ssp{\mu}(r\sfs{Z}(\tau)) = 1 + O^+(\frac{1}{r})
\end{equation*}
where $O(1/r)$ means the quantity is positive and of the same order as $1/r$ when $r\to\infty$. So
\begin{equation}
  \label{eq:accum-ser-r-est}
  \ssp{S}(rl+rs,rl+rt) 
  = \int_{s}^{t} \frac{1}{\sfs{Z}(\tau)}d\tau
  +O^+(\frac{1}{r}).
\end{equation}
Intuitively, $\sfs{Z}$ is close to some fluid limit denoted by $\tilde Z$ as $r$ becomes very large (in the mathematical sense of convergence in probability), then 
\begin{equation}
  \ssp{S}(rl+rs,rl+rt) 
  \dto \int_{s}^{t} \frac{1}{\tilde{Z}(\tau)}d\tau.
\end{equation}
So we can conclude that the underlying fluid is the same as the one for the regular LPS system. Thus, we can use existing properties developed in \cite{ZhangDaiZwart2011}.
We hope to make the argument rigorous and concise in the follows.

\noindent\textbf{Some Bound Estimation}\\
The tightness property, which guarantees that the shifted fluid scaled process $\{\sfs{\buf},\sfs{\ser}\}$ has convergent subsequence, can be proved in a similar way as in \cite{ZhangDaiZwart2011}. There are two key differences. First is the service process as pointed out before. Second, is that \cite{ZhangDaiZwart2011} heavily relies on the known result on the diffusion of the workload (see Proposition~2.1). However, we do not have such a diffusion limit of workload a priori. Instead, we try to prove such diffusion limit by SSC. Looking into the details of the machinery in \cite{ZhangDaiZwart2011}, what essentially is needed about the workload process is some kind of stochastic bound, which we prove in the following lemma.

\begin{lemma}[An Upper Bound of the Workload]
  \label{lem:workload-upperbound}
  For any $\eta>0$ there exists a constant $M$ such that
  \begin{equation}\label{ineq:W-bound}
    \prs{
      \max_{l\le {rT}}\sup_{t\in[0,L]}\sfs{W}(t)<M
    }>1-\eta.
  \end{equation}
\end{lemma}
\proof{Proof}
Using the relationship between the shifted fluid scaling and diffusion scaling, we essentially need to prove that 
  \begin{equation*}
    \prs{
      \sup_{t\in[0,L]}\ds{W}(t)<M
    }>1-\eta.
  \end{equation*}
 Recall the representation \eqref{eq:workload-diffusion-map} for the diffusion scaled workload processes.
Since $\theta(x)\ge 0$ for all $x$, so the process $\ds W_1$ satisfying
 \begin{equation*}
    \ds W_1(t)
    = \ds W(0) + \ds M_s(t) + \ds M_a(t) + \ds G_1(t) + \ds G_2(t)
    + r\int_0^t \id{\ds W_1(s)=0}ds,
\end{equation*}
is an upperbound of $\ds W$. By Lemma~\ref{lem-reflection-map}, $\ds W_1$ converges to a driftless reflected Brownian motion, which is stochastic bounded. This implies the result.
\Halmos
\endproof

Such an stochastic bound of the workload process helps to establish some useful bound estimation for the stochastic processes underlying the Sd-LPS model. 
\begin{lemma}[Further Bound Estimations]
  \label{lem:bound-estimation}
  For any $\eta>0$, there exists a constant $M>0$ and a probability event $\Omega^r_B(M)$ for each index $r$ such that
  \begin{equation}\label{ineq:Omega-B}
    \liminf_{r\to\infty}\prs{\Omega^r_B(M)}\ge 1-\eta,
  \end{equation}
  and on the event $\Omega^r_B(M)$, we have
  \begin{align}
    \label{eq:Q-bound}
    &\max_{l\le\fl{rT}}\sup_{t\in[0,L]} \sfs Q(t)\le M,\\
    \label{eq:mvp-p-bound}
    &\max_{l\le\fl{rT}}\sup_{t\in[0,L]}
       \inn{\chi^{1+p}}{\sfs\buf(t)+\sfs\ser(t)}\le M.
  \end{align}
\end{lemma}
\proof{Proof}
The result \eqref{eq:Q-bound} holds due to Lemma~4.2 in \cite{ZhangDaiZwart2011}, which only utilize the regularity of the arrival process \eqref{eq:HT-arrival} and the stochastic bound \eqref{ineq:W-bound} for the workload process proved in Lemma~\ref{lem:workload-upperbound}. For \eqref{eq:mvp-p-bound}, the first half $\max_{l\le\fl{rT}}\sup_{t\in[0,L]}\inn{\chi^{1+p}}{\sfs\buf(t)}\le M$ also follows the same reasoning as Lemma~4.3 in \cite{ZhangDaiZwart2011}. Essentially, any results for the ``queue'' part follows the same argument in \cite{ZhangDaiZwart2011}. 

The challenge brought by the state-dependent service rate lies in the analysis of the server. It follows from the shifted-fluid scaled dynamic equation \eqref{eq:mechanism-S} that for any Borel set $A\subset (0,\infty)$, 
\begin{align*}
  \frac{1}{r}\ssp\ser(rl+rt)(A)
  &=\frac{1}{r}\ssp\ser(0)(A+\ssp{S}(0,rl+rt))\\
  &+\sum_{j=0}^{m-1}\frac{1}{r}\sum_{i= \ssp{B}(r(l-j-1))+1}^{\ssp{B}(r(l-j))}
  \delta_{v_i}(A+\ssp{S}({\ssp{\tau}_i},rl+rt))\\
  &+\frac{1}{r}\sum_{i=\ssp{B}(rl)+1}^{\ssp{B}(rl+rt)}
  \delta_{v_i}(A+\ssp{S}({\ssp{\tau}_i},rl+rt)).   
\end{align*}
Given $0\le j\le m-1$, for those $i$'s with $\ssp{B}(r(l-j-1))<i\le \ssp{B}(r(l-j))$ we have
\[{\ssp{\tau}_i}\in[r(l-j-1),r(l-j)].\]
For the sake of simplicity, let's assume that $\ssp{Z}(s)>0$ for all $s\in[0,rl+rt]$. If this does not hold, there is some technical trick presented in the proof of Lemma~4.3 in \cite{ZhangDaiZwart2011} to deal with it.  Here we show the main difference coming from the state dependent service rate. By \eqref{eq:accum-ser-r-est} and the fact that $\ssp{Z}\le \ssp{k}$, we have a lower bound on the cumulative service amount
\begin{equation}
  \label{eq:accu-ser-lower-bound}
  \ssp{S}(rs,rt) \ge \int_{rs}^{rt}\frac{1}{\ssp{Z}(s)}ds
  \ge \frac{r(t-s)}{\ssp{k}}.
\end{equation}
Thus,
\begin{equation*}
  \ssp{S}({\ssp{\tau}_i},rl+rt)\ge
  \ssp{S}(r(l-j),rl)
  \ge\frac{rj}{\ssp{k}}\ge\frac{j}{2K},    
\end{equation*}
for all large $r$ where the last inequality is due to \eqref{eq:K-r}.  For those $i$'s such that $\ssp{\tau}_i$ larger than $\ssp{B}(rl)$, we use the trivial lower bound $\ssp{S}({\ssp{\tau}_i},rl+rt)\ge 0$.  Also take the trivial lower bound that $\ssp{S}(0,rl+rt)\ge 0$.  Then we have the following inequality on the $(1+p)$th moment
\begin{equation}\label{ineq:1+p-moment-bound-est-1}
  \begin{split}
    \inn{\chi^{1+p}}{\frac{1}{r}\ssp{\ser}(rl+rt)}
    &\le\inn{\chi^{1+p}}{\frac{1}{r}\ssp{\ser}(0)}\\
    &+\sum_{j=0}^{m-1}
    \inn{\big((\chi-\frac{j}{2K})^+\big)^{1+p}}
    {\frac{1}{r}\sum_{i= \ssp{B}(r(l-j-1))+1}^{\ssp{B}(r(l-j))}\delta_{v_i}}\\
    &+\inn{\chi^{1+p}}
    {\frac{1}{r}\sum_{i=\ssp{B}(rl)+1}^{\ssp{B}(rl+rt)}\delta_{v_i}}.
  \end{split}
\end{equation}
This is the same as (4.22) in \cite{ZhangDaiZwart2011}. The estimation of the first term on the right hand side in the above follows directly from the initial condition \eqref{eq:cond-initial-u}. The analysis of the second and third terms follows the same way as in \cite{ZhangDaiZwart2011}. 
\Halmos
\endproof

To prove that a family of measure-valued processes is tight, there are three properties to verify, namely \emph{Compact Containment}, \emph{Asymptotic Regularity} and \emph{Oscillation Bound}. For brevity, we will not repeat the exact mathematical statements and their proofs. For the LPS system, these three properties were proved in Lemmas~4.4--4.6 in \cite{ZhangDaiZwart2011}. We just point out that the proof for the above mentioned three properties for the Sd-LPS system relies on b) the bound estimate in Lemma~\ref{lem:bound-estimation}; b) the fact that \eqref{eq:accum-ser-r-est} implies the lower bound for the accumulative service process \eqref{eq:accu-ser-lower-bound}. We hope the proof of Lemma~\ref{lem:bound-estimation} has demonstrated point b) clearly, and omit further repeat of the argument used in \cite{ZhangDaiZwart2011}. So we reach the conclusion

\begin{proposition}[Tightness of Shifted Fluid Scaled Processes]
  The family of shifted fluid scaled processes $\{(\sfs\buf,\sfs\ser\}_{l\le rT, r\in\N}$ is tight.  
\end{proposition}

Loosely speaking, tightness means that any subsequence from the family of shifted fluid scaled processes has convergent subsequence. This is formally stated in Theorem~4.1 in \cite{ZhangDaiZwart2011}. 

\subsection{Bramson's Framework for SSC}
The Sd-LPS and LPS essentially use the same measure-valued framework. The difference lies in the accumulative service process as we explained when deriving \eqref{eq:accum-ser-r-est} and the workload process as we studied in Lemma~\ref{lem:workload-upperbound}. After obtaining the tightness, same adoption of the framework invented by \cite{Bramson1998} applies. The adoption of Bramson's framework to the measure-valued process has been done in Section~5 in \cite{ZhangDaiZwart2011}. The high level logic is as the follows: shifted fluid scaled processes are ``close'' to the fluid model solution, and fluid model solution converges to some invariant which exhibit SSC (Theorem~3.1 in \cite{ZhangDaiZwart2011}). Thus SSC, which happens on the diffusion scaling, can be proved based on the relationship \eqref{eq:relation-frm-dr} between diffusion scaling and shifted fluid scaling. We thus refer to Section~5 in \cite{ZhangDaiZwart2011} as the proof of Theorem~\ref{thm:full-ssc}. 


% ====================================================================================

% \begin{repeattheorem}[Theorem~\ref{thm:W_process_convergence}] Denoting the diffusion-scaled workload for the $r$th LPS system by $\ds W(t)$, we have:
%   \begin{align}
%     \ds W &\dto W^*,
%   \end{align}
%   where $W^*$ is a RBM with drift $-\theta(\Delta(W^*(t)) \wedge K)$ and variance $\sigma^2 = \lambda m^2(c_a^2+c_s^2)$, satisfying the initial condition 
% \begin{align*}
% \ds W(0) &\dto W^*(0).
% \end{align*}
% \end{repeattheorem}


% \begin{lemma}
% \label{aux-lem1}
% In a 
% \end{lemma}


% \proof{Proof of Lemmas \ref{aux-lem1} } See 
% \Halmos
% \endproof



